Multiparty Motion Coordination: From Choreographies to Robotics Programs

We present a programming model and typing discipline for complex multi-robot coordination programming. Our model encompasses both synchronisation through message passing and continuous-time dynamic motion primitives in physical space. We specify \emph{continuous-time motion primitives} in an assume-guarantee logic that ensures compatibility of motion primitives as well as collision freedom. We specify global behaviour of programs in a \emph{choreographic} type system that extends multiparty session types with jointly executed motion primitives, predicated refinements, as well as a \emph{separating conjunction} that allows reasoning about subsets of interacting robots. We describe a notion of \emph{well-formedness} for global types that ensures motion and communication can be correctly synchronised and provide algorithms for checking well-formedness, projecting a type, and local type checking. A well-typed program is \emph{communication safe}, \emph{motion compatible}, and \emph{collision free}. Our type system provides a compositional approach to ensuring these properties. We have implemented our model on top of the ROS framework. This allows us to program multi-robot coordination scenarios on top of commercial and custom robotics hardware platforms. We show through case studies that we can model and statically verify quite complex manoeuvres involving multiple manipulators and mobile robots---such examples are beyond the scope of previous approaches.

==> abstract.tex <==
We present a programming model and typing discipline for complex multi-robot coordination programming.
Our model encompasses both synchronisation through message passing and continuous-time 
dynamic motion primitives in physical space.
We specify \emph{continuous-time motion primitives} in an assume-guarantee 
logic that ensures compatibility of motion primitives as well as collision freedom.
We specify global behaviour of programs in a \emph{choreographic} type system that extends
multiparty session types with jointly executed motion primitives, predicated refinements, 
as well as a \emph{separating conjunction} that allows reasoning about subsets of interacting
robots.
We describe a notion of \emph{well-formedness} for global types 
that ensures motion and communication can be correctly synchronised and provide algorithms for
checking well-formedness, projecting a type, and local type checking.
A well-typed program is \emph{communication safe}, \emph{motion compatible}, and \emph{collision free}.
Our type system provides a compositional approach to ensuring these properties.

We have implemented our model on top of the ROS framework.
This allows us to program multi-robot coordination scenarios 
on top of commercial and custom robotics hardware platforms.
We show through case studies that we can model and statically verify quite
complex manoeuvres involving multiple manipulators and mobile robots---such
examples are beyond the scope of previous approaches.
%
% We present a proof system to formally and compositionally reason about complex robotics applications.
% Our proof system is unique in that it simultaneously reasons about computation, communication,
% and control of physical components situated in 3D space.
% Such reasoning is essential in the verification of 
% robotics assemblies: correctness for these systems involve the interplay between
% control, coordination through communication, and geometric reasoning to avoid collisions.
% 
% We present our proof system on a core imperative language with synchronous message passing
% and physical dynamics.
% Our proof system has two ingredients.
% First, we abstract from continuous-time trajectories to \emph{abstract motion primitives}.
% We provide an \emph{assume guarantee logic} to reason compositionally about physical state
% and to abstract a piece of code to a motion primitive.
% The proof system checks for the existence of joint trajectories in coupled dynamical systems as
% well as that two components do not collide in space.
% 
% Second, we extend \emph{multiparty session types} to reason about synchronisation through message passing
% as well as dynamics.
% Our type system extends motion session types with predicate refinements and with abstract motion
% primitives.
% Overall, our proof system ensures that a type-correct program is \emph{communication safe}---it does
% not get stuck sending messages without recipients---and \emph{collision free}---any two components
% are always separated in space.
% We are able to use many techniques from classical program logics through
% the use of nonstandard models in our operational semantics, which allows modeling 
% continuous-time trajectories with (infinitesimally small) discrete-time steps.
% 
% Together, we show for the first time how one can compositionally reason about
% complex coordinated robotic control. 




==> acks.tex <==
We thank the OOPSLA reviewers for useful comments and suggestions; and
Julia Gabet for testing the artifact.
Majumdar and Zufferey are supported in part by 
the Deutsche Forschungsgemeinschaft project 389792660 TRR 248--CPEC
% (see \url{https://perspicuous-computing.science})
and by the European Research Council under the
Grant Agreement 610150 (http://www.impact-erc.eu/) (ERC Synergy Grant ImPACT).
Yoshida is supported in part by
  EPSRC EP/T006544/1, EP/K011715/1, EP/K034413/1, EP/L00058X/1, EP/N027833/1,
  EP/N028201/1, EP/T006544/1, EP/T014709/1 and EP/V000462/1, and NCSS/EPSRC VeTSS. 




==> basic_example.tex <==
\begin{figure*}[t]
{
  \small
\begin{align*}
\mu & \ty. \!\!\!\!\!
% \colorlet{oldcolor}{.}\color{green}\boxed{\color{oldcolor}
% \Cart\to \Green: \START.\Cart\to\Red:\START
% }.\\
 & 
  \left( \begin{array}{l}
     \left( 
          \begin{array}{l}  
                    \colorlet{oldcolor}{.} \color{blue}\boxed{\color{oldcolor}\Cart\to\Green:\ARRIVE.\Cart\to\Red:\FREE}.  \\[5px]
                    \left(\begin{array}{cc}
                         \left( \colorlet{oldcolor}{.} \color{green} \boxed{\color{oldcolor} \begin{array}{l}
                             \motion{\dtsess}{\Cart:\MOVEM^\delayed(\mathsf{point}),\Green:\WORKM^\instantaneous}.\\
                             \Cart\to\Green:\READY.\\
                              \motion{\dtsess}{\Cart:\IDLEM^\instantaneous,\Green:\PICKM^\delayed}.\\ 
                             \Green\to\Cart:\OK.\\
                             (\motion{\dtsess}{\Cart:\MOVEM^\delayed(\mathsf{point})} ~\GLPAR~ \motion{\dtsess}{\Green:\WORKM^\instantaneous})
                         \end{array}}  \color{oldcolor} \right)
                      & \!\!\GLPAR~ \motion{\dtsess}{\Red:\WORKM^\instantaneous}
                      \end{array} \right)
 \end{array}\right) \\
 + \\
 \big( \text{\quad as the above swapping $\Green$ with $\Red$\quad } \big) 
 \end{array} \right).\ty
\end{align*}
}
\vspace{-3mm}
\caption{Global choreography for the example\label{fig:basic-example}}
\vspace*{-4mm}
\end{figure*}


==> basic_example_figure.tex <==
% Gradient Info
  
\tikzset {_mwlgzwu4u/.code = {\pgfsetadditionalshadetransform{ \pgftransformshift{\pgfpoint{89.1 bp } { -108.9 bp }  }  \pgftransformscale{1.32 }  }}}
\pgfdeclareradialshading{_4euyx15e0}{\pgfpoint{-72bp}{88bp}}{rgb(0bp)=(1,1,1);
rgb(0bp)=(1,1,1);
rgb(25bp)=(0,0,0);
rgb(400bp)=(0,0,0)}

% Gradient Info
  
\tikzset {_7ai0opi17/.code = {\pgfsetadditionalshadetransform{ \pgftransformshift{\pgfpoint{89.1 bp } { -108.9 bp }  }  \pgftransformscale{1.32 }  }}}
\pgfdeclareradialshading{_co9gpcsuk}{\pgfpoint{-72bp}{88bp}}{rgb(0bp)=(1,1,1);
rgb(0bp)=(1,1,1);
rgb(25bp)=(0,0,0);
rgb(400bp)=(0,0,0)}

% Gradient Info
  
\tikzset {_eoe8gdy8h/.code = {\pgfsetadditionalshadetransform{ \pgftransformshift{\pgfpoint{89.1 bp } { -108.9 bp }  }  \pgftransformscale{1.32 }  }}}
\pgfdeclareradialshading{_dhd3hjkey}{\pgfpoint{-72bp}{88bp}}{rgb(0bp)=(1,1,1);
rgb(0bp)=(1,1,1);
rgb(25bp)=(0,0,0);
rgb(400bp)=(0,0,0)}

% Gradient Info
  
\tikzset {_cis49r535/.code = {\pgfsetadditionalshadetransform{ \pgftransformshift{\pgfpoint{89.1 bp } { -108.9 bp }  }  \pgftransformscale{1.32 }  }}}
\pgfdeclareradialshading{_9wx7ylssl}{\pgfpoint{-72bp}{88bp}}{rgb(0bp)=(1,1,1);
rgb(0bp)=(1,1,1);
rgb(25bp)=(0,0,0);
rgb(400bp)=(0,0,0)}
\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-0.6,xscale=0.6]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Straight Lines [id:da23197315574045008] 
\draw    (177,145) -- (400.5,146) ;
%Shape: Rectangle [id:dp6936911124730185] 
\draw   (256.5,128) -- (318.5,128) -- (318.5,138) -- (256.5,138) -- cycle ;
%Shape: Circle [id:dp9503375349756615] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (263.5,138.5) .. controls (263.5,134.08) and (267.08,130.5) .. (271.5,130.5) .. controls (275.92,130.5) and (279.5,134.08) .. (279.5,138.5) .. controls (279.5,142.92) and (275.92,146.5) .. (271.5,146.5) .. controls (267.08,146.5) and (263.5,142.92) .. (263.5,138.5) -- cycle ;
%Shape: Circle [id:dp7091290910424632] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (296.5,139) .. controls (296.5,134.44) and (300.19,130.75) .. (304.75,130.75) .. controls (309.31,130.75) and (313,134.44) .. (313,139) .. controls (313,143.56) and (309.31,147.25) .. (304.75,147.25) .. controls (300.19,147.25) and (296.5,143.56) .. (296.5,139) -- cycle ;
%Shape: Trapezoid [id:dp6938704427934026] 
\draw   (434,146) -- (428,126) -- (403.74,126) -- (397.74,146) -- cycle ;
%Shape: Donut [id:dp5750186371629784] 
\path  [shading=_4euyx15e0,_mwlgzwu4u] (419.45,126.5) .. controls (419.45,124.22) and (417.85,122.37) .. (415.87,122.37) .. controls (413.89,122.37) and (412.29,124.22) .. (412.29,126.5) .. controls (412.29,128.78) and (413.89,130.63) .. (415.87,130.63) .. controls (417.85,130.63) and (419.45,128.78) .. (419.45,126.5)(424.81,126.5) .. controls (424.81,121.25) and (420.81,117) .. (415.87,117) .. controls (410.93,117) and (406.93,121.25) .. (406.93,126.5) .. controls (406.93,131.75) and (410.93,136) .. (415.87,136) .. controls (420.81,136) and (424.81,131.75) .. (424.81,126.5) ; % for fading 
 \draw   (419.45,126.5) .. controls (419.45,124.22) and (417.85,122.37) .. (415.87,122.37) .. controls (413.89,122.37) and (412.29,124.22) .. (412.29,126.5) .. controls (412.29,128.78) and (413.89,130.63) .. (415.87,130.63) .. controls (417.85,130.63) and (419.45,128.78) .. (419.45,126.5)(424.81,126.5) .. controls (424.81,121.25) and (420.81,117) .. (415.87,117) .. controls (410.93,117) and (406.93,121.25) .. (406.93,126.5) .. controls (406.93,131.75) and (410.93,136) .. (415.87,136) .. controls (420.81,136) and (424.81,131.75) .. (424.81,126.5) ; % for border 

%Shape: Donut [id:dp7264825829475394] 
\path  [shading=_co9gpcsuk,_7ai0opi17] (394.31,101.5) .. controls (394.31,99.22) and (392.71,97.37) .. (390.73,97.37) .. controls (388.75,97.37) and (387.15,99.22) .. (387.15,101.5) .. controls (387.15,103.78) and (388.75,105.63) .. (390.73,105.63) .. controls (392.71,105.63) and (394.31,103.78) .. (394.31,101.5)(399.67,101.5) .. controls (399.67,96.25) and (395.67,92) .. (390.73,92) .. controls (385.79,92) and (381.78,96.25) .. (381.78,101.5) .. controls (381.78,106.75) and (385.79,111) .. (390.73,111) .. controls (395.67,111) and (399.67,106.75) .. (399.67,101.5) ; % for fading 
 \draw   (394.31,101.5) .. controls (394.31,99.22) and (392.71,97.37) .. (390.73,97.37) .. controls (388.75,97.37) and (387.15,99.22) .. (387.15,101.5) .. controls (387.15,103.78) and (388.75,105.63) .. (390.73,105.63) .. controls (392.71,105.63) and (394.31,103.78) .. (394.31,101.5)(399.67,101.5) .. controls (399.67,96.25) and (395.67,92) .. (390.73,92) .. controls (385.79,92) and (381.78,96.25) .. (381.78,101.5) .. controls (381.78,106.75) and (385.79,111) .. (390.73,111) .. controls (395.67,111) and (399.67,106.75) .. (399.67,101.5) ; % for border 

%Straight Lines [id:da3295560472533152] 
\draw [line width=2.25]    (415.87,117) -- (399.67,101.5) ;
%Straight Lines [id:da024676671233982317] 
\draw [line width=2.25]    (406.93,126.5) -- (390.73,111) ;
%Straight Lines [id:da3897211783479426] 
\draw [line width=2.25]    (385.17,95) -- (366.8,102) ;
%Straight Lines [id:da09009712306824369] 
\draw [line width=2.25]    (383.24,108) -- (368.73,112) ;
%Straight Lines [id:da3956873498966671] 
\draw    (365.83,97) -- (370.67,117) ;
%Shape: Triangle [id:dp21495214354306902] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (357.5,102.59) -- (365.53,98.71) -- (366.35,102.1) -- cycle ;
%Shape: Triangle [id:dp6457811552629551] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (360.4,116.59) -- (368.43,112.71) -- (369.25,116.1) -- cycle ;

%Shape: Trapezoid [id:dp5843282139175887] 
\draw   (139.5,145) -- (145.5,125) -- (171.1,125) -- (177.1,145) -- cycle ;
%Shape: Donut [id:dp30824825158076785] 
\path  [shading=_dhd3hjkey,_eoe8gdy8h] (154.59,125.5) .. controls (154.59,123.33) and (156.25,121.57) .. (158.3,121.57) .. controls (160.35,121.57) and (162.01,123.33) .. (162.01,125.5) .. controls (162.01,127.67) and (160.35,129.43) .. (158.3,129.43) .. controls (156.25,129.43) and (154.59,127.67) .. (154.59,125.5)(149.03,125.5) .. controls (149.03,120.25) and (153.18,116) .. (158.3,116) .. controls (163.42,116) and (167.58,120.25) .. (167.58,125.5) .. controls (167.58,130.75) and (163.42,135) .. (158.3,135) .. controls (153.18,135) and (149.03,130.75) .. (149.03,125.5) ; % for fading 
 \draw   (154.59,125.5) .. controls (154.59,123.33) and (156.25,121.57) .. (158.3,121.57) .. controls (160.35,121.57) and (162.01,123.33) .. (162.01,125.5) .. controls (162.01,127.67) and (160.35,129.43) .. (158.3,129.43) .. controls (156.25,129.43) and (154.59,127.67) .. (154.59,125.5)(149.03,125.5) .. controls (149.03,120.25) and (153.18,116) .. (158.3,116) .. controls (163.42,116) and (167.58,120.25) .. (167.58,125.5) .. controls (167.58,130.75) and (163.42,135) .. (158.3,135) .. controls (153.18,135) and (149.03,130.75) .. (149.03,125.5) ; % for border 

%Shape: Donut [id:dp3306790068033889] 
\path  [shading=_9wx7ylssl,_cis49r535] (180.66,100.5) .. controls (180.66,98.33) and (182.32,96.57) .. (184.37,96.57) .. controls (186.42,96.57) and (188.08,98.33) .. (188.08,100.5) .. controls (188.08,102.67) and (186.42,104.43) .. (184.37,104.43) .. controls (182.32,104.43) and (180.66,102.67) .. (180.66,100.5)(175.1,100.5) .. controls (175.1,95.25) and (179.25,91) .. (184.37,91) .. controls (189.5,91) and (193.65,95.25) .. (193.65,100.5) .. controls (193.65,105.75) and (189.5,110) .. (184.37,110) .. controls (179.25,110) and (175.1,105.75) .. (175.1,100.5) ; % for fading 
 \draw   (180.66,100.5) .. controls (180.66,98.33) and (182.32,96.57) .. (184.37,96.57) .. controls (186.42,96.57) and (188.08,98.33) .. (188.08,100.5) .. controls (188.08,102.67) and (186.42,104.43) .. (184.37,104.43) .. controls (182.32,104.43) and (180.66,102.67) .. (180.66,100.5)(175.1,100.5) .. controls (175.1,95.25) and (179.25,91) .. (184.37,91) .. controls (189.5,91) and (193.65,95.25) .. (193.65,100.5) .. controls (193.65,105.75) and (189.5,110) .. (184.37,110) .. controls (179.25,110) and (175.1,105.75) .. (175.1,100.5) ; % for border 

%Straight Lines [id:da08267629863338244] 
\draw [line width=2.25]    (158.3,116) -- (175.1,100.5) ;
%Straight Lines [id:da5117197942692417] 
\draw [line width=2.25]    (167.58,125.5) -- (184.37,110) ;
%Straight Lines [id:da6225215240693751] 
\draw [line width=2.25]    (190.14,94) -- (209.19,101) ;
%Straight Lines [id:da32517246128382027] 
\draw [line width=2.25]    (192.14,107) -- (207.19,111) ;
%Straight Lines [id:da39391406285899655] 
\draw    (210.19,96) -- (205.18,116) ;
%Shape: Triangle [id:dp8041932555907878] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (218.83,101.59) -- (210.51,97.71) -- (209.65,101.11) -- cycle ;
%Shape: Triangle [id:dp2578698299103319] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (215.82,115.59) -- (207.5,111.71) -- (206.64,115.11) -- cycle ;

%Shape: Rectangle [id:dp1942699846225675] 
\draw  [fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=1 ] (446.74,133.54) -- (458.24,133.54) -- (458.24,143.54) -- (446.74,143.54) -- cycle ;
%Shape: Rectangle [id:dp6329804393445349] 
\draw  [fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=1 ] (451.24,123.54) -- (462.74,123.54) -- (462.74,133.54) -- (451.24,133.54) -- cycle ;
%Shape: Rectangle [id:dp6489484559599064] 
\draw  [fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=1 ] (458.24,133.54) -- (469.74,133.54) -- (469.74,143.54) -- (458.24,143.54) -- cycle ;
%Shape: Rectangle [id:dp15032900977810182] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (128.35,133) -- (116.43,133) -- (116.43,143) -- (128.35,143) -- cycle ;
%Shape: Rectangle [id:dp9604858708201851] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (116.43,133) -- (104.5,133) -- (104.5,143) -- (116.43,143) -- cycle ;
%Shape: Rectangle [id:dp4049648885597761] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (122.13,122) -- (110.2,122) -- (110.2,132) -- (122.13,132) -- cycle ;
%Shape: Rectangle [id:dp06896096651057149] 
\draw  [fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=1 ] (281.74,117.54) -- (293.24,117.54) -- (293.24,127.54) -- (281.74,127.54) -- cycle ;
%Left Arrow [id:dp8439528850056612] 
\draw   (247.5,107.5) -- (256.3,101) -- (256.3,104.25) -- (269.5,104.25) -- (269.5,110.75) -- (256.3,110.75) -- (256.3,114) -- cycle ;
%Left Arrow [id:dp2747854968621888] 
\draw   (328.49,107.16) -- (319.88,113.94) -- (319.79,110.67) -- (306.59,111.04) -- (306.41,104.52) -- (319.61,104.15) -- (319.51,100.88) -- cycle ;

% Text Node
\draw (405,157) node   [align=left] {$\displaystyle \mathsf{GRobot}$};
% Text Node
\draw (292,157) node   [align=left] {$\displaystyle \mathsf{Cart}$};
% Text Node
\draw (158,157) node   [align=left] {$\displaystyle \mathsf{RRobot}$};


\end{tikzpicture}



==> basic_example_msc.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-0.6,xscale=1]
%uncomment if require: \path (0,442); %set diagram left start at 0, and has height of 442

%Straight Lines [id:da1600470735495363] 
\draw [line width=2.25]    (200.97,24.47) -- (198.46,300) ;
\draw [shift={(198.42,304)}, rotate = 270.52] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=2.25]    (17.49,-5.26) .. controls (11.12,-2.23) and (5.29,-0.48) .. (0,0) .. controls (5.29,0.48) and (11.12,2.23) .. (17.49,5.26)   ;
%Straight Lines [id:da17654801632920147] 
\draw [line width=2.25]    (310.21,25.97) -- (307.69,298.49) ;
\draw [shift={(307.66,302.49)}, rotate = 270.53] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=2.25]    (17.49,-5.26) .. controls (11.12,-2.23) and (5.29,-0.48) .. (0,0) .. controls (5.29,0.48) and (11.12,2.23) .. (17.49,5.26)   ;
%Shape: Rectangle [id:dp04299445629443044] 
\draw  [fill={rgb, 255:red, 238; green, 10; blue, 10 }  ,fill opacity=1 ] (193.32,76.46) -- (205.57,76.46) -- (205.57,144.27) -- (193.32,144.27) -- cycle ;
%Shape: Rectangle [id:dp7915097130160935] 
\draw  [fill={rgb, 255:red, 184; green, 233; blue, 134 }  ,fill opacity=1 ] (205.57,154.82) -- (194.34,154.82) -- (194.34,206.8) -- (205.57,206.8) -- cycle ;
%Straight Lines [id:da27813177601484784] 
\draw [line width=2.25]    (403.11,25.22) -- (400.6,297.74) ;
\draw [shift={(400.56,301.74)}, rotate = 270.53] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=2.25]    (17.49,-5.26) .. controls (11.12,-2.23) and (5.29,-0.48) .. (0,0) .. controls (5.29,0.48) and (11.12,2.23) .. (17.49,5.26)   ;
%Shape: Rectangle [id:dp0824929773405314] 
\draw  [fill={rgb, 255:red, 30; green, 211; blue, 231 }  ,fill opacity=1 ] (315.82,78.72) -- (303.57,78.72) -- (303.57,145.77) -- (315.82,145.77) -- cycle ;
%Straight Lines [id:da10416962657650264] 
\draw    (200.46,51.59) -- (307.7,59.73) ;
\draw [shift={(309.7,59.88)}, rotate = 184.34] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da5615241369165318] 
\draw    (200.46,62.14) -- (402.65,77.06) ;
\draw [shift={(404.64,77.21)}, rotate = 184.22] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da765869767634296] 
\draw    (201.48,144.27) -- (308.73,152.4) ;
\draw [shift={(310.72,152.55)}, rotate = 184.34] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Rectangle [id:dp978596576487264] 
\draw  [fill={rgb, 255:red, 65; green, 117; blue, 5 }  ,fill opacity=1 ] (314.8,155.57) -- (303.57,155.57) -- (303.57,207.56) -- (314.8,207.56) -- cycle ;
%Straight Lines [id:da801291448443189] 
\draw    (309.7,209.06) -- (200.41,220.9) ;
\draw [shift={(198.42,221.12)}, rotate = 353.82] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Rectangle [id:dp6718200900343567] 
\draw  [fill={rgb, 255:red, 238; green, 10; blue, 10 }  ,fill opacity=1 ] (193.32,222.63) -- (205.57,222.63) -- (205.57,287.42) -- (193.32,287.42) -- cycle ;
%Shape: Rectangle [id:dp2915325089071221] 
\draw  [fill={rgb, 255:red, 30; green, 211; blue, 231 }  ,fill opacity=1 ] (312.76,221.87) -- (301.53,221.87) -- (301.53,286.67) -- (312.76,286.67) -- cycle ;
%Shape: Rectangle [id:dp7777787956405315] 
\draw  [fill={rgb, 255:red, 30; green, 211; blue, 231 }  ,fill opacity=1 ] (408.73,79.47) -- (395.45,79.47) -- (395.45,286.67) -- (408.73,286.67) -- cycle ;
%Straight Lines [id:da18044399025145985] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (153.5,76.46) -- (446.5,78.72) ;
%Straight Lines [id:da8233449212078279] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (153.5,144.27) -- (346.45,145.77) ;
%Straight Lines [id:da06710897658613546] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (154.52,206.05) -- (347.47,207.56) ;
%Straight Lines [id:da5445207548180246] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (159.63,286.67) -- (426.08,287.42) ;

% Text Node
\draw (201.99,12.41) node  [font=\large] [align=left] {Cart};
% Text Node
\draw (401.07,13.16) node  [font=\large] [align=left] {RRobot};
% Text Node
\draw (260.31,43.58) node  [font=\large] [align=left] {$\displaystyle \mathit{arrive}$};
% Text Node
\draw (311.23,12.41) node  [font=\large] [align=left] {GRobot};
% Text Node
\draw (355.28,61.15) node  [font=\large] [align=left] {$\displaystyle \mathit{free}$};
% Text Node
\draw (259.18,160.32) node  [font=\large] [align=left] {$\displaystyle \mathit{ready}$};
% Text Node
\draw (257.25,223.8) node  [font=\large] [align=left] {$\displaystyle \mathit{ok}$};
% Text Node
\draw (358.41,154.02) node [anchor=north west][inner sep=0.75pt]  [font=\Huge] [align=left] {*};
% Text Node
\draw (202,127) node [anchor=north west][inner sep=0.75pt]  [font=\large] [align=left] {$\displaystyle {\displaystyle \rightsquigarrow }$};
% Text Node
\draw (202,269) node [anchor=north west][inner sep=0.75pt]  [font=\large] [align=left] {$\displaystyle \rightsquigarrow $};
% Text Node
\draw (286,189) node [anchor=north west][inner sep=0.75pt]  [font=\large] [align=left] {$\displaystyle \leftsquigarrow $};


\end{tikzpicture}


==> calculus.tex <==
\section{Multiparty Motion Session Calculus}
\label{sec:calculus}
We now describe the motion session calculus, extending from \cite{ECOOP19}.
%% In concurrent robotics programming, the number of participants (robotic components) is fixed.  
%% Hence our motion session calculus follows the calculi in \cite{DGJPY2016,GHPSY19,ECOOP19},
%% which simplifies the synchronous multiparty session calculus in \cite{KY13} by eliminating both shared channels
%% for session initiations and session channels for communications inside sessions.

%% \begin{notation}[Base sets]
%%   \label{notation:sets}
%% \RMi{omit or update}
%%   We use the following base sets:
%%   \emph{values}, ranged over by $\val,\val',\ldots$;
%%   \emph{expressions}, ranged over by $\e,\e',\ldots$;
%%   \emph{expression variables}, ranged over by $x,y,z\dots$;
%%   \emph{labels}, ranged over by $\ell,\ell',\dots$;
%%   \emph{session participants}, ranged over by $\pp,\pq,\ldots$;
%%   \emph{motion primitives}, ranged over by \ma, \mb, $\ldots$;
%%   \emph{process variables}, ranged over by $X,Y,\dots$;
%% \RM{to fix}
%%   \emph{processes}, ranged over by $P,Q,\dots$; and %
%%   \emph{multiparty sessions}, ranged over by $\N,\N',\dots$.
%% \end{notation}

\subsection{Syntax} 
\myparagraph{Physical Components and Processes}
%
We assume a fixed static set $\PC$
of \emph{physical components} (ranged over by $\pp$, $\q$,...), which
are often called \emph{participants} or \emph{roles};
these are the different components that constitute the overall system.
Each physical component executes a software process, which 
takes care of communication, synchronisation and motion.
We describe the motion session calculus, which forms the core of the software process.

A value $\val$ can be a natural number $\valn$, an integer $\valr$, a boolean $\true$/$\false$, or a real number. %
An expression $\e$ can be a variable, a value, or a term built from expressions by applying (type-correct) computable operators.
A \emph{motion primitive} (\ma, \mb, $\ldots$) is an abstraction of underlying physical trajectories; for the moment,
consider a motion primitive simply as a name and describe its semantics later.
We use the notation $\motion{dt}{\ma}$ to represent that a motion primitive executes and time elapses.
We write the tuple $\motion{dt}{(\pp_i: \ma_i)}$ to denote a group of processes executing their respective motion primitives at the same time.
For the sake of simplicity, we sometimes use $\ma$ for both single or grouped motions.

The \emph{processes} ($\PP,Q,R,...$) of the multiparty motion session calculus are defined by:
\[
\begin{array}{lll}\PP   ::=  \procout {\pp}{\ell}{\e}{\PP} 
            \SEP \sum\limits_{i\in I}
            \procin{\pp}{\ell_i(x_i)}{\PP_i} \SEP \cond{\e}\PP \PP %\\[1mm]
            %& \SEP  &
            \SEP
             \sum\limits_{i\in I}
            \procin{\pp}{\ell_i(x_i)}{\PP_i}+\motion{dt}{a}.{\PP}
            \SEP
            \motion{dt}{\ma}.\PP \SEP \mu\procvar.\PP \SEP \procvar % \SEP \inact 
\end{array}
\]
The output process $\procout{\pp}{\ell}{\e}{\Q}$ sends the value of expression $\e$ with label $\ell$ to participant $\pp$.
The sum of input processes (external choice) 
$\sum_{i\in I}\procin{\pp}{\ell_i(x_i)}{\PP_i}$ is a process that can accept a value
with label $ \ell_i $ from participant $ \pp$ for any $ i\in I$; 
$\sum_{i\in I}\procin{\pp}{\ell_i(x_i)}{\PP_i}+\motion{dt}{a}.{\PP}$
is an external choice with a \emph{default branch} with a motion action $\motion{dt}{a}.{\PP}$ which can always proceed when there is no message to receive.
According to the label $\ell_i$ of the received value, the variable $x_i$
is instantiated with the value in the continuation process $ \PP_i$. 
We assume that the set $I$ is always finite and non-empty. 
Motion primitives are indicated by $\motion{dt}{\ma}$; the $\kf{dt}$ denoting
that real time progresses when a motion primitive $\ma$ is executed.
The conditional process $\cond{\e}{\PP}{Q} $ represents the internal choice between processes $ \PP $ and $ \Q $. 
Which branch of the conditional process will be taken depends on the evaluation of the expression $ \e. $ 
The process $\mu \procvar.\PP$ is a recursive process.  
%% We assume that the recursive processes are \emph{guarded}. For example, $\mu \procvar.\procin\pp{\ell(\x)}\procvar$ is a valid process, while $\mu \procvar.\procvar$ is not.
% We often omit $\inact$ from the tail of processes.
Note that our processes do not have a null process: this is because a physical component does not ``disappear'' when the program stops.
Instead, we model inaction with an iteration of some default motion primitive.

\begin{example}[Processes]\rm
The processes for the cart 
and the two robots from Figure~\ref{fig:basic_example_fig} are given as:
\[
\begin{array}{cc}
\begin{array}{rl}\small
\Cart:\!\!\!\!\!\!\!\!\!\!\!\!\\  
\mu \procvar.\!\!\!\!\!\!
& (\Green!\ARRIVE.\Red!\FREE.\\
& \quad \motion{dt}{\MOVEM(\text{co-ord of }\Green)}.\Green!\READY.\\
&  \quad \motion{dt}{\IDLEM}.\Green?\OK.\motion{dt}{\MOVEM(\text{base})}.\procvar\\
& + \textrm{ symmetrically for $\Red$ })
\end{array}
&
\!\!\!\!\!\!\!\!
\begin{array}{rl}
\small
\Red,\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\\\
\Green:\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\\
\mu \procvar.\!\!\!\!\!\!& 
(\Cart?\ARRIVE.\motion{dt}{\WORKM}.\Cart?\READY.\\
& \quad \ \motion{dt}{\PICKM}.\Cart!\OK.\motion{dt}{\WORKM}).\procvar\\
& \ + \ (\Cart?\FREE.\motion{dt}{\WORKM}).\procvar\\
\end{array}
\end{array}
\]
%% As usual, we write
%% $\pp!\ell$ for \textbf{\emph{sending}} a message $\ell$ to a process $\pp$ 
%% and
%% $\pp?\ell$ for \textbf{\emph{receiving}} a message $\ell$ from $\pp$, respectively.
%% The $+$ denotes \textbf{\emph{choice}} and the $\mu$ operator denotes a \textbf{\emph{recursion}}.
%
Note that for both processes, the recursion ensures that the program does not terminate.
Motion primitives for the cart involve moving to various locations $\MOVEM(\mathit{pos})$
and idling at a location ($\IDLEM$), and those for the robots involve doing some (unspecified)
work $\WORKM$ or picking items off the cart $\PICKM$
(internally, these motion primitives would involve motion planning and inverse kinematics for the robot arms).
Next, we describe the modelling and representation of motion primitives in more detail.
\end{example}

\myparagraph{Physical Variables and Footprint}
%
Motion primitives make the robot ``move'' in the physical world.
Each motion primitive represents an abstraction of an underlying controlled dynamical
system, such as the controller for the robot arm or the controller for a cart.
The dynamical system changes underlying physical state (such as the position and orientation of the arm
or the position and velocity of the cart).
The dynamics can be coupled: for example, if an arm is mounted on a cart, then the motion of the cart
is influenced by the mass and position of the arm.

We model the underlying physical system using \emph{physical variables}, and we partition these
into state variables $X$ (dynamical variables read and controlled by the component),
input variables $W$ (dynamical variables read by the component, whose values are provided by the environment).
The specification of a motion primitive will constrain the values of these variables over time.
We make the physical variables clear by writing $\pc \plays\proc{\PP}{{X}}{{W}}$ for a 
physical component $\pc\in \PC$ with state and input
variables $X$ and $W$, respectively, which executes the process $\PP$.

Each physical component $\pc\in \PC$ has a \emph{geometric footprint} $\geom{\pc}$ associated
with it.
This represents the physical space occupied by the component, and will be used to ensure that two
components do not collide.
The footprint is a function from valuations to variables in $X$ to a subset of $ℝ^3$.
It describes
% , in the reference frame of the component, 
an overapproximation of the space
occupied by the component as a function of the current state.
Note that the footprint can depend on the state.
% For example, the footprint of the crane when the cable is retracted is simply a bounding box
% around the winch, but includes the geometric space occupied by the cable when it is unbound.

\begin{example}\rm
\label{ex:mp-footprint}
Let $x$ and $v$ denote the position and the velocity of the cart, respectively, restricting
the discussion only on one axis.
Thus, $X = \set{x, v}$. If we assume there are no external influences on the cart, we can
take $W = \emptyset$.
The footprint provides a bounding box around the cart as it moves.
If the cart has dimensions $(l, w, h)$, the footprint at the location $(x, y, z)$ is 
\begin{align}
\set{(\mathsf{x}, \mathsf{y}, \mathsf{z}) \mid 
% \begin{array}{c}
x-\frac{l}{2} \leq \mathsf{x} \leq x+\frac{l}{2} \wedge 
0\leq \mathsf{y} \leq h 
\wedge z -\frac{w}{2} \leq \mathsf{z} \leq z+\frac{w}{2}
% \end{array}
}
\end{align} 
\end{example}

\myparagraph{Composition}
We now define parallel composition of physical components.
Composition of physical components ensure the following aspects.
First, like process calculi, parallel composition provides a locus for message
exchange: a physical component can send messages to, or receive messages from, another one.
Second, composition connects physical state variables of one component to the physical input variables
of another---this enables the coupling of the underlying dynamics.
% Finally, composition of physical components corresponds to physical attachments in the world.
% Thus, geometric entities communicated between two components may require a relative frame shift to be interpreted
% correctly, and the composition operation must specify the frame shift.

To ease reasoning about connections between physical variables,
we assume that the components in a composition have disjoint sets of physical and
logical variables, and connections occur through syntactic naming of input variables.
Thus, a component with an input variable $x$ gets its value from the unique component that has a physical
state variable called $x$. 
Hence, there is no ambiguity in forming connections.
We refer to the variables of $\pc$ as $\pc.X$ and $\pc.W$.
%% $\pc.V$.

We define a \emph{multiparty session} as a parallel composition of pairs of participants and processes:
\[ 
\begin{array}{lll}
   \N  &  ::=   & \pp\plays\proc{\PP}{X}{W}  \SEP \N \parcomp \N
 \end{array}
\]
with the intuition that process $\PP$ plays the role of participant $\pp$, %
and can interact with other processes playing other roles in $M$. %
A multiparty session is \emph{well-formed} if all its participants are different, 
and for each input variable of each participant there is a syntactically unique
state variable in a different participant so that connections between physical variables is well-defined.
We consider only well-formed processes. 

\begin{example}\rm
For the example from \Sec~\ref{sec:example}, the multiparty session is
\[
\Cart\plays\proc{\text{proc.\ for $\Cart$}}{\set{x,v}}{\emptyset} \parcomp
\Red \plays\proc{\text{proc.\ for $\Red$}}{\cdot}{\cdot} \parcomp
\Green \plays\proc{\text{proc.\ for $\Green$}}{\cdot}{\cdot} 
\]
(we have omitted the physical variables for the robot arms for simplicity).
\end{example}

 




\subsection{Motion Primitives}
\label{sec:mp-rules}

Before providing the operational semantics, we first
consider how motion primitives 
are specified. 
Recall that motion primitives of a component $\pc\plays\proc{\PP}{X}{W}$
abstract a trajectory arising out of the underlying dynamics. 
A first idea is to represent a motion primitive as a pair 
$\tuple{\pre, \post}$---this provides a precondition $\pre$ that specifies 
the condition on the state under which the 
motion primitive can be applied and 
a postcondition $\post$ that specifies the effect of applying the
motion primitive on the physical state. 
However, this is not sufficient: the motion of two components can be coupled in time and the  
trajectory of a component depends on the inputs it gets from other components 
and, in turn, its trajectory influences the trajectories of the other components. 
Therefore, a motion primitive also needs to specify \emph{assumptions} on its external inputs and 
\emph{guarantees} it provides to other processes over time.
These predicates are used to decouple the dynamics. 

Our motion primitive has three more ingredients. 
The first is the \emph{footprint}:
the geometric space used by a process over time while it executes its trajectory and is used 
to ensure geometric separation between components. 
The second is a pair $(D, \timestep)$ of a \emph{time interval and an annotation}: the time interval 
bounds the \emph{minimal} and \emph{maximal times} between which a motion primitive is ready to communicate 
via message passing, and the 
$\timestep$ annotation distinguishes between motion primitives
that are interruptible by external messages 
from those that cannot be interrupted. 

We assume preconditions and postconditions only depend on the state, while assumptions, guarantees,
and footprints may depend on both the state and the elapsed time. 
% Accordingly, we represent pre- and post-conditions using first order logic formulas over $X\cup W$,
% assumptions as formulas over $W\cup\set{\clock}$ and guarantees as formulas over $X\cup\set{\clock}$, 
% where $\clock$ is a new variable denoting elapsed time (from the start of the execution of the motion primitive). 
% Finally, a footprint is represented as a predicate over $X$ and the 
% formal variables $\set{\mathsf{x}, \mathsf{y}, \mathsf{z}, \clock}$
% representing the three spatial coordinates for the reference frame and elapsed time. 

\begin{definition}[Motion primitive]
The specification for a motion primitive $\ma$ of a physical process $\pc\plays\proc{\PP}{X}{W}$,
written 
$\judgement{\ma}{\pre,A,G,\post,\FP,D, \timestep}$,
consists of 
two predicates \emph{precondition} $\pre$ and \emph{postcondition} $\post$ over $X\cup W$, 
an \emph{input assumption} $A$ which is a predicate over $W\cup\set{\clock}$, 
an \emph{output guarantee} $G$ which is a predicate over $X\cup\set{\clock}$, 
a \emph{footprint} $\FP$ which is a predicate over $X \cup \set{\mathsf{x},\mathsf{y},\mathsf{z},\clock}$,
a \emph{duration} $D\in (ℝ\cup\set{\infty})^2$ which is a time interval,
and 
$\timestep\in\set{\instantaneous,\delayed}$ which indicates if the motion primitive can be interrupted 
by an external message ($\instantaneous$) or not ($\delayed$). 

Given motion primitives $\ma$ and $\ma'$, we say $\ma$ \emph{refines} $\ma'$, denoted by 
$\ma \refines \ma'$,  
with $\judgement{\ma}{φ,A,G,ψ,\FP, D, \timestep}$  
and $\judgement{\ma'}{φ',A',G',ψ',\FP', D', \timestep'}$
iff 
(1) $φ ⇒ φ'$,
(2) $A ⇒ A'$,
(3) $G' ⇒ G$,
(4) $ψ' ⇒ ψ$, 
(5) $\FP' ⊆ \FP$, 
(6) $\timestep = \timestep'$, and
(7) either $\timestep =\instantaneous$ and $D⊆ D'$ or
$\timestep=\delayed$ and $D' ⊆ D$. 
\end{definition}

% A motion primitive is \emph{well-formed} iff 
% (1) $\pre$, $A$, $\post$, $G$ are all satisfiable,
% and 
% (2) $\pre \wedge A\{0/\clock\} \Rightarrow G\{0/\clock\}$ 
% and for all $\forall t \in [0, \infty)$ we have $\post \wedge A\{t/\clock\} \Rightarrow G\{t/\clock\}$. 
% We assume all motion primitives are well-formed.

\subsection{Operational Semantics}
\label{sec:opsem}
The operational semantics is given as reduction rules relative to \emph{stores} $\sstore{X},\sstore{W}$
(Figure~\ref{fig:opsem})
that map physical variables to values. 
The semantics uses the standard structural rules defined
in Figure~\ref{tab:sync:congr}. 
% Since the physical variables only occur in the rules for motion, we omit writing them in rules for communication. 

We adopt some standard conventions regarding the syntax of processes and sessions. 
Namely, we  will use 
$\prod_{i\in I} {\pp_i}\plays\proc{\PP_i}{X_i}{W_i}$ for ${\pp_1}\plays\proc{\PP_1}{X_1}{W_1}\parcomp \ldots\parcomp {\pp_n}\plays\proc{\PP_n}{X_n}{W_n},$ 
where $I=\set{1,\ldots,n}$, or simply as $\prod_{i\in I} \pa{\pp_i}{\PP_i}$ when the physical variables are not important. %\DZ{I tried to limit the use of the 2nd form} 
We use infix notation for external choice process, 
e.g., instead of $\sum_{i\in \{1,2\}}
\procin{\pp}{\ell_i(\x)}{\PP_i}$, we write 
$\procin{\pp}{\ell_1(\x)}{\PP_1}+\procin{\pp}{\ell_2(\x)}{\PP_2}.$
{\em The value $\val$ of expression $\e$ with physical state $\sstore{X}$} (notation $\evalState{\e}{\val}{\sstore{X}}$) is computed as expected. 
We assume that $\evalState{\e}{\val}{\sstore{X}}$ is effectively computable and takes logical ``zero time.'' 


%(see Appendix \ref{app:calculus} for the full rules).  
\begin{figure}[!t]
  \label{tab:sync:red}
\small
\[
\begin{array}[t]{@{}c@{}}
\rulename{recv}\inferrule%[\rulename{recv}]
{
j\in I 
}
{
\pp\plays\proc{\sum\limits_{i\in I} \procin{\q}{\ell_i(\x)}{\PP_i} + \motion{dt}{a}.{\PP} }{\sstore{X}}{\sstore{W}}
\xrightarrow{\q?\ell_j(v)}
\pp\plays\proc{\PP_j\set{v/x}}{\sstore{X}}{\sstore{W}}
}
\\[5mm]
\rulename{send}
\inferrule%[\rulename{send}]
          {
            \evalState{\e}{\val}{\sstore{X},\sstore{W}}
}{
\pp\plays\proc{\procout{\q}{\ell_j}{\e}{Q}}{\sstore{X}}{\sstore{W}}
\xrightarrow{\q!\ell\tuple{\val}}
\pp\plays\proc{Q}{\sstore{X}}{\sstore{W}}
}
          \quad
          \rulename{comm}
          \inferrule%[\rulename{comm}]
{
\pa\pp{\PP} \xrightarrow{\q!\ell\tuple{\val}} \pa\pp{\PP'}\\
\pa\q{\Q} \xrightarrow{\pp?\ell(\val)} \pa\q{\Q'}\\
}
{
  \pa\pp{\PP} \parcomp \pa\q{\Q} %\parcomp \N
  \red{} \pa\pp{\PP'} \parcomp \pa\q{\Q'} %\parcomp \N
}
\\[6mm]
\inferrule[\rulename{default}]
{
\pp\plays \proc{\motion{\dtsess}{\ma}.\PP}{\sstore{X}}{\sstore{W}} \xrightarrow{\tau}
\pp\plays \proc{\motion{\dtsess}{\ma\AT 0}.\PP}{\sstore{X}}{\sstore{W}} \\
\pp\plays \proc{\motion{\dtsess}{\ma\AT 0}.\PP}{\sstore{X}}{\sstore{W}} \xrightarrow{\motion{\dtsess}{\ma},\xi,\nu, t} 
\pp\plays \proc{\motion{\dtsess}{\ma\AT t}.\PP}{\sstore{X}'}{\sstore{W}'}
} 
{
\pp\plays \proc{\sum\limits_{i\in I} \procin{\q}{\ell_i(\x)}{\PP_i} + \motion{\dtsess}{a}.{\PP}}{\sstore{X}}{\sstore{W}}
\xrightarrow{\motion{\dtsess}{\ma},\xi,\nu, t} 
\pp\plays \proc{\motion{\dtsess}{\ma\AT t}.\PP}{\sstore{X}'}{\sstore{W}'}
 }
\\[5mm]
\inferrule[\rulename{traj-base}]
          {
\pre\{\sstore{X}/X,\sstore{W}/W, 0/\clock\}\quad 
A\{\sstore{W}/W, 0/\clock\}\wedge G\{\sstore{X}/X, 0/\clock\} \\
\geom{\pp}(\sstore{X})\subseteq\FP\set{\sstore{X}/X,0/\clock}
}
{
\pp\plays \proc{\motion{\dtsess}{\ma}.\PP}{\sstore{X}}{\sstore{W}} \xrightarrow{\tau}
\pp\plays \proc{\motion{\dtsess}{\ma\AT 0}.\PP}{\sstore{X}}{\sstore{W}}
}
\\[5mm]
\rulename{traj-step}
\inferrule%[\rulename{traj-step}]
          {
  \xi: [t_1,t_2] \rightarrow ℝ^X, \nu: [t_1,t_2] \rightarrow ℝ^W\\
  \xi(t_1) = \sstore{X}, \xi(t_2) = \sstore{X}' \\
  \nu(t_1) = \sstore{W}, \nu(t_2) = \sstore{W}' \\
  \forall t\in [t_1,t_2].\ A\{\nu(t)/W, t/\clock\} \wedge G\{\xi(t)/X, t/\clock\}
\ \wedge \geom{\pp}(\xi(t))\subseteq\FP\set{\sstore{X}/X,t/\clock}
}
{
\pp\plays \proc{\motion{\dtsess}{\ma\AT t_1}.P}{\sstore{X}}{\sstore{W}} \xrightarrow{\motion{\dtsess}{\ma},\xi,\nu, t_2-t_1} 
\pp\plays \proc{\motion{\dtsess}{\ma\AT t_2}.P}{\sstore{X}'}{\sstore{W}'}
}
\\[7mm]
\inferrule[\rulename{t-conditional}]
{
  \evalState{\e}{\true}{\sstore{X},\sstore{W}}
}
{
\pp\plays\proc{\cond{\e}{\PP}{\Q}}{\sstore{X}}{\sstore{W}}
\xrightarrow{}
\pp\plays\proc{\PP}{\sstore{X}}{\sstore{W}}
}
\quad 
\inferrule[\rulename{non-interrupt}]
{
t \in D\\ 
\timestep = \delayed\\
\post\set{\sstore{X}/X,\sstore{W}/W,t/\clock}\\
}
{
\pp\plays \proc{\motion{\dtsess}{\ma\AT t}.\PP}{\sstore{X}}{\sstore{W}} \xrightarrow{\tau} \pp\plays \proc{\PP}{\sstore{X}}{\sstore{W}}
}
\\[5mm]
\rulename{interrupt}
\inferrule%[\rulename{interrupt}]
    {
t \in D\\ 
\timestep = \instantaneous\\
\post\set{\sstore{X}/X,\sstore{W}/W,t/\clock}\\
\pp\plays \proc{\PP}{\sstore{X}}{\sstore{W}} \xrightarrow{\q?\ell(\val)} \pp\plays \proc{\PP'}{\sstore{X}}{\sstore{W}}
}
{
\pp\plays \proc{\motion{\dtsess}{\ma\AT t}.\PP}{\sstore{X}}{\sstore{W}}
\xrightarrow{\q?\ell(\val)} 
\pp\plays \proc{\PP'}{\sstore{X}}{\sstore{W}}
}
\\[5mm]
\rulename{m-par}
\inferrule%[\rulename{m-par}]
    {
\exists \xi, \nu.~ \forall i,j \in I.\\
  i\neq j \Rightarrow \mathsf{disjoint}(\ma_i,\ma_j) \\
  \pp_i\plays\proc{P_i}{\sstore{X}_i}{\sstore{W}_i}
    \xrightarrow{\motion{\dtsess}{\ma_i},\xi|_{X_i}, (\xi\cup\nu)|_{W_i}, t}
    \pp_i\plays\proc{P_i'}{\sstore{X}'_i}{\sstore{W}'_i}\\
}
{
  \prod_{i \in I} \pp_i\plays\proc{P_i}{\sstore{X}_i}{\sstore{W}_i} 
  \xrightarrow{\motion{\dtsess}{\ma_i}, t}
  \prod_{i \in I} \pp_i\plays\proc{P_i'}{\sstore{X}'_i}{\sstore{W}'_i}
}
\\[6mm]
%% \quad 
%% \inferrule[\rulename{f-conditional}]{
%%   \evalState{\e}{\false}{\sstore{X},\sstore{W}}
%% }
%% {
%% \pp\plays\proc{\cond{\e}{\PP}{\Q}}{\sstore{X}}{\sstore{W}}
%% \xrightarrow{}
%% \pp\plays\proc{\Q}{\sstore{X}}{\sstore{W}}
%% }
%\\[5mm]
\rulename{r-par$\tau$}
\inferrule%[\rulename{r-par$\tau$}]
    {
%\pa\pp\proc{\Q}{\sstore{X}}{\sstore{W}}
\N_1
\xrightarrow{\tau}
\N_2
%\pa\pp\proc{\Q'}{\sstore{X}'}{\sstore{W}'}
}
{
%\pa\pp\proc{\Q}{\sstore{X}}{\sstore{W}}
\N_1
\parcomp \N \xrightarrow{\tau}
\N_2
%\pa\pp\proc{\Q'}{\sstore{X}'}{\sstore{W}'}
\parcomp \N 
}
\qquad
\rulename{r-par}
\inferrule%[\rulename{r-par}]
          {
%\pa\pp\proc{\Q}{\sstore{X}}{\sstore{W}}
\N_1
\red{}
\N_2
%\pa\pp\proc{\Q'}{\sstore{X}'}{\sstore{W}'}
}
{
%\pa\pp\proc{\Q}{\sstore{X}}{\sstore{W}}
\N_1
\parcomp \N \red{}
\N_2
%\pa\pp\proc{\Q'}{\sstore{X}'}{\sstore{W}'}
\parcomp \N 
}
\qquad
\rulename{r-struct}
\inferrule%[\rulename{r-struct}]
{
  \N'_1\equiv \N_1 \xrightarrow{\alpha} \N_2 \equiv \N'_2 
}
{ 
  \N'_1 \xrightarrow{\alpha} \N'_2 
}
\end{array}
\]
%% \DZi{summary of changes:
%% updates \rulename{interrupt},
%% added $\tau$ labels,
%% added $\motion{\dtsess}{\ma}$ to all motion labels,
%% refactored notation to use $\proc{\PP}{\sstore{X}}{\sstore{W}}$ more uniformly,
%% evalation of expression can read from physical state,
%% added frame to \rulename{comm}
%% }
\noindent
We omit \rulename{f-conditional}. 
We use $\xrightarrow{\alpha}$ for 
any labelled transition relation or reduction ($\xrightarrow{}$). 
\caption{Operational semantics}
\label{fig:opsem}
\vspace*{-0.5cm}
\end{figure}
\begin{figure}{}
$
\small
\begin{array}[t]{@{}c@{}}
  \inferrule[\rulename{s-rec}]{}{ \mu \procvar.\PP \equiv \PP\sub{\mu \procvar.\PP}{\procvar} }
\quad
\inferrule[\rulename{s-multi}]{}{
	\PP \equiv \Q  \Rightarrow \pa\pp\PP \ | \  M\equiv\pa\pp\Q \ | \ M
} \quad 
\inferrule[\rulename{s-par 1}]{}{
	M \ | \ M' \equiv M' \ | \  M
}
\quad      
\inferrule[\rulename{s-par 2}]{}{
	(M \ | \ M') \ | \ M'' \equiv M \ | \ ( M' \ | \  M'')
} 
\end{array}
$
\caption{Structural congruence rules}
\label{tab:sync:congr}
\vspace*{-0.5cm}
\end{figure}

%given in Table~\ref{tab:sync:red}.
% In rule \rulename{comm}, the participant $\q$ sends the value $\val$ choosing the label $\ell_j$ to participant $\pp$, 
% who offers inputs on all labels $\ell_i$ with $i\in I$; and
For reduction rules that do not change the physical state, we omit writing the physical state in the rule.
Time is global, and processes synchronize in time to make concurrent
motion steps of the same (but not pre-determined) duration.
Communication (\rulename{comm}) is synchronous and puts together sends and receives.
Rule \rulename{default} selects the default branch.
Rules for conditionals, communication without default motion  
and parallel composition 
are defined in a standard way \cite{ECOOP19,DGJPY2016,GHPSY19}.



%% \NYi{I found several problems in the operational semsntics. I need your input.
%%   }
%% \begin{enumerate}
%% \item Default has a problem. We need to put some label such as ``start''
%%   Similarly [TRAJ-BASE] should have ``start'' 
%% \item Non-inerrupt or Interrupt is the termination rules to go next stage.
%%   To match [M-Par], we need to put dt<a>, xi, v, t but not sure where they can come from except dt<a>.
%% \item Interrupt needs to be changed: 
%%   \begin{enumerate}
%%   \item
%%  $\motion{\dtsess}{\ma\AT t}.Q + \sum\limits_{i\in I}\procin{\pp}{\ell_i(x_i)}{\PP_i}$ or
%%   \item
%%     $\motion{\dtsess}{\ma\AT t}.P$ with the assumption. 
%% \end{enumerate}    
  
%% \item M-Par  we need $dt<(a_i:p_i)>$ in the conclusion.
%% \end{enumerate}


%% In rules \rulename{t-conditional} and \rulename{f-conditional}, the  participant $\pp$ chooses to continue as $\PP$ 
%% if the condition $\e$ evaluates to $\true$ and as $\Q$ if $\e$ evaluates to $\false$.  
%% Rule \rulename{r-struct} states that the reduction relation is closed
%% with respect to  structural congruence.
%% The rules are closed with respect to structural congruence $\equiv$.  
%% The structural congruence includes a recursion rule 
%% $\mu \procvar.\PP \equiv \PP\sub{\mu \procvar.\PP}{\procvar}$, as well as 
%% expected rules for multiparty sessions such as   
%% $\PP \equiv \Q  \Rightarrow \pa\pp\PP\parcomp\N\equiv\pa\pp\Q\parcomp\N$.   
%% Other rules are standard from \cite{DGJPY2016,GHPSY19}. 
%% However, unlike the usual treatment of $\pi$-calculi, 
%% our structural congruence does not have 
%% a rule to simplify inactive processes ($\pa\pp{\inact}$). 
%% The reason is that even when a program might be logically terminated, 
%% the physical robot continues to exist and may still collide with another robot. 
%% Therefore, in our model, all processes need to terminate at the 
%% same time, and so we need to keep $\pa\pp{\inact}$. 

To define the operational semantics for motions, we extend the process
syntax $P$ with time-annotated motion primitives, 
%\PP ::= \ldots \SEP
$\motion{dt}{\ma\AT t}\quad \text{ for }t\geq 0$. 
%\]
Let us fix a component $\pp$ and its motion primitive
$\judgement{\ma}{\pre,A,G,\post,\FP,D,\timestep}$.
Rules \rulename{traj-base} and \rulename{traj-step} set up trajectories for each motion primitive.
We distinguish between interruptible (\rulename{interrupt}) and non-interruptible (\rulename{non-interrupt})
motion primitives.
Non-interruptible motion primitives are consumed by the process.
Interruptible motion primitives consume the motion primitive on a message receipt.
The parallel composition rule \rulename{m-par} requires a consistent global trajectory and
ensures that when (physical) time elapses for one process, it elapses equally for all processes. 
Here, $\mathsf{disjoint}(\ma_i, \ma_j)$ states that the footprints along the trajectory are disjoint: 
    $\ma_i.\FP\set{\xi_i(t')/X,t'/\clock}\cap\ma_j.\FP\set{\xi_j(t')/X,t'/\clock}=\emptyset$ for all $t'\in[0,t]$.
%This style of synchronisation is reminiscent of broadcast calculi~\cite{DBLP:journals/scp/Prasad95}. 
%Instead of broadcast messages, we broadcast \emph{time}. 

We use $\red^*$ for the reflexive transitive closure of $\red$.
We say a program state $\prod_i \pp_i \plays\proc{\PP_i}{\sstore{X}_i}{\sstore{W}_i}$ is
\emph{collision free} if $\geom{\pp_i}(\sstore{X}_i)\cap\geom{\pp_j}(\sstore{X}_j) = \emptyset$
for every $i\neq j$.



\subsection{Joint Compatibility of Motion Primitives}
Two motion primitives are \emph{compatible} if they can be jointly executed.
To decide compatibility, we compose the specifications using the following
\emph{assume-guarantee proof rule}:\\
\centerline{
$
\small
\begin{array}{ll}
  \begin{array}{ll}
    \rulename{AGcomp}\\\\\\\\\
          \end{array}
    &
\inferrule{
\exists \FP_1, \FP_2.\
G_1 \wedge G_2 \Rightarrow \FP_1 \cap FP_2 = \emptyset\quad
G_1 \wedge G_2 \Rightarrow \FP_1 \cup FP_2 \subseteq \FP\\\\
 \timestep_1 =\instantaneous \vee \timestep_2 = \instantaneous \quad
 \timestep_1 =\delayed ⇒ D₁ ⊆ D₂ \quad
 \timestep_2 =\delayed ⇒ D₂ ⊆ D₁ \\\\
 \ma_1 \refines \tuple{φ₁,A∧ G₂,G₁,\FP_1,ψ₁,D_1,\timestep_1}\quad 
 \ma_2 \refines \tuple{φ₂,A∧ G₁,G₂,\FP_2,ψ₂,D_2,\timestep_2} 
}
          {\hspace*{-2mm}\judgement{\tuple{\pp_1{:}\ma_1, \pp_2{:}\ma_2}}{φ₁∧φ₂,A,G₁∧G₂,\FP,ψ₁∧ψ₂,D₁∩D₂,\timestep_1\oplus\timestep_2}}
          \end{array}
$}%

\noindent The $\oplus$ operator combines the interruptibility: 
$\instantaneous \oplus \instantaneous = \instantaneous$ and
$\instantaneous \oplus \delayed = \delayed \oplus \instantaneous = \delayed \oplus\delayed = \delayed$.

The \rulename{AGcomp} rule performs three checks.
First, the check on footprints ensures that the motion primitives are disjoint in space
(there is a way to find subsets $\FP_1$ and $\FP_2$ of the footprint $\FP$ so that the composed
motion primitives are in these disjoint portions).
Second, the guarantee of one motion primitive is used as the assumption of the other to check
that they are compatible.
Third, the checks on timing ensures that 
at most one process executes a non-interruptible motion primitive and 
the interruptible ones are ready before the non-interruptible one. 

We say 
$\motion{\dtsess}{(\pp_i {:} \ma_i)}$ is \emph{compatible} from $\pre$ if
there exist $G$, $\post$, $\FP$, and $D$ such that $\judgement{\prod_i{\pp_i:\ma_i}}{\pre, \true, G, \post, \FP, D, \timestep}$ is derivable
using \rulename{AGcomp} repeatedly.
Thus, compatibility checks that motion primitive specifications can be put together if 
processes start from their preconditions:
first, the assumptions and guarantees are compatible; 
second, there is no ``leftover'' assumption;
and
third, the footprints of the motion primitives do not intersect in space. 
Compatibility provides the ``converse'' condition that allows joint
trajectories in \rulename{M-par} to exist.

The next theorem formalizes what motion compatibility guarantees.
Intuitively, motion compatibility means it is sufficient to check the compatibility of contracts
to guarantee the existence of a joint trajectory, i.e., the execution is defined for all the components
and the joint trajectory satisfies the composition of the contracts.

\begin{restatable}[Motion Compatibility]{theorem}{theoremMC}
\label{th:motion-compat}
Suppose $\motion{\dtsess}{(\pp_1:\ma_1,\pp_2:\ma_2)}$ is compatible.
For every $t\in D$, if there exist trajectories $\xi_1, \xi_2,\nu_1,\nu_2$ such that
$\pa{\pp_i}{\PP_i} \xrightarrow{\motion{\dtsess}{\ma_i},\xi_i, \nu_i, t} \pa{\pp_i}{\PP_i'}$
for $i\in \set{1,2}$, then there exist trajectories
$\xi:[0,t]\rightarrow  ℝ^{X_1\cup X_2},
\nu:[0,t]\rightarrow ℝ^{W_1\cup W_2 \setminus (X_1\cup X_2)}$
such that
$\pa{\pp_i}{\PP_i} \xrightarrow{\motion{\dtsess}{\ma_i},\xi|_{X_i}, \nu|_{W_i}, t} \pa{\pp_i}{\PP_i'}$
and for all $0 \leq t' \leq t$, 
the footprints of $\pp_1$ and $\pp_2$ are disjoint:
$\geom{\pp_1}({\xi(t')|_{X_1}}) \cap \geom{\pp_2}({\xi(t')|_{X_2}}) = \emptyset$.
\end{restatable}

\begin{proof}
(Sketch.) %\DZ{a proof sketch need some more elaboration.}
This theorem is proved along the lines of the AG rule by \citet{DBLP:conf/hybrid/HenzingerMP01}.
Their proof relies on motion primitives having the following properties:
prefix closure,
%if a component permits a flow of a certain duration, then all restrictions of the flow to shorter durations, including 0, are also permitted.
deadlock freedom,
and input permissiveness.
Deadlock freedom is, in this setting \cite{DBLP:conf/hybrid/HenzingerMP01}, means that
    if a precond is satisfied then the trajectory must exists, and
    every execution that does not yet satisfies the postcondition can be prolonged be extended.
Input permissiveness states that a component cannot deadlock no matter how the environment decides to change the inputs.
This condition is needed to do induction over time.
Input permissiveness does not directly follow from the definition of our contracts.
However, it holds when the environment changes the inputs in a way that is allowed by the assumptions.
As \rulename{AGcomp} checks that this is true and rejects the composition otherwise, we can reuse the same proof strategy.
A process should not be allowed to block time making the system ``trivially safe'' but physically meaningless.
We also need to check the disjointness of footprints which is new in our model (needed by \rulename{M-par}).
This is also checked by \rulename{AGcomp}.
\end{proof}
% 
% for every $\sstore{X}_1$ satisfying $\ma_1.\pre$ and $\sstore{X}_2$ satisfying $\ma_2.\pre$,
% if
% \begin{align*}
% \pp_1& \plays\proc{\motion{\dtsess}{\ma_1}.\PP_1}{\sstore{X}_1}{\sstore{W}_1} \parcomp \pp_2\plays\proc{\motion{\dtsess}{\ma_2}.\PP_2}{\sstore{X}_2}{\sstore{W}_2} 
% \rightarrow^*\\
% \pp_1& \plays\proc{\PP_1}{\sstore{X}_1}{\sstore{W}_1} \parcomp \pp_2\plays\proc{\PP_2}{\sstore{X}_2}{\sstore{W}_2} 
% \end{align*}
% then there is a $t$ such that 
% $\pp_1\plays\proc{\motion{\dtsess}{\ma_1\AT t}.\PP_1}{\sstore{X}'_1}{\sstore{W}'_1} \parcomp \pp_2\plays\proc{\motion{\dtsess}{\ma_2\AT t}.\PP_2}{\sstore{X}'_2}{\sstore{W}'_2}$
% that is reachable from the first state and that can reach the second state,
% there exists a global trajectory $\xi:[0,t]\rightarrow ℝ^{X_1\cup X_2}$ with
% $\xi(0)|_{X_i} = \sstore{X}_i$, $\ma_i.\pre\set{\sstore{X}_i/X_i}$ holds, $\xi(t)|_{X_i}$ satisfies $\ma_i.\post$ for $i\in\set{1,2}$,
% and for all $\nu:[0,t]\rightarrow ℝ^{W_1\cup W_2 \setminus(X_1\cup X_2)}$ and all 
% $0\leq t' \leq t$, $\xi(t')|_{X_i}, t'$ satisfies $\ma_i.G$, and the footprints of $\pp_1$ and $\pp_2$ are disjoint:
% $\geom{\pp_1}({\xi(t)|_{X_1}}) \cap \geom{\pp_2}({\xi(t)|_{X_2}}) = \emptyset$.
% \RMi{CHECK: DISCUSS IN CALL}

\subsection{Examples for motion primitives, compatibilities and environments}
%We finish this section with examples.
\myparagraph{Motion primitives from dynamics}
\label{ex:motion}
For the $\Cart$ in \Sec~\ref{sec:example}, we can derive motion primitives from
a simple dynamical model $\dot{x} = v, \dot{v} = u$.
Here, $X = \set{x,v}$ and $W= \emptyset$. 
For simplicity, assume the cart moves along a straight line (its $x$-axis)
and that the control $u$ can apply a fixed 
acceleration $a_{\max}$ or a fixed deceleration $-a_{\max}$.
Consider the motion primitive $\MOVEM$ which takes the cart from an initial position
and velocity $(x_i, v_i)$ to a final position $(x_f, v_f)$.
From high school physics, we can solve for $x$ and $v$, given initial values $x_i$ and $v_i$:\\
\centerline{$
x = x_i + v_it + \frac{1}{2}a_{\max} t^2 \mbox{ and } v = v_i + a_{\max} t
$}
from which, by eliminating $t$, we have $(v - v_i)^2 = 2 a (x - x_i)$.
Suppose that the cart starts from rest ($v_i=0$), accelerates until the midpoint $\mathit{mid} = \frac{1}{2}(x_i+x_f)$, 
and thereafter decelerates to reach $x_f$ again with velocity $v_f= 0$.
The precondition $\pre$ is $x_f > x\wedge v = 0$, the first conjunction saying we move right
(we can write another motion primitive for moving left).
The assumption $A$ is $\true$, and the guarantee is\\
\centerline{
$x_i \leq x \leq x_f \wedge \left(
\begin{array}{c}
(x_i \leq x \leq \mathit{mid} \Rightarrow v^2 = 2 a_{\max} (x - x_i))  \wedge\\
(\mathit{mid} \leq x \leq x_f \Rightarrow v^2 = 2 a_{\max} (x_f - x))
\end{array}
\right)
$}\\[1mm]
The postcondition is $x = x_f \wedge v = 0$.
% In order for the equations of motion to apply, we assume the crane is wound up and not swinging throughout the motion:
% $A \equiv R = 0 \wedge \theta = 0$.
% Using our proof rules, we can derive
% \[
% \judgement{\Cart\plays \MOVEM(x_i,x_f)}{
% 	\pre,	
% 	A,	
% 	G,
% 	v = 0 \wedge x = x_f,
% 	\FP, \delayed}
% \]
% where 
% The guarantee $G$ is given by
% \[
% x_i \leq x \leq x_f \wedge \left(
% \begin{array}{c}
% x_i \leq x \leq \mathit{mid} \Rightarrow v^2 = 2 a_{\max} (x - x_i) \\
% \wedge\\
% \mathit{mid} \leq x \leq x_f \Rightarrow v^2 = 2 a_{\max} (x_f - x)
% \end{array}
% \right)
% \]
The footprint provides a bounding box around the cart as it moves, and is given as in Example~\ref{ex:mp-footprint}.
We assume that the motion cannot be interrupted. Thus, we place the annotation $\delayed$.
The least time to destination is $t_m = 2\sqrt{(x_f-x_i)/a_{\max}}$ and the duration (the interval when it is ready to communicate) is $[t_m, \infty)$. 
A simpler primitive is $\IDLEM$: it keeps the cart stationary.
Its assumption is again $\true$, guarantee (and postcondition) is $x = x_i \wedge v = 0$, footprint is a bounding box around the fixed position.
It is interruptible by messages from other components (annotation $\instantaneous$) at any time: $D = [0,\infty)$. 
%
% Other primitives can be obtained similarly.
% In particular, note that the postcondition of $\IDLEM$ states that the position and velocity on termination is the same
% as that at the start of execution. 
% To express this, we introduce auxiliary variables to track the state at the start of the execution \cite{AptBO09}. We omit the details.

\myparagraph{Compatibility}
Now consider the constraints that ensure the joint trajectories involving the $\Cart$'s motion
and the $\Producer$'s $\WORKM$ primitive are compatible. 
First, note that the motion of the cart is non-interruptible ($\delayed$) but we assume the arm is interruptible,
satisfying the constraint in \rulename{AGcomp} that at most one motion is not interruptible.
Instead of the complexities of modeling the geometry and the dynamics of the arm, we approximate the footprint of the arm
(the geometric space it occupies) as a half-sphere centered at the base of the arm and extending upward.
Assume first that the motion primitive guarantees that the state is always within this half-sphere. 
In order for the cart and the robot arm to be compatible, we have to check that the footprints do not overlap.
Our guarantee is too weak to prove compatibility, as the footprint of the cart and the arm can intersect when the
cart is close to the arm.
Instead, we strengthen the guarantee to state that the arm can use the entire sphere when the cart is far and
as the cart comes closer the arm effector moves up to make space.

To realise this motion, the cart sends the arm the following information with $\ARRIVE$:\footnote{
	For clarity, the type in Figure~\ref{fig:basic-example} omits parameters to messages. Our type system
	uses predicated refinements to reason about parameters.
}
its current position $x_i$, its target position $x_f$, and a lower bound $t_{\mathit{ref}}$ on the time
it will take to arrive at $x_f$.
The footprint for the cart's motion can be specified by 
$\set{(\mathsf{x}, \mathsf{y}, \mathsf{z}) \mid \mathsf{x} ≤ x_0 + l/2 + (x_1 - x_0) * t / t_{\mathit{ref}} ∧ … }$.
For the producer, suppose $R_{\mathit{base}}$ is the radius of its base and $x_{\Producer}$ its $x$ coordinate. 
The footprint of the $\WORKM$ action is strengthened 
as $\set{(\mathsf{x}, \mathsf{y}, \mathsf{z}) \mid (\mathsf{z} >  \min(c t, h) \lor |\mathsf{x} - x_\Producer| ≤ R_{\mathit{base}})  ∧ … }$,
where $c ≥ h \cdot |x_0 -l - x_\Producer - R_{\mathit{base}}| / t_{\mathit{ref}}$.
% 
Finally, for compatibility, we need to check that both $\Cart$ and $\Producer$ can adhere 
to their footprint and that the footprints are disjoint.
Disjointness is satisfied if $x_1 + l < x_\Producer - R_{\mathit{base}}$, set this as a precondition to $\MOVEM$.


\myparagraph{Environment Assumptions}
We can model a more complex cart moving in a dynamic environment
by adding a new component (participant) $\Env$ (for \emph{environment}). 
The physical variables of the environment process encode dynamic properties of the state, such as
obstacles in the workspace or external disturbances acting on the cart.
We can abstract the environment assumptions into a single motion primitive whose guarantees provide
assumptions about the environment behavior to the other components.
For example, the environment providing a bounded disturbance of magnitude to the cart's acceleration could be 
modeled as the guarantee $-1 \leq d \leq 1$ for a physical variable $d$ (for \emph{disturbance}) of $\Env$.
The cart can include this input variable in its dynamics: $\dot{v} = u + d$.
We can also model sensor and actuator errors in this way.
Likewise, we can model obstacles by a physical variable in the environment that denotes the portions
of the state space occupied by obstacles, exporting this information through the guarantees, and
using this information when the cart plans its trajectory in $\MOVEM$. 

\begin{comment}

\RMi{NEED TO FIX FROM HERE}
%
We impose more structured communications by checking 
the compatibility of assume-guarantee contracts in motion types.
Suppose that $\Gmotion{\dtsess}{(\pp_i{:}\ma_i)}{\GL}$ appears in the global type.
This indicates that the specification expects the components $\pp_i$, $i\in I$, to jointly
execute motion primitives $\ma_i$.
The proof rules of \Sec~\ref{sec:motion} provide contracts for each individual motion primitive.
Compatibility checks that these contracts can be put together:
first, the assumptions and guarantees are compatible; 
second, there is no ``leftover'' assumption;
and
third, the footprints of the motion primitives do not intersect in space. 
The compatibility check is performed bottom up in the tree structure of a program.
For this, we introduce the program-level judgement
$\pjudgement{\Pi}{\phi,A, G, \psi,\FP, \timestep}$
extending the judgement
$\judgement{\pc\plays S}{\cdot}$ in Figure~\ref{fig:proof-system}
to programs.
At the leaves, the program-level judgement holds if the corresponding motion primitive holds:
\[
\small
\inferrule*[Left=\rulename{HCompBase}]{
     \judgement{\pp \plays S}{φ,A,G,ψ,\FP,D,\timestep} 
}{
     \pjudgement{\pp \plays S}{φ,A,G,ψ,\FP,D,\timestep} 
}
\]
Recursively, the program-level judgement composes the motion primitives:
\[
\small
\inferrule[\rulename{HComp}]
    { ∃ \FP_1, \FP_2.\\
      G₁\wedge G₂ ⇒ \FP_1 ∩ \cTop(\FP_2) = ∅ \\
      G₁ \wedge G₂ ⇒ \FP_1 ∪ \cTop(\FP_2) ⊆ \FP \\
      \timestep_1 =\instantaneous \vee \timestep_2 = \instantaneous \\\\
      \timestep_1 =\delayed ⇒ D₁ ⊆ D₂ \\
      \timestep_2 =\delayed ⇒ D₂ ⊆ D₁ \\\\
     \pjudgement{P}{φ₁,A∧\con(G₂),G₁,\FP_1,ψ₁,D_1,\timestep_1} \\\\
     \pjudgement{Q}{\pToc(φ₂),\pToc(A∧\con(G₁)),\pToc(G₂),\FP_2,\pToc(ψ₂),D_2,\timestep_2} \\
     }
    {\pjudgement{\comp{P}{\con}{\cTop}{Q}}{φ₁∧φ₂,A,G₁∧G₂,\FP,ψ₁∧ψ₂,D₁∩D₂,\timestep_1\oplus\timestep_2}}
\]
There are three checks.
First, the check on footprints ensures that the motion primitives are disjoint in space
(there is a way to find subsets $\FP_1$ and $\FP_2$ of the footprint $\FP$ so that the composed
motion primitives are in these disjoint portions).
Second, the guarantee of one motion primitive is used as the assumption of the other to check
that they are compatible.
Third, at most one process executes a non-interruptible motion primitive.
We say 
$\Gmotion{\dtsess}{(\pp_i {:} \ma_i)}{\GL}$ is \emph{compatible} if
$\pjudgement{\Pi}{\true, \true, \cdot, \cdot, \FP, \timestep}$ is derivable using these rules.

Note that the composition rule restricts the use of joint motion primitives to the common case
that at most one component executes a non-interruptible motion primitive while the others execute
interruptible ones. 
This is sufficient for a number of common robotics coordination case studies \cite{PGCD}, e.g.,
our running example. 
A more complex rule that allows multiple non-interruptible trajectories that require different 
execution times would additionally track the minimum and maximum durations of trajectories but we
prefer our current rule for simplicity.

% 
% \[
% \inferrule[(HComp)]
%     { ∃ \FP_1, \FP_2.\\
%       G₁ ⇒ \FP_1 ∩ \cTop(\FP_2) = ∅ \\
%       G₁ ⇒ \FP_1 ∪ \cTop(\FP_2) ⊆ \FP \\\\
%      \judgement{\pp \plays S₁}{φ₁,A∧\con(G₂),G₁,\FP_1,ψ₁,\timestep} \\
%      \judgement{\q \plays S₂}{\pToc(φ₂),\pToc(A∧\con(G₁)),\pToc(G₂),\FP_2,\pToc(ψ₂),\timestep} \\
%      }
%     {\judgement{\comp{(\pp \plays S_1)}{\con}{\cTop}{(\q \plays S_2)}}{φ₁∧φ₂,A,G₁∧G₂,\FP,ψ₁∧ψ₂,\timestep}}
% \]

Theorem~\ref{th:motion-compatibility} below lifts Theorem~\ref{th:motion-soundness} to programs using
(\rulename{HComp}) to combine processes.

\begin{theorem}[Compatibility] 
\label{th:motion-compatibility}
Let $\pjudgement{P}{\phi,A,G,ψ,\FP, \timestep}$.
For any 
$\rbtstate{P}{\sstore{X}_0}{\sstore{W}_0}{\sstore{V}_0}$,
if $\sstore{X}_0, \sstore{W}_0, \sstore{V}_0$ satisfies $\phi$
then
for all 
$\rbtstate{P_1}{\sstore{X}_1}{\sstore{W}_1}{\sstore{V}_1}$
$n$-reachable from
$\rbtstate{P}{\sstore{X}_0}{\sstore{W}_0}{\sstore{V}_0}$ under $A$ for some hyperinteger $n\geq 0$,
we have $\sstore{X}_1$ satisfies $G[n\cdot\dt/\clock]$ and
one of the following holds.
\begin{enumerate}
\item
There is no
$\rbtstate{P_2}{\sstore{X}_2}{\sstore{W}_2}{\sstore{V}_2}$ such that
$\rbtstate{P_1}{\sstore{X}_1}{\sstore{W}_1}{\sstore{V}_1} \rightarrow 
\rbtstate{P_2}{\sstore{X}_2}{\sstore{W}_2}{\sstore{V}_2}$
and $\sstore{X}_1,\sstore{W}_1,\sstore{V}_1$ satisfies $\psi$.

\item
For every 
$\rbtstate{P_1}{\sstore{X}_1}{\sstore{W}_1}{\sstore{V}_1} \xrightarrow{\tau} \rbtstate{P_2}{\sstore{X}_2}{\sstore{W}_2}{\sstore{V}_2}$
we have 
$\sstore{X}_2$ satisfies $G[n\cdot \dt/\clock]$ and $\geom{\pc}(\sstore{X}_2,\sstore{V}_2)\subseteq \FP[n \cdot \dt/\clock]$;
and
for every 
$\rbtstate{P_1}{\sstore{X}_1}{\sstore{W}}{\sstore{V}} \xrightarrow{\dt} \rbtstate{P_2}{\sstore{X}_2}{\sstore{W}_2}{\sstore{V}_2}$
we have $\sstore{X}_2$ satisfies $G[(n+1)\cdot \dt/\clock]$ and 
$\geom{\pc}(\sstore{X}_2,\sstore{V}_2)\subseteq \FP[(n+1) \cdot \dt/\clock]$.
\end{enumerate}
\end{theorem}

\end{comment}





==> experiments.tex <==
\section{Implementation and Case Study}
\label{sec:eval}
\myparagraph{Implementation}
%
Our implementation has two parts.
The first part takes a program, a specification for each motion primitive, and a global type and checks
that the type is well-formed and that each process satisfies its local type.
The second part implements the program on top of
the Robotic Operating System (ROS)~\cite{ROS}, a software ecosystem for robots.
We reuse the infrastructure of motion session types \cite{ECOOP19}; for example, we write programs in \PGCD syntax \cite{PGCD}.
The verification infrastructure is about 4000 lines of Python code, excluding the solver.
The code is available at \url{https://github.com/MPI-SWS/pgcd} and instructions to run these experiments are located in the \texttt{oopsla20\_artifact} branch.

Internally, we represent programs and global types as state machines \cite{DBLP:conf/esop/DenielouY12}, and implement the dataflow analysis
on this representation.
Additionally, we specify motion primitives in the local co-ordinate system for each robot and automatically
perform frame transformations between two robots.
The core of ROS is a publish-subscribe messaging system; we extend the messaging layer to implement a synchronous message-passing layer.
Our specifications contain predicates with nonlinear arithmetic, for example, to represent footprints of components as spheres.
Obstacle are represented as passive components, i.e., components which have a physical footprint but do not execute program.
Such components can interact with normal components through input and state variables and their are considered when checking the absence of collision.
On the other hand, the obstacles are excluded from the checks related to communication, e.g., synchronisability.
We use the dReal4 SMT solver \cite{dReal} to discharge validity queries.
The running times are obtained on a Intel i7-7700K CPU at $4.2$GHz and dReal4 running in parallel on 6 cores.

\myparagraph{Tests}
We evaluate our system on two benchmarks and a more complex case study:
(1) We test scalability of the verification using micro-benchmarks. 
(2) We compare our approach with previous approaches
on a set of robotic coordination scenarios from the literature \cite{PGCD,ECOOP19}, and
(3) As a large case study, we verify and implement 
a complex choreography example based on a variation of the example from \Sec~\ref{subsec:large}.


% An object is loaded by the producer on the cart and all the participants gets notified.
% The difference is that the cart does not yet know the color of the object.
% It first drive to a sensor (color sorter) which tells what the color is.
% Then the protocol continues as described in the example.

\begin{wrapfigure}{r}{5cm}
\centering
\includegraphics[width=45mm]{figs/lanes.pdf}
\vspace{-2ex}
\caption{Parallel lanes micro-benchmarks}
\label{fig:lanes}
\vspace{-2ex}
\end{wrapfigure}

\myparagraph{(1) Micro-benchmarks}
The micro-benchmarks comprise a parametric family of examples that highlight the advantage 
of our motion session calculus, specifically the separating conjunction, over previous typing
approaches \cite{ECOOP19}.
The scenario consists of carts moving back and forth along parallel trajectories, and is
parameterised by the number of carts.
Fig.~\ref{fig:lanes} shows the verification times for this example in the two systems.
We start with 2 robots and increase the number of robots until we reach a $200$ s. timeout for the verification.
The previous calculus is discrete-time and does not separate independent components.
Thus, the type system synchronises every process and, therefore, generates complex collision checks which quickly overwhelms the verifier.
Our global types use the separating conjunction to split the specifications into independent pieces
and the verifcation time increases linearly in the number of processes.

\myparagraph{Setup for (2) and (3)}
For examples used previously in related works \cite{PGCD,ECOOP19}, we write specifications
using our motion session types, taking advantage of the modularity of the type system. 
% We show that the richer specifications presented in this paper can also help the verification.
For the new case study (part (3)), we implement a variation of the example presented in \Sec~\ref{sec:example},
where we decouple the producer placing an object and a sensor that determines if the object is green or red.
Thus, after the producer places an object on the cart, the cart first moves to the sensor, communicates with
the sensor to get the color, and then delivers the object as described in the protocol.
We filmed our experiments and a short video can be seen in the \textbf{\emph{supplementary materials}}.
%
We use three robots: a custom-built robot arm modified from an open-source arm, a commercial manipulator,
and a mobile cart, as shown in Figure~\ref{fig:robots-xp}.
We use placeholders for the producer arm and color sensor, as we do not have additional hardware (and arms are expensive).
The robots are built with a mix of off-the-self parts and 3D printed parts as described below.

% \begin{description}
\textbf{\emph{Arm}.}\ 
    The arm is a modified BCN3D MOVEO ({\url{https://github.com/BCN3D/BCN3D-Moveo}}).
    The upper arm section is shortened to make it lighter and easier to mount on a mobile cart. 
    % Due to the large power consumption of the stepper motors, it is powered by a tether.
    It has three degrees of freedom.
    % The arm with its control electronics is mounted on top of the larger cart.
    % In this experiment, we do not use the larger cart which only acts as the base of the arm.
    The motion primitives consist of moving between poses and opening/closing the gripper.
    The motion is a straight line in the configuration space (angles of the joints) which corresponds to curves in physical space.

\textbf{\emph{Panda Arm.}} \ 
    The Panda arm by Franka Emika ({\url{https://www.franka.de/technology}}) is a seven degrees of freedom commercial manipulator platform.
    It is controlled similarly to the MOVEO arm but with a more complex configuration space.
	The Panda arm has a closed-loop controller and can get to a pose with an error less than 0.1mm.
	The controller also comes with collision detection using feedback from the motors.
	We command this arm using a library of motion primitives provided by the manufacturer.

\textbf{\emph{Mobile Carts}.} \ 
    There are two carts.
    Both are omnidirectional driving platforms.
    One uses mecanum wheels and the other omniwheels to get three degrees of freedom 
    (two in translation, one in rotation) and can move between any two positions on a flat ground.
    The advantage of using such wheels is that all the three degrees of freedom are controllable and movement does not require complex planning.
    Its basic motion primitives are moving in the direction of the wheels, moving perpendicularly to the direction of the wheels, and rotating around its center.
    % The cart is battery powered.
% \end{description}

The arm and cart are equipped with RaspberryPi 3 model B to run their
processes and use stepper motors.
This enables a control of the joints and wheels with less than 1.8 degree of error.
However, these robots do not have global feedback on their position and keep track of their state using \emph{dead reckoning}.
This can be a challenge for the cart, which keeps accummulating error over time.
As our example is a loop, we manually reset the cart's position when it gets back to the producer after delivering the object.
(A more realistic implementation would use feedback control, but we omit this because control algorithms are a somewhat orthogonal
concern.)
For the producer and the color sorter, we run the processes but have placeholders in the physical world and realise the corresponding action manually.
%For the producer, we place a new cube on the arm manually and then trigger sending the next message.
% For the color sorter, we fix a priori a sequence of colors.
% Therefore, when a request for the color is received.
% For first request is a red object and then green objects.
%These two programs run on a separate laptop.
%
All computers run Ubuntu 18.04 with ROS 2 Dashing Diademata.

Table~\ref{tbl:xp1} shows the specification for the robots and their motions.
As the two carts share most of their specification, we group them together.
The specification includes the geometrical description of the robots and the motion primitives.


\myparagraph{(2) Revisiting the Examples from \PGCD}
As we build on top of \PGCD, we can use the examples used to evaluate that system.
We take 4 examples, for which we compare the specification effort 
in the previous calculus \cite{ECOOP19} to our new calculus.
As the two calculi have different models for the time and synchronisation, we 
made some minor adaptations such that the same programs can be described by the two calculi.
The old calculus requires motion primitives to have fixed duration and does not support interruptible motions.
Furthermore, there is no ``$\GLPAR$'' in the old calculus so all the motions are always synchronised.
In our new specification, we take advantage of our richer calculus to better decompose the protocol.
% 
% Illustrations of the examples can be found in \cite{PGCD}.
We use the following scenarios.
\begin{description}
\item[Fetch.]
    in this experiment, the Moveo arm is attached on top of a cart.
    The goal is to get an object.
    The cart moves toward the object until the object if within the arm's reach.
    The arm grabs the object and the cart goes back to its initial position.
\item[Handover.]
    This experiment is a variation of the previous one.
    There are two carts instead of one and the object to fetch is on top of the new cart.
    The two carts meet before the arm takes an object placed on top of the second cart and then, both go back to their initial positions.
\item[Twist and Turn.]
    In this experiment, the two carts start in front of the each other.
    The arm takes an object from the small cart.
    Then all three robots move simultaneously.

    The cart carrying the arm rotates in place, the other cart describes a curve around the first cart, and arm moves 
    from one side of the cart to the other side.
    At the end, the arm puts the object on the carrier.
\item[Underpass.]
    In this experiment, the arm and the cart cooperate to go under an obstacle.
    First, the cart goes toward the arm, which takes the object from the cart. 
    The cart goes around the arm passing under an obstacle. 
    Finally, the arm puts the object back on the cart on the other side of the obstacle.
\end{description}

Table~\ref{tbl:xp-revisit} reports the size of the examples and their specifications, as well as the verification time.
The verification time is broken down into syntactic well-formedness checks on the choreography, 
the motion compatibility checks for the trajectories, and typing the processes w.r.t.\ local types.
The motion compatibility checks dominate the verification time.
When we compare our new calculus to the previous approach, we can 
observe that the global types are slightly larger but the verification time can be significantly smaller.
The increase in specification size comes with the addition of new Assume-Guarantee contracts when $\GLPAR$ is used.

The verification time from the existing specification are higher than the time reported in the previously published results.
When implementing our new calculus, we found and fixed some bugs in the verifier code from \PGCD.
Those bugs resulted in incomplete collision checks and fixing them increased the burden on the SMT solver.\footnote{\label{note:dreal}
	Two out of 217 queries in the Fetch example are particularly hard for the solver and could not be solved with 1 hour.
	We suspect a bug in the solver as all the other queries are solved in $134$s.
}

\newcommand{\centercell}[1]{\multicolumn{2}{c}{#1}}

\begin{table}[t]
\centering
\caption{Programs, specification, and verification time for the \PGCD examples. ``Prev'' refers to \cite{ECOOP19}.}
\vspace{-1ex}
\scriptsize
\begin{tabular}{lrrr|cc|cc|cc|cc} \toprule
Scenario        & \multicolumn{3}{c}{Program (Loc)}     & \centercell{Global Type}  & \centercell{Syntactic}    &  \centercell{Motion}         & \centercell{Typing (s.)}  \\
                &           &         &                 & \centercell{(LoC)}        & \centercell{Checks (s.)}  &  \centercell{Compatibility (s.)}     &                      \\ 
                &   Arm     & Cart 1  & Cart 2          & Prev & This work&  Prev & This work  & Prev &  This work   &  Prev & This work   \\ \midrule
Fetch           &  $14$     &  $19$   &  $-$            &    $22$ & $42$            &       $0.1$  & $0.1$      & $> 3600$ \footnoteref{note:dreal} &   $\bf 7$           &  $0.1$ & $0.1$       \\
Handover        &   $9$     &   $8$   &  $6$            &    $14$ & $26$            &       $0.1$  & $0.1$      &   $2224$  &   $\bf 70$           &  $0.1$ & $0.1$       \\
Twist and turn  &   $12$    &  $16$   &  $6$            &    $15$ & $17$            &       $0.1$  & $0.1$      &    $599$  &  $\bf 203$           &  $0.1$ & $0.1$       \\ 
Underpass       &   $18$    &   $3$   & $14$            &    $21$ & $65$            &       $0.1$  & $0.1$      &    $187$  &  $\bf 114$           &  $0.1$ & $0.1$       \\ \bottomrule
\end{tabular}
\label{tbl:xp-revisit}
\end{table}


\begin{figure}[t]
\centering
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=0.965\textwidth]{sorting_setup.jpg}
        \caption{Setup}
        \label{fig:robots-xp-setup}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{sorting.jpg}
        \caption{Sequence of motions}
        \label{fig:robots-xp}
    \end{subfigure}
\vspace{-1ex}
    \caption{Experimental setup for the sorting example}
\vspace{-1ex}
\end{figure}
%
\myparagraph{(3) A Complex Case Study}
%
The purpose of the case study is to show that we can semi-automatically verify systems beyond the scope of previous work. 
Table~\ref{tbl:xp1} shows the sizes of the processes (in lines of code, in the syntax of \PGCD)
and statistics related to the global specification and verification time. 
The global specification consists of the global type, the environment description, 
and (manually provided) annotations for the verification.
The annotations are mostly related to the footprints and the parallel composition.
Each time we use the parallel composition operator we specify a partition of 
the current footprint (the ``$\exists \FP_1,\FP_2$'' in rule \rulename{AGcomp}).

% We call each validity query arising out of motion compatibility checking or during type checking a process against
% a local type and a \emph{verification condition}.
In Table~\ref{tbl:xp1}, we split the running times into the well-formedness checks which can be done syntactically,
the verification conditions for the execution of the motion primitives, and the typing.
We did not try to encode this example using the older \PGCD specifications for two reasons.
First, the stronger requirement on discrete time steps and global synchronisation in time in the previous calculus would subtantially change this example.
Remember that motions in \cite{ECOOP19} are specified simultaneously for all the robots and must have the same duration.
When multiple motion primitives have different durations, a motion step 
can only be as long as the shortest motion. 
Thus, we would need to chunk the longer motions into a sequence of smaller steps. 
This would, in turn, make the (sub)typing much more difficult as one motion step in the code would correspond to 
a sequence of motion steps in the specification.
%
Second, as the previous calculus does not include the separating conjunction, 
there is little hope that the SMT solver can cope with the compelxity of this example: it contains more robots and more complex ones.
Because our global types include separating conjunctions, we can more efficiently generate and discharge the 
verification conditions.
At the modest cost of specifying the footprints for each thread, the 
collision checks only need to consider the robots within a thread and not all the robots in the system.
This brings a substantial reduction in the complexity of the verification conditions.
% In particular the number of collision checks is quadratic in the number of robots.
% In Table~\ref{tbl:xp1}, we also compare our method to the verification 
% used in earlier work on motion session types \cite{ECOOP19}: while our checks terminated in less than 10 minutes,
% the non-modular checks of \cite{ECOOP19} timed out (after 1 hour).

In conclusion, the case study demonstrates the power of our method
in specifying and verifying non-trivial coordination tasks between multiple robots.
% The more precise analysis of the motion duration and the distinction between (non-)interruptible motions 
% allows for complex co-ordination protocols.
It requires the expressiveness of our motion primitive specifications
and the modularity of our separating conjunction.

\begin{table}[t]
\centering
\caption{Programs, motion specification, type, and verification time}
\vspace{-1ex}
\small
\begin{tabular}{lcc|lrl} \toprule
Robot     &   Motion Spec (LoC)   &   Program (LoC)   & Specification      \\ \midrule
Moveo arm &   306                 &   28              & Global type          &  96               & LoC          \\
Panda arm &   348                 &   31              & Syntactic   checks   &  0.2              & s.           \\
Carts     &   404                 &   45              & Compatibility checks &  2410             & s.           \\
Sensor/Producer    &   105        &   17 / 10             & Typing               &  3.1              & s.           \\ \bottomrule
\end{tabular}
\label{tbl:xp1}
\vspace{-1ex}
\end{table}



==> intro.tex <==
\section{Introduction}
\label{sec:intro}

Modern robotics applications are often deployed in safety- or business-critical applications
and formal specifications and reasoning about their correct behaviours is a difficult and challenging problem.
These applications tightly  
integrate computation, communication, control of physical dynamics,
and geometric reasoning.
Developing programming models and frameworks for such applications has been long noted as an important and challenging problem
in robotics \cite{Lozano-Perez}, 
and yet very little support exists today for compositional specification of behaviours or their static enforcement. 
% No existing formalism is capable of 
% modelling all these features together, directly guiding  
% safe and correct programming of robotics systems assisted 
% by static and compositional behavioural specifications and program 
% verifications.  

In this paper, we present a programming model for concurrent robotic systems
and a type-based approach to statically analyse programs. 
Our programming model uses \emph{choreographies}---global protocols which allow implementing distributed and concurrent 
components without a central control---to compositionally specify and statically verify both 
message-based communications and jointly executed motion between robotics components in the physical world.
Our choreographies 
extend \emph{multiparty session types} \cite{HYC08}
with \emph{dynamic motion primitives}, which represent 
pre-verified motions that the robots can execute in the physical world.
We compile well-typed programs into robotics platforms.
We show through a number of nontrivial usecases 
how our programming model can be used to design and implement
correct-by-construction, complex, robotic applications on top 
of commercial and custom-build robotic hardware.

Our starting point is the theory of motion session types
\cite{ECOOP19}, which forms 
a type discipline based on global types with simple, discrete-time motion primitives. 
For many applications, we found this existing model 
too restrictive: it requires that all components agree on a pre-determined, global,
discrete clock and it forces \emph{global synchronisation} among all robots at the fixed interval
determined by the ``tick'' of the global clock.
For example, two robots engaged in independent
activities in different parts of a workspace must 
nevertheless stop their motion and synchronise every tick.
This leads to communication-heavy programs in which the programmer must either pick
a global clock that ensures every motion primitive can finish within one tick
(making the system very slow) or that every motion primitive is interruptible
(all robots stop every tick and coordinate).
Our new model enhances the scope and applicability of motion sesstion types to robots: 
we go from the global and discrete clock to \emph{continuous
behaviours} over time, allowing complex synchronisations as well as
\emph{frame separation} between independent subgroups of robots.
That is, the programmer does
not need to think about global ticks when writing the program. 
Instead, they think in terms of motion primitives and the type system enforces that concurrent composition of 
motions is well-formed and that trajectories exist in a global timeline.


Reasoning simultaneously about dynamics and message-based
synchronisation is difficult because time is global and can be used as
an implicit broadcast synchronisation mechanism.  
The complexity of our model arises from the need to ensure that every component is
simultaneously ready to let time progress (through dynamics) or 
ready to send or receive messages (property \emph{communication
  safety}).  At the same time, we must ensure that systems 
are able to correctly execute motion primitives
(property \emph{motion compatibility});
and jointly executed
trajectories are separated in space and time (property \emph{collision
  freedom}).  
Our verification technique is \emph{static}: if a program type checks, then
every execution of the system satisfies communication safety, motion compatibility, and collision freedom. 
We manage the complexity of reasoning about the interplay between dynamics and concurrency
through a separation of concerns.

First, we specify \emph{continuous-time trajectories} as \emph{motion primitives}.  
Since the dynamics of different components can
be coupled, the proof system uses 
an \emph{assume-guarantee proof system}
\cite{AbadiLamport93,ChandyMisra88,Jones83,DBLP:journals/pieee/NuzzoSBGV15} on continuous time
processes to relate an abstract motion primitive to the original
dynamics.  The assume guarantee contracts decouple the dynamics.  
Additionally, the proof system also checks that trajectories
ensure disjointness of the use of geometric space over time.

Second, we interpret choreographic specifications in continuous time, 
and extend the existing formalism in \cite{ECOOP19} with \emph{predicate refinements}---to reason about
permissions (i.e., what parts of the state space an individual robot can access without colliding into a different robot). 
This is required for motion compatibility and collision freedom. 
We also introduce a \emph{separating conjunction} operator to reason about disjoint frames.  
The combination of message passing and dynamics makes static verification challenging.
We introduce a notion of \emph{well-formedness} of choreographies 
that ensures motion and communication can
be synchronised and disallows, e.g., behaviours when a message is blocked because a motion
cannot be interrupted.
We give an algorithm for checking well-formedness using a dataflow
analysis on choreographies.
We show that well-formed types can be projected on to end-components
and provide a local type checking that allows refinement between
motion primitives. %using a technique in \cite{LiquidTypes}. 

Checking compatibility and collision freedom reduces to validity queries in the underlying logic.
%  that we discharge through an SMT solver.
Interestingly, the separating conjunction allows subgroups of robots to
interact---through motion and messages---disjointly from other subgroups;
this reduces the need for global communication in our implementations.

We compile well-typed programs into programs in the PGCD \cite{PGCD} and ROS \cite{ROS} frameworks.
We have used our implementation to program and verify a number of complex robotic coordination and manipulation
tasks.
Our implementation uses both commercial platforms (e.g., the Panda 7DOF manipulator, the BCN3D MOVEO arm)
and custom-built components (mobile carts).
In our experience, our programming model and typing discipline are sufficient to specify 
quite complex manoeuvres between multiple robots and to obtain verified implementations.
Moreover, the use of choreographies and the separating conjunction are crucial in reducing verification effort: 
without the separating conjunction, verification times out on more complex examples. 
Our implementation uses SMT solvers to discharge validity queries arising out of the proof system;
our initial experience suggests that while the underlying theories (non-linear arithmetic) are 
complex, it is possible to semi-automatically prove quite involved specifications. 

\paragraph{\bf Contributions and Outline}
This paper provides a static compositional modelling,
verification, and implementation framework through behavioural 
specifications for
concurrent robotics applications 
that involve reasoning about message
passing, continuous control, and geometric separation.
We manage this complexity by decoupling dynamics and message
passing and enables us to specify and implement robotic applications on top of commercial and custom-build robotic hardware.
Our framework coherently integrates programming languages techniques,
session type theories, 
and static analysis techniques; 
this enables us to model \emph{continuous behaviours} over time in the presence of
complex synchronisations between independent subgroups of robots.
We extend the global types in \cite{ECOOP19}
  to \emph{choreographies} including 
  key constructs such as framing and predicate refinements,
  together with separation conjunctions,  
  and integrate the typing system with an assume-guarantee proof system. We
  implement our verification system using a new set of robots
  (extending \cite{ECOOP19,PGCD}) in order to 
program and verify complex coordinations and manipulation tasks.

The rest of the paper is organised as follows.
\begin{description}
\item[\underline{\sc\Sec~\ref{sec:example}}:]
  We first motivate our design for robotics specifications, 
and explain the correctness
  criteria -- \emph{communication safety},
  \emph{motion compatibility}, and
  \emph{collision freedom} with an example.
\item[\underline{\sc\Sec~\ref{sec:calculus}:}]
We introduce a \emph{multiparty motion session calculus} with 
\emph{dynamic abstract motion primitives};
we provide an assume guarantee proof
system to construct abstract motion primitives 
for maintaining geometric
separation in space and time for concurrently executed motion
primitives. We then
prove Theorem~\ref{th:motion-compat} (\emph{Motion Compatibility}).  
\item[\underline{\sc\Sec~\ref{sec:proof-system}:}]
  We provide \emph{choreographic specifications}
enriched with dynamic motion primitives and separation operator,  
and define their dataflow analysis. 
We propose a typing system and prove 
its main properties, 
Theorem~\ref{th:SR} (\emph{Subject Reduction}),
Theorem~\ref{th:progress} (\emph{Communication and Motion Progress} and
\emph{Collision-free Progress}). 
%
\item[\underline{\sc\Sec~\ref{sec:eval}:}]  
We describe our implementation, evaluation, and case studies. 
Our evaluation demonstrates that our framework allows specifying
complex interactions and verifying examples beyond the scope of previous work.
%
\item[\underline{\sc\Sec~\ref{sec:related} and \Sec~\ref{sec:discussion}:}]
  We discuss related work and conclude with 
  a number of open challenges in reasoning about robotics applications. 
\end{description}
%
Putting it all together, we obtain a compositional specification and 
implementation framework for concurrent robotics applications.
% that goes beyond the scope of existing techniques.
Our paper is a starting point rather than the final word on robot programming.
Indeed, we make many simplifying assumptions about world modeling,
sensing and filtering, and (distributed) feedback control and planning.
Even with these simplifications, the theoretical development is non-trivial.
With a firm understanding of the basic theory, we hope that future work
will lift many of the current limitations.

% \iffull
% {\bf\emph{{Artifact}}}
% contains an implementation of our typing system, a verification backend, 
% and the code and specification for our test examples.
% This will enable checking the verification aspects of our system.
% Running the scenario requires access to specialised hardware.
% {\bf\emph{{Appendix}}} \cite{} includes the detailed proofs and 
% omitted definitions.

% \else
% {\bf\emph{{The full version}}} \cite{fullversion} 
% includes the detailed proofs. 
% \fi
% {\bf\emph{Supplementary material}} includes 
% a video of our case study. Please cite link here. 

\begin{comment}
We expand the example in Figure~\ref{fig:cart-crane} and motivate the constructions in our language in \Sec~\ref{sec:example}.
\Sec~\ref{sec:lang} defines a core language for robotic interactions and its operational semantics.
Sections~\ref{sec:motion} and~\ref{sec:proof-system} build our proof system: first, by constructing abstract motion
primitives from programs and then by incorporating them into a multiparty motion session type system.
We discuss related work in \Sec~\ref{sec:related} and
conclude with future work in \Sec~\ref{sec:conclusion}. 

\RMi{OLD:}
In this paper, we provide a compositional proof system for robotics applications.
To understand the capabilities such a proof system must provide, let us consider a simple example
of a cart and crane assembly transporting a mass from a trolley (Figure~\ref{fig:cart-crane}).
The cart assembly rolls on horizontal tracks and has a motor that produces a horizontal force.
The crane consists of a winch with a cable that can be used to hoist a load.
The combination of the cart and the crane can transport a load from some initial
position to another; the cart communicates with a trolley to find the initial 
position for the load and to inform it when the load is picked up. 
Figure~\ref{fig:cart-crane}(a) shows the schematic of the system.
The task of transporting the load from the trolley requires several steps and involve synchronisation between the software 
running on each component and joint execution of trajectories in space such that there is no collision.

In more detail, a possible protocol for the task is as follows (see Figure~\ref{fig:cart-crane}(b) to see the visual
flow of messages and control actions).
Initially, we assume that the cart is at rest.
First, the trolley sends a message giving the initial position of the load to the cart and remains
at rest at that location.
The cart sends a message to the crane to roll up its cable.
This is to ensure the cable does not swing around (and hit objects in the workspace)
while the cart moves to the load as well as to remove a drag due to the cable.
While the cart remains stationary, the crane rolls its cable.
When it is done, the crane sends an acknowledgement to the cart.
At this point, the cart executes a motion primitive to move it on top of the load to be transported.
In the meantime, the crane remains idle.
Once the cart is on top of the load and stationary, it sends the crane a message to unroll
the cable up to the position of the load and to grip the load.
This involves the crane executing a motion primitive to unroll the cable, grab the object, and roll it
up again.
When this action is done, the crane synchronises with the cart.
At this point, the cart confirms the pickup with the trolley and the protocol is over.

In summary, a correct implementation of the task requires coordination and planning at the discrete level and executing trajectories
at the continuous level, while ensuring components do not collide.
% The flow of information is bidirectional: the planning informs the control but, in the presence of new
% information from the controllers, the plan may need to be changed. 
% A software stack \cite{DBLP:journals/jfr/CremeanFGHKKLLLRSBM06,DBLP:journals/tecs/WongpiromsarnMLM12} for such system may start with a decision stage to sequence of actions in order to achieve an objective.
% At that level actions are black box we call \emph{motion primitives}.
% At an intermediate level, a planner decides how theses black box actions are implemented and finds a trajectory that the system needs to follow.
% At the lowest level, controller are tasked to follow the trajectory.
% The flow of information between layer is not only top-down but also bottom-up.
% When sensors report new information, a trajectory may need to be adjusted or may become impossible in which case a new sequence of action needs to be recomputed.
% Depending on the level of abstraction, different layers have different views over the same action.
%
Formally reasoning about such interaction between planning and control involves a number of challenges.
Since the system is \emph{concurrent} and synchronises through \emph{message passing}, formal reasoning 
inherits the complexities of concurrent systems.
Since the components control physical state in continuous space and time, and the dynamics
of these states are coupled, reasoning inherits the complexities of continuous control systems and hybrid systems.
Finally, since components reside in geometric space and must be collision-free, 
formal reasoning must consider the use of geometric space by components over time 
as well as reference frame transformations between components. 

There are many languages to model and implement robotics applications---from general purpose
languages like C++ or Python on top of libraries such as ROS to domain-specific languages
\cite{Nordmann2016survey} and to generic modelling languages such as Simulink or Modelica.
They usually provide features for concurrency, dynamics, and geometric reasoning but little 
support for compositional reasoning.
Typically, verification support is limited to testing/simulation or global model checking.

On the other hand, models and verification tools from formal methods typically support
a subset of these features.
For example, \emph{hybrid automata} \cite{ACHH,Henzinger96} support continuous dynamics but little support for
compositional reasoning about concurrency and geometry.
\emph{Session types} \cite{THK,HKV98} support modular specifications and type-checking about message-passing but not continuous dynamics.
\emph{Program logics} \cite{AptBO09,DBLP:conf/lics/Reynolds02,DBLP:conf/lics/CalcagnoOY07} support 
compositional reasoning about concurrency but do not support continuous dynamics
or geometric reasoning.

Our contribution is a compositional proof system based on session types
to reason about robotics applications with support for dynamics, concurrency, and geometry.
Our starting point is \PGCD \cite{PGCD}, a recent ``core'' language for robotics applications.
We extend \PGCD with explicit support for dynamics in the language (the original papers \cite{PGCD,ECOOP19} 
either abstracted away the dynamics or used a discrete-time semantics) 
and provide an operational semantics for \PGCD programs.
One nontrivial feature of our operational semantics is the use of nonstandard models of reals to give a uniform 
semantics to both continuous and discrete evolution of the system as a sequence of infinitesimally small discrete steps.

Reasoning about dynamics and message-based synchronisation is difficult because time is global in the system.
Thus, our proof system has to ensure that every component is simultaneously ready to let time progress (through dynamics).
Similarly, we must ensure that such jointly executed trajectories are separated in space and time.
We manage the complexity of this reasoning through a separation of concerns. 

First, we abstract the original continuous-time trajectories into \emph{abstract motion primitives}.
Since the dynamics of different components can be coupled, the proof system uses assume guarantee reasoning.
Precisely, we use an \emph{assume-guarantee proof system} \cite{AbadiLamport93,ChandyMisra88,Jones83}
on continuous time processes to relate an abstract motion primitive to the original dynamics.
Our proof system uses the assume guarantee contracts to decouple the dynamics.
Additionally, it also checks that trajectories ensure disjointness of the use of geometric space over time.
% In particular, the separating conjunction is used to account for the use of (geometric) space over time as resources.

Second, we use \emph{multiparty session types} \cite{HYC2016} over abstract motion primitives \cite{ECOOP19}
as the basis for reasoning about global sequences of messages and motions.
The global specification is written as a global type,
which extends existing session typing systems with \emph{predicate refinements} and  
motion primitives connected by separating conjunction.
A global type is projected onto each component to generate a local type for each component.
Our soundness result states that if each component refines its local type, then the composition of the system satisfies the global type.
The combination of message passing and dynamics makes
static type checking challenging but our subtyping relations, which relate structured concurrency with motion,
enable us to handle this complexity. 


In summary, 
we provide the first compositional reasoning framework for robotics applications that involve
reasoning about concurrent message passing, continuous control, and geometric separation.
Our framework manages the complexity of reasoning by decoupling dynamics and message passing.
For the dynamics, we provide an assume guarantee proof system to construct abstract motion primitives.
For concurrency, we define a multiparty motion session type system, which uses motion primitives as abstract
actions, to specify valid sequences.
We show how an implementation of a component can be type checked against the local type obtained by projecting the 
multiparty session type onto the component.
Along the way, our proof systems maintain geometric separation in space and time for concurrently executed motion
primitives.
Putting it all together, we obtain a fully compositional framework for reasoning with complex, distributed robotics applications
that goes significantly beyond the scope of existing techniques.

The rest of the paper is organised as follows.
We expand the example in Figure~\ref{fig:cart-crane} and motivate the constructions in our language in \Sec~\ref{sec:example}.
\Sec~\ref{sec:lang} defines a core language for robotic interactions and its operational semantics.
Sections~\ref{sec:motion} and~\ref{sec:proof-system} build our proof system: first, by constructing abstract motion
primitives from programs and then by incorporating them into a multiparty motion session type system.
We discuss related work in \Sec~\ref{sec:related} and
conclude with future work in \Sec~\ref{sec:conclusion}. 


\end{comment}


% The hybrid and distributed behaviours of CPS requires dealing with
% (1) continuous trajectories of physical components,
% (2) discrete jumps related to the discrete nature of the control software, and
% (3) partial views of the distributed components which need to communicate in order to synchronize their actions.

 
% Having more of less abstract perspective over an event is necessary to handle the complexity.
% However, this raise the question about modeling and formalizing such systems.
% On one hand, on needs to accommodate all theses perspectives while maintaining a consistent model.
% In this work we present a calculus for CPS and an associated proof system.
% Our calculus has a discrete semantics on non-standard analysis \cite{10.2307/j.ctt1cx3vb6}.
% This enables us to use powerful proof systems developed for programming languages.
% In particular, we base our specification and proof system on multiparty sessions types \cite{DBLP:journals/pacmpl/ScalasY19} and separation logics \cite{DBLP:conf/lics/Reynolds02,DBLP:conf/lics/CalcagnoOY07}.
% Our proof system handles at the same time low level controller following continuous trajectories and planning over discrete actions.
% In particular, we show that the discrete, black box motion primitives arise naturally as a form of abstraction \cite{DBLP:conf/popl/OHearnYR04,DBLP:conf/popl/ParkinsonB05} in the proof system.


% \RMi{contributions}
% Ingredients
% 
% - first compositional proof system 
% 
% - reasoning with dynamics, concurrency, and geometry.
% discrete planning and coordination is mixed with control of dynamical systems
% 
% - operational semantics performs frame transforms
% 
% - operational semantics uses nonstandard models to treat continuous flows as (infinitesimally small) discrete steps.
% as a result, classical proof techniques from program logics apply naturally, without extra notational burden
% 
% - dynamics is naturally abstracted as motion primitives
% 
% - space is tracked as a resource in separation logic; this naturally allows geometric reasoning
% 
% - a combination of session types with predicate refinements and rely-guarantee separation logic
% 
% Extensions:
% 
% - multiparty session types + predicate refinement + hybrid dynamics
% 
% - physical state as resource: introducing separation logics to hybrid dynamical systems




==> macro_unicode.tex <==
\usepackage{newunicodechar}
\newunicodechar{∃}{\ensuremath{\exists}}
\newunicodechar{∀}{\ensuremath{\forall}}
\newunicodechar{θ}{\ensuremath{\theta}}
\newunicodechar{τ}{\ensuremath{\tau}}
\newunicodechar{φ}{\ensuremath{\varphi}}
\newunicodechar{ξ}{\ensuremath{\xi}}
\newunicodechar{ζ}{\ensuremath{\zeta}}
\newunicodechar{ψ}{\ensuremath{\psi}}
\newunicodechar{π}{\ensuremath{\pi}}
\newunicodechar{α}{\ensuremath{\alpha}}
\newunicodechar{β}{\ensuremath{\beta}}
\newunicodechar{γ}{\ensuremath{\gamma}}
\newunicodechar{δ}{\ensuremath{\delta}}
\newunicodechar{ε}{\ensuremath{\epsilon}}
\newunicodechar{λ}{\ensuremath{\lambda}}
\newunicodechar{ρ}{\ensuremath{\rho}}
\newunicodechar{σ}{\ensuremath{\sigma}}
\newunicodechar{ω}{\ensuremath{\omega}}
\newunicodechar{Γ}{\ensuremath{\Gamma}}
\newunicodechar{Φ}{\ensuremath{\Phi}}
\newunicodechar{Δ}{\ensuremath{\Delta}}
\newunicodechar{Σ}{\ensuremath{\Sigma}}
\newunicodechar{Π}{\ensuremath{\Pi}}
\newunicodechar{∑}{\ensuremath{\Sigma}}
\newunicodechar{∏}{\ensuremath{\Pi}}
\newunicodechar{Θ}{\ensuremath{\Theta}}
\newunicodechar{Ω}{\ensuremath{\Omega}}
\newunicodechar{⇒}{\ensuremath{\Rightarrow}}
\newunicodechar{⇐}{\ensuremath{\Leftarrow}}
\newunicodechar{⇔}{\ensuremath{\Leftrightarrow}}
\newunicodechar{→}{\ensuremath{\rightarrow}}
\newunicodechar{←}{\ensuremath{\leftarrow}}
\newunicodechar{↔}{\ensuremath{\leftrightarrow}}
\newunicodechar{¬}{\ensuremath{\neg}}
\newunicodechar{∧}{\ensuremath{\land}}
\newunicodechar{∨}{\ensuremath{\lor}}
\newunicodechar{≠}{\ensuremath{\neq}}
\newunicodechar{≡}{\ensuremath{\equiv}}
\newunicodechar{∼}{\ensuremath{\sim}}
\newunicodechar{≈}{\ensuremath{\approx}}
\newunicodechar{≥}{\ensuremath{\geq}}
\newunicodechar{≤}{\ensuremath{\leq}}
\newunicodechar{≫}{\ensuremath{\gg}}
\newunicodechar{≪}{\ensuremath{\ll}}
\newunicodechar{∅}{\ensuremath{\emptyset}}
\newunicodechar{⊆}{\ensuremath{\subseteq}}
\newunicodechar{⊂}{\ensuremath{\subset}}
\newunicodechar{∩}{\ensuremath{\cap}}
\newunicodechar{⋂}{\ensuremath{\cap}}
\newunicodechar{∪}{\ensuremath{\cup}}
\newunicodechar{⋃}{\ensuremath{\cup}}
\newunicodechar{⊎}{\ensuremath{\uplus}}
\newunicodechar{∈}{\ensuremath{\in}}
\newunicodechar{∉}{\ensuremath{\not\in}}
\newunicodechar{⊤}{\ensuremath{\top}}
\newunicodechar{⊥}{\ensuremath{\bot}}
\newunicodechar{₀}{\ensuremath{_0}}
\newunicodechar{₁}{\ensuremath{_1}}
\newunicodechar{₂}{\ensuremath{_2}}
\newunicodechar{₃}{\ensuremath{_3}}
\newunicodechar{₄}{\ensuremath{_4}}
\newunicodechar{₅}{\ensuremath{_5}}
\newunicodechar{₆}{\ensuremath{_6}}
\newunicodechar{₇}{\ensuremath{_7}}
\newunicodechar{₈}{\ensuremath{_8}}
\newunicodechar{₉}{\ensuremath{_9}}
\newunicodechar{⁰}{\ensuremath{^0}}
\newunicodechar{¹}{\ensuremath{^1}}
\newunicodechar{²}{\ensuremath{^2}}
\newunicodechar{³}{\ensuremath{^3}}
\newunicodechar{⁴}{\ensuremath{^4}}
\newunicodechar{⁵}{\ensuremath{^5}}
\newunicodechar{⁶}{\ensuremath{^6}}
\newunicodechar{⁷}{\ensuremath{^7}}
\newunicodechar{⁸}{\ensuremath{^8}}
\newunicodechar{⁹}{\ensuremath{^9}}
\newunicodechar{𝔹}{\ensuremath{\mathbb{B}}}
\newunicodechar{ℝ}{\ensuremath{\mathbb{R}}}
\newunicodechar{ℕ}{\ensuremath{\mathbb{N}}}
\newunicodechar{ℂ}{\ensuremath{\mathbb{C}}}
\newunicodechar{ℚ}{\ensuremath{\mathbb{Q}}}
\newunicodechar{𝕋}{\ensuremath{\mathbb{T}}}
\newunicodechar{𝕏}{\ensuremath{\mathbb{X}}}
\newunicodechar{ℤ}{\ensuremath{\mathbb{Z}}}
\newunicodechar{✓}{\checkmark}
\newunicodechar{✗}{\ensuremath{\times}}
\newunicodechar{◊}{\ensuremath{\lozenge}}
\newunicodechar{□}{\ensuremath{\square}}
\newunicodechar{𝓐}{\ensuremath{\mathcal{A}}}
\newunicodechar{𝓑}{\ensuremath{\mathcal{B}}}
\newunicodechar{𝓒}{\ensuremath{\mathcal{C}}}
\newunicodechar{𝓓}{\ensuremath{\mathcal{D}}}
\newunicodechar{𝓔}{\ensuremath{\mathcal{E}}}
\newunicodechar{𝓕}{\ensuremath{\mathcal{F}}}
\newunicodechar{𝓖}{\ensuremath{\mathcal{G}}}
\newunicodechar{𝓗}{\ensuremath{\mathcal{H}}}
\newunicodechar{𝓘}{\ensuremath{\mathcal{I}}}
\newunicodechar{𝓙}{\ensuremath{\mathcal{J}}}
\newunicodechar{𝓚}{\ensuremath{\mathcal{K}}}
\newunicodechar{𝓛}{\ensuremath{\mathcal{L}}}
\newunicodechar{𝓜}{\ensuremath{\mathcal{M}}}
\newunicodechar{𝓝}{\ensuremath{\mathcal{N}}}
\newunicodechar{𝓞}{\ensuremath{\mathcal{O}}}
\newunicodechar{𝓟}{\ensuremath{\mathcal{P}}}
\newunicodechar{𝓠}{\ensuremath{\mathcal{Q}}}
\newunicodechar{𝓡}{\ensuremath{\mathcal{R}}}
\newunicodechar{𝓢}{\ensuremath{\mathcal{S}}}
\newunicodechar{𝓣}{\ensuremath{\mathcal{T}}}
\newunicodechar{𝓤}{\ensuremath{\mathcal{U}}}
\newunicodechar{𝓥}{\ensuremath{\mathcal{V}}}
\newunicodechar{𝓦}{\ensuremath{\mathcal{W}}}
\newunicodechar{𝓧}{\ensuremath{\mathcal{X}}}
\newunicodechar{𝓨}{\ensuremath{\mathcal{Y}}}
\newunicodechar{𝓩}{\ensuremath{\mathcal{Z}}}
\newunicodechar{…}{\ensuremath{\ldots}}
\newunicodechar{∗}{\ensuremath{\ast}}
\newunicodechar{⊢}{\ensuremath{\vdash}}
\newunicodechar{⊧}{\ensuremath{\models}}
\newunicodechar{′}{\ensuremath{'}}
\newunicodechar{″}{\ensuremath{''}}
\newunicodechar{‴}{\ensuremath{'''}}
\newunicodechar{∥}{\ensuremath{\|}}
\newunicodechar{⊕}{\ensuremath{\oplus}}
\newunicodechar{⁺}{\ensuremath{^+}}
\newunicodechar{⊇}{\ensuremath{\supseteq}}
\newunicodechar{∘}{\ensuremath{\circ}}
\newunicodechar{∙}{\ensuremath{\cdot}}
\newunicodechar{⋅}{\ensuremath{\cdot}}
\newunicodechar{≈}{\ensuremath{\approx}}
\newunicodechar{×}{\ensuremath{\times}}
\newunicodechar{∞}{\ensuremath{\infty}}


==> macros.tex <==
%%% Theorem-like environments
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \newtheorem{theorem}{Theorem}[section]%
% \newtheorem{lemma}[theorem]{Lemma}%
% \newtheorem{corollary}[theorem]{Corollary}%
% \newtheorem{proposition}[theorem]{Proposition}%
% 
% \newtheorem{definition}[theorem]{Definition}%
% \newtheorem{example}[theorem]{Example}%
% \newtheorem{remark}[theorem]{Remark}%
% \newtheorem{notation}[theorem]{Notation}%

%\crefname{proposition}{Prop.\@\!}{Propositions}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Conditionals
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% If/then check for empty strings (requires xifthen for \isempty)
\newcommand{\ifempty}[3]{%
  \ifthenelse{\isempty{#1}}{#2}{#3}%
}%

\makeatletter
\newcommand\footnoteref[1]{\protected@xdef\@thefnmark{\ref{#1}}\@footnotemark}
\makeatother

%%%% MACROS 
\newcommand{\RedG}{\Longrightarrow}
\newcommand{\dlsqb}{[\![}
\newcommand{\drsqb}{]\!]}

\renewcommand{\l}{l}
%\newcommand{\T}{{\mathsf T}}
\newcommand{\T}{T}
\newcommand{\R}{R}
\renewcommand{\S}{S}


\newcommand{\rulename}[1]{\text{\textnormal{\small[\textsc{#1}]}}}

\newcommand{\PGCD}{\textsf{PGCD}\xspace}

%%%%%%%%%%%%%%%%%%%%%%
%%%     NAMES      %%%
%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\s}{s}
\newcommand{\pp}{{\roleP}}
\newcommand{\pq}{{\roleQ}}
\newcommand{\pr}{{\roleR}}
\newcommand{\ps}{{\roleS}}
\newcommand{\q}{\pq}
%\newcommand{\pp}{{\sf p}}
%\newcommand{\pq}{{\sf q}}
%\newcommand{\pr}{{\sf r}}
%\newcommand{\ps}{{\sf s}}
%\newcommand{\q}{\pq}
\newcommand{\e}{\kf{e}}
\newcommand{\x}{x}
\newcommand{\y}{y}
\newcommand{\bfx}{\mathbf{x}}
\newcommand{\bfy}{\mathbf{y}}
\newcommand{\bfzero}{\mathbf{0}}
\newcommand{\bfone}{\mathbf{1}}
\newcommand{\h}{h}
%\newcommand{\val}{\kf{v}}
\newcommand{\val}{v} % changed 
\newcommand{\valn}{\kf{n}}
\newcommand{\valr}{\kf{i}}
\newcommand{\vali}{\valr}
\newcommand{\valb}{\kf{b}}
\newcommand{\SEP}{\ensuremath{~~\mathbf{|\!\!|}~~ }}
\newcommand{\kf}[1]{\ensuremath{\mathsf{#1}}}
\newcommand{\ma}{\ensuremath{\mathit{a}}}
\newcommand{\mb}{\ensuremath{\mathit{b}}}
\newcommand{\mc}{\ensuremath{\mathit{c}}}

%   \newcommand{\G}{\ensuremath{{\sf G}}}
\newcommand{\Gvti}[5]{\ensuremath{#1\to#2:\{#3_i({#4}_i). #5_i \}_{i \in I}}}
\newcommand{\Gvtj}[5]{\ensuremath{#1\to#2:\{#3_j({#4}_j). #5_j \}_{j \in J}}}
\newcommand{\Gvtk}[5]{\ensuremath{#1\to#2:\{#3_k({#4}_k). #5_k \}_{k \in K}}}
\newcommand{\GvtiSet}[6]{\ensuremath{#1\to#2:\{#3_i({#4}_i). #5_i \}_{i \in {#6}}}}
\newcommand{\GvtlSet}[6]{\ensuremath{#1\to#2:\{#3_l({#4}_l). #5_l \}_{l \in {#6}}}}
\newcommand{\GvtmSet}[6]{\ensuremath{#1\to#2:\{#3_m({#4}_m). #5_m \}_{m \in {#6}}}}
\newcommand{\Gvt}[5]{\ensuremath{#1\to#2: #3({#4}). #5 }}
\newcommand{\GvtPre}[4]{\ensuremath{#1\to#2: #3({#4})}}
\newcommand{\GvtIdx}[6]{\ensuremath{#1\to#2: \{#3({#4}). #5\}_{#6}}}
\newcommand{\ty}{\mathbf{t}}
\newcommand{\GvtPair}[3]{\ensuremath{#1\to#2: \{#3\}_{i\in I}}}

\newcommand{\minimal}{\ensuremath{\mathsf{minimal}}}
%\newcommand{\exclude}{\ensuremath{\mathsf{PC}}}
\newcommand{\exclude}{\ensuremath{\mathbb P}}
\newcommand{\Sy}{\ensuremath{\mathcal S}}
%\newcommand{\N}{\ensuremath{\mathcal M}}
\newcommand{\N}{M}
\newcommand{\M}{\ensuremath{\mathcal M}}

\newcommand{\pa}[2]{#1 \triangleleft  #2}
\newcommand{\set}[1]{\{#1\}}
\newcommand{\powerset}[1]{\mathcal{P}(#1)}
\newcommand{\eval}[2]{#1 \downarrow #2}
\newcommand{\evalState}[3]{#1 \downarrow_{#3} #2}
\newcommand{\true}{\kf{true}}
\newcommand{\false}{\kf{false}}
\newcommand{\ns}[1]{{}^*{#1}}

\newcommand{\myrule}[3]{\begin{prooftree} #1 \justifies   #2   \using{\rln{#3}} \end{prooftree}}
\newcommand{\rln}[1]{\textsc{#1}}
\newcommand{\der}[3]{ #1 \vdash   #2  :#3}
\newcommand{\pro}[3]{ #1 \upharpoonright_#2 #3}
\newcommand{\CP}[1]{ {\mathcal P}\!\left({#1}\right)}
\newcommand{\CG}[2]{ {\mathcal G}(#1,#2)}
\newcommand{\CGZ}[3]{ {\mathcal G}_0(#1,#2,#3)}
\newcommand{\res}{\setminus}
\newcommand{\rem}{\bbslash}
\newcommand{\CC}[1]{ {\mathcal C}[#1]}

\newcommand{\inout}[1]{{\mathtt {actions}}(#1)}
%%%%%%%%%%%%%%%%%%%%%%
%%% FUNCTIONS      %%%
%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\participant}[1]{\mathtt{pt}\{#1\}}
\newcommand{\pn}[1]{\mathtt{pn}(#1)}
\newcommand{\pnin}[1]{\mathtt{pn}_?(#1)}
\newcommand{\pnout}[1]{\mathtt{pn}_!(#1)}
\newcommand{\proj}[2]{ #1 \upharpoonright_{#2}}
\newcommand{\projt}[2]{{#1}{\upharpoonright}{#2}}
\newcommand{\sub}[2]{\set{#1/#2}}

\newcommand{\exprt}[2]{\mathtt{expression}(#1,#2)}
\newcommand{\valt}[1]{\mathtt{value}(#1)}

%%%%%%%%%%%%%%%%%%%%%%
%%% PROCESSES      %%%
%%%%%%%%%%%%%%%%%%%%%%

%\newcommand{\ENCan}[1]{\langle#1\rangle}
\newcommand{\MP}{M}
\newcommand{\motion}[2]{\kf{#1}\ENCan{#2}}
\newcommand{\Gmotion}[3]{\kf{#1}\ENCan{#2}.{#3}}
\newcommand{\Lmotion}[3]{\kf{#1}\ENCan{#2}.{#3}}
\newcommand{\inmotion}[4]{#1 ? \kf{#2}\ENCan{#3}.#4}
\newcommand{\new}[1]{(\nu#1)}
\newcommand{\procin}[3]{#1 ?  #2 .#3}
\newcommand{\procoutabb}[3]{#1 ! #2. #3}
\newcommand{\procout}[4]{#1 ! #2\ENCan{#3}. #4}
\newcommand{\procdag}[3]{#1 \dagger  #2 .#3}
\newcommand{\procddag}[3]{#1 \dagger #2. #3}
\newcommand{\error}{\kf{error}}
\newcommand{\PP}{\ensuremath{{P}}}
%\newcommand{\PC}{\ensuremath{\mathsf{PC}}}
\newcommand{\PC}{\ensuremath{\Bbb P}}
\newcommand{\plays}{\ensuremath{\triangleleft{}}}
\newcommand{\proc}[3]{\ensuremath{\langle{#2,#3\mathsf{;}\, #1}\rangle}}
\newcommand{\geom}[1]{\ensuremath{\mathsf{geom}\left({#1}\right)}}
\newcommand{\parcomp}{\ensuremath{~|~}}

\newcommand{\Q}{\ensuremath{Q}}
\newcommand{\procwait}[2]{\kf{wait}~ (\motion{dt}{#1})\; \{~#2 \}}
\newcommand{\procwhile}[3]{\kf{while}~ (#1,\;#2).~#3}
\newcommand{\cond}[3]{\kf{if}~ #1 ~\kf{then} ~#2 ~\kf{else}~#3}
\newcommand{\ccond}[2]{\kf{if}~ #1 ~\kf{then} ~#2 ~\kf{else}}
%\newcommand{\condML}[4]{\kf{if}~ #1 ~\kf{then} ~#2 {\phantom{#4}}\kf{else}~#3}
\newcommand{\inact}{\ensuremath{\mathbf{0}}}
\newcommand{\internal}{\oplus}
\newcommand{\external}{+}
\newcommand{\co}[1]{\mathtt{coherent}\{#1\}}
\newcommand{\emptyqueue}{\epsilon}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% ENDPOINT and other TYPES %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\tend}{\mathtt{end}}
\newcommand{\tunit}{\mathtt{unit}}
\newcommand{\tbool}{\mathtt{bool}}
\newcommand{\tnat}{\mathtt{nat}}
\newcommand{\tint}{\mathtt{int}}
\newcommand{\treal}{\mathtt{real}}
\newcommand{\tstring}{\mathtt{string}}
\newcommand{\tin}[3]{#1?#2(#3)}
\newcommand{\tout}[3]{#1!#2(#3)}
\newcommand{\tdag}[3]{#1\dagger #2(#3)}
\newcommand{\tddag}[3]{#1\ddagger #2 (#3)}
\newcommand{\tinternal}{\vee}
\newcommand{\texternal}{\wedge}

\newcommand{\lin}{part}
\newcommand{\lout}{lab}

\renewcommand{\S}{S}
\newcommand{\queue}{\mathtt{queue}}
\newcommand{\lts}[1]{\xrightarrow{#1}}
\newcommand{\redG}[4]{#1\setminus#2\xrightarrow#3#4}
\newcommand{\redGM}[2]{#1\setminus#2}
\newcommand{\redGequiv}[2]{#1 \rightsquigarrow #2}
\newcommand{\redastGequiv}[2]{#1 \rightsquigarrow^\ast #2}
\newcommand{\SortI}[2]{ {#1}_{#2}}
%%%%%%%%%%%%%%%%%%%%%%
%%% CONTEXTS
%%%%%%%%%%%%%%%%%%%%%%

%\newcommand{\Ghole}{[~]}
\newcommand{\context}{\mathcal{C}}
\newcommand{\Econtext}{\mathcal{E}}

%%% Global type contexts
\newcommand{\Gctx}[1][]{\ifempty{#1}{\textswab{G}}{\textswab{G}_{#1}}}%
\newcommand{\GctxHole}[1]{[\;]^{#1}}%
\newcommand{\GctxApp}[4]{{#1}[{#2}]^{#3}_{#4}}%

%%%%%%%%%%%%%%%%%%%%%%
%%%    RELATIONS   %%%
%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\enm}[1]{\ensuremath{#1}\xspace}
\newcommand{\trans}[1]{\enm{\stackrel{#1}{\longrightarrow}}}
\newcommand{\motiontrans}[2]{\enm{\stackrel{\motion{#1}{#2}}{\longrightarrow}}}
\newcommand{\subt}{\leqslant}
\newcommand{\subta}{\mathrel{\leqslant_a}}
\newcommand{\subs}{\leq\vcentcolon}
\newcommand{\nsubs}{\not\leq\vcentcolon}
\newcommand{\red}{\longrightarrow}
\newcommand{\nsubt}{\not\trianglelefteq}
\newcommand{\someRel}[1][]{\mathrel{\ifempty{#1}{\mathcal{R}}{\mathcal{R}_{#1}}}}%
\newcommand{\someReli}[1][]{\mathrel{\ifempty{#1}{\mathcal{R}'}{\mathcal{R}'_{#1}}}}%

%%%%%%%%%%%%%%%%%%%%%%
%%%%    FUNCTIONS    %
%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\fsqrt}[1]{{\tt neg}(#1)}
\newcommand{\fneg}{\fsqrt}
\newcommand{\fsucc}[1]{{\tt succ}(#1)}
\newcommand{\sbj}[1]{{\tt subj}(#1)}
\newcommand{\fail}[1]{{\tt fail}(#1)}
\newcommand{\stuck}[1]{{\tt stuck}\!\left({#1}\right)}
\newcommand{\dual}[1]{\overline #1}

\newcommand{\fpv}[1]{\mathit{fpv}(#1)}

\newcommand{\dom}[1]{\operatorname{dom}({#1})}
\newcommand{\ran}[1]{\operatorname{ran}({#1})}
\newcommand{\subst}[2]{\{\nicefrac{#1}{#2}\}}%

%%%%%%%%%%%%%%%%%%
%%% Type trees %%%
%%%%%%%%%%%%%%%%%%
\newcommand{\contTag}{{\,\mathsf{C}}}%
\newcommand{\payloadTag}{{\,\mathsf{P}}}%
\newcommand{\ttreeSym}{\mathcal{T}}%
\newcommand{\ttree}[1]{\operatorname{\ttreeSym}\!\left({#1}\right)}%
%\newcommand{\tsynt}[1]{\mathbb{#1}}%
\newcommand{\tsynt}[1]{\mathbb{#1}}%
\newcommand{\ts}{\tsynt}%


%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\cinferrule}[3][]{
  \mprset{fraction={===},
  fractionaboveskip=0.2ex,
  fractionbelowskip=0.4ex}
  \inferrule[#1]{#2}{#3}
}

\newcommand{\ccinferrule}[3][]{
  \mprset{fraction={===},
  fractionaboveskip=1.8ex,
  fractionbelowskip=0.4ex}
  \inferrule[#1]{#2}{#3}
}

\newcommand{\AContext}{\mathcal{A}}
\newcommand{\BContext}{\mathcal{B}}
\newcommand{\AContextf}[1]{\AContext [ #1 ]}
\newcommand{\AContextfp}[1]{\AContext' [ #1 ]}
\newcommand{\AContextfi}[2]{\AContext_#1 [ #2 ]}
\newcommand{\AContextfip}[2]{\AContext'_#1 [ #2 ]}
%\newcommand{\I}{\bigwedge\!\!\!\!\bigwedge}
\newcommand{\I}{\bigsqcap}%

%%%%%%%%%%%%%%%%%%%%%%
%%%%%%  COLORS       %
%%%%%%%%%%%%%%%%%%%%%%
\definecolor{ceca}{rgb}{1,0.5,0}
\newcommand{\sj}[1]{{\color{ceca}{#1}}}

\newcommand{\SUB}[3]{{\mathcal S}(#1,#2,#3)}
\newcommand{\Gvtir}[5]{\ensuremath{#1\to#2:\{#3_i({#4}_i). \redG{#5_i}\pp\ell\q \}_{i \in I}}}
%\newcommand{\Gvti}[5]{\ensuremath{#1\to#2:\{#3_i({#4}_i). #5_i \}_{i \in I}}}

\newcommand{\wtp}[3]{
      #1 \vdash   #2 \triangleright #3  
}


\newcommand{\Alice}{\ensuremath{\mathtt{Alice}}}
\newcommand{\Bob}{\ensuremath{\mathtt{Bob}}}
\newcommand{\Carol}{\ensuremath{\mathtt{Carol}}}
\newcommand{\ENCan}[1]{\langle #1 \rangle}
\newcommand{\GS}[4]{\TO{#1}{#2}\colon \!{#3}(#4)}
\newcommand{\GSS}[3]{\TO{#1}{#2}\colon \!{#3}}
%\newcommand{\GS}[3]{\TO{#1}{#2}\colon \!\ENCan{#3}}
\newcommand{\Nat}{\kf{nat}}
\newcommand{\TO}[2]{#1\to #2}

\newcommand{\merger}{\bigsqcap}

\newcommand{\subtree}{{\tt subterm}}
\newcommand{\measure}{{\tt measure}}

\newcommand{\fv}{\mathrm{fv}}
\newcommand{\vars}{\mathrm{vars}}
\newcommand{\duration}{\mathit{duration}}


% from ICCPS paper

\newcommand{\cartPosition}{{\ensuremath{\mathbf{p}_\Cart}}}
\newcommand{\carriertPosition}{{\ensuremath{\mathbf{p}_\Carrier}}}
\newcommand{\cartOrientation}{{\ensuremath{\mathbf{r}_\Cart}}}
\newcommand{\cartSpeed}{{\ensuremath{\mathbf{s}_\Cart}}}
\newcommand{\cartPayload}{{\ensuremath{\mathbf{w}_{\mathbf{obj}}}}}
\newcommand{\pre}{\ensuremath{\mathrm{Pre}\xspace}}
\newcommand{\post}{\ensuremath{\mathrm{Post}\xspace}}
\newcommand{\invariant}{\ensuremath{\mathrm{Inv}\xspace}}
\newcommand{\pred}{\mathcal{P}}
\newcommand{\resource}{{{\mathit{rsrc}}}}
\newcommand{\vvars}{{\mathit{Var}}}

\newcommand{\prj}[2]{#1|_{#2}}
\newcommand{\step}[3]{#1 \xrightarrow{#2} #3}
\newcommand{\mapstep}[3]{#1 \xmapsto{#2} #3}
\newcommand{\id}{\ensuremath{\mathsf{id}}\xspace}
\newcommand{\dt}{\ensuremath{\mathsf{dt}}\xspace}
\newcommand{\clock}{\ensuremath{\mathsf{clock}}\xspace}


\definecolor{dtsessColor}{rgb}{0.8, 0.0, 0.0}%
\newcommand{\dtsessCol}[1]{{\color{dtsessColor}#1}}%
\newcommand{\dtsess}{\dtsessCol{\mathsf{dt}}}%

\newcommand{\leftmost}{\ensuremath{\mathsf{left}\xspace}}
\newcommand{\disjoint}{\ensuremath{\mathsf{disjoint}\xspace}}
\newcommand{\compatible}{\ensuremath{\mathsf{compatible}\xspace}}

\def\set#1{\{#1 \}}
\def\tuple#1{\langle #1 \rangle }
\def\dbrkts#1{[\![ #1 ]\! ]}

\newcommand{\sethree}{\mathit{SE}(3)}
\newcommand{\sothree}{\mathit{SO}(3)}

\newcommand{\comp}[4]{#1 \lhd_{#2, #3} #4}      % attached composition
%\newcommand{\sstore}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\sstore}[1]{\ensuremath{\vecFmt{#1}}}
\newcommand{\rbtstate}[4]{\ensuremath{\tuple{#2,#3,#4\mid\;#1}}} % robot state
\newcommand{\htriple}[3]{\ensuremath{\{#1\}#2\{#3\}}} % Hoare triple
\newcommand{\judgement}[2]{\ensuremath{ #1 ~\vdash~(#2)}}
% \newcommand{\judgement}[2]{\ensuremath{\vdash #1 ~\text{\textbf{sat}}~(#2)}}
\newcommand{\pjudgement}[2]{\ensuremath{\vdash #1 ~\text{\textbf{psat}}~(#2)}}
\newcommand{\timestep}{{\ddagger}}
\newcommand{\instantaneous}{{\mathsf{\lightning}}}
\newcommand{\delayed}{{\mathsf{\rightsquigarrow}}}

\newcommand{\sexpr}{\ensuremath{\mathit{expr}}\xspace}
\newcommand{\smp}{\ensuremath{\mathit{mp}}\xspace}
\newcommand{\sskip}{\ensuremath{\texttt{\textbf{skip}}}\xspace}
\newcommand{\sdone}{\ensuremath{\texttt{\textbf{end}}}\xspace}
\newcommand{\sabort}{\ensuremath{\texttt{\textbf{abort}}}\xspace}
%\newcommand{\ssend}{\ensuremath{\mathbf{send}}\xspace}
\newcommand{\ssend}{\ensuremath{\texttt{\textbf{send}}}\xspace}
\newcommand{\srecv}{\ensuremath{\texttt{\textbf{receive}}}\xspace}
\newcommand{\site}[3]{\ensuremath{\texttt{\textbf{if}} ~ #1 ~ \texttt{\textbf{then}} ~ #2 ~ \texttt{\textbf{else}} ~ #3}}
\newcommand{\swhile}[2]{\ensuremath{\texttt{\textbf{while}} ~ #1 ~ \texttt{\textbf{do}} ~ #2}}
\newcommand{\sflow}[2]{\ensuremath{\texttt{\textbf{flow}} ~ #1 ~ \texttt{\textbf{do}} ~ #2}}
\newcommand{\sder}[2]{\ensuremath{#1 ~ +\hspace{-0.8ex}= #2 \cdot \dt}}
\newcommand{\msgSend}[2]{\ensuremath{#1!#2}}
\newcommand{\msgRecv}[2]{\ensuremath{#1?#2}}
\newcommand{\ichoice}[2]{\ensuremath{#1 ⊕ #2}}
\newcommand{\echoice}[2]{\ensuremath{#1 {\bf \,\&\,} #2}}

\newcommand{\unitv}[1]{\mathbf{u}_{#1}}
\newcommand{\world}{{\mathcal{W}}}
\newcommand{\st}[1]{{\mathit{st}(#1)}}

\newcommand{\FP}{\ensuremath{\mathit{FP}}}
\newcommand{\attachedSeparation}{\ensuremath{*_{\lhd}}}

\newcommand{\myparagraph}[1]{\paragraph{\bf #1}}

\newcommand{\vc}{{\color{roleColor}\roleFmt{vc}}}
\definecolor{vecColor}{rgb}{0.5, 0.0, 0.0}%
\newcommand{\vecCol}[1]{{\color{vecColor}#1}}%
\newcommand{\conCol}[1]{{\color{blue}#1}}%
%\newcommand{\vecSet}{\roleCol{\mathbb{V}}}%
%\newcommand{\vecFmt}[1]{\boldsymbol{\vecCol{\mathtt{#1}}}}%
\newcommand{\vecFmt}[1]{\boldsymbol{\mathtt{#1}}}%

\newcommand{\fs}{\boldsymbol{\vecCol{\mathtt{e}}}}%
\newcommand{\idfs}{\boldsymbol{\vecCol{\mathtt{id}}}}%
\newcommand{\pToc}{\mu^{-1}}
\newcommand{\cTop}{\mu}
%\newcommand{\pToc}{\ensuremath{\boldsymbol{\vecCol{\mathtt{e}^{-1}}}}\xspace}  % parent to child
%\newcommand{\cTop}{\ensuremath{\fs}\xspace}       % child to parent
%\newcommand{\con}{\boldsymbol{\conCol{\mathbb{c}}}}%
%\newcommand{\con}{\boldsymbol{\conCol{\textfrak{R}}}}%
%\newcommand{\con}{\boldsymbol{\conCol{\Re}}}%
\newcommand{\con}{{\boldsymbol{\conCol{\mathbbmtt{c}}}}}%
\newcommand{\obj}[1]{\mathsf{obj}({#1})}%
\newcommand{\shiftTo}[1]{\con_{\rightarrow #1}}
\newcommand{\shiftFromTo}[2]{\con_{#1 \rightarrow #2}}
\newcommand{\freevars}{\ensuremath{\mathit{fv}}}
\newcommand{\refines}{\ensuremath{\preceq}}

\def\Cart{{\color{roleColor}{\mathsf{Cart}}}}
\def\Env{{\color{roleColor}{\mathsf{Env}}}}
\def\Crane{{\color{roleColor}{\mathsf{Crane}}}}
\def\Trolley{{\color{roleColor}{\mathsf{Trolley}}}}
\def\Arm{{\color{roleColor}{\mathsf{Arm}}}}
\def\Producer{{\color{roleColor}{\mathsf{Prod}}}}
\def\Red{{\color{roleColor}{\mathsf{RRobot}}}}
\def\Green{{\color{roleColor}{\mathsf{GRobot}}}}

\def\FOLD{\mathit{fold}}
\def\UNFOLD{\mathit{unfold}}
\def\START{\mathit{start}}
\def\GREEN{\mathit{green}}
\def\RED{\mathit{red}}
\def\OK{\mathit{ok}}
\def\FREE{\mathit{free}}
\def\GRAB{\mathit{grab}}
\def\DROP{\mathit{drop}}
\def\PICK{\mathit{pick}}
\def\ARRIVE{\mathit{arrive}}
\def\READY{\mathit{ready}}
\def\DONE{\mathit{done}}

\def\FOLDM{\mathsf{c\_fold}}
\def\UNFOLDM{\mathsf{c\_unfold}}
\def\GRIPM{\mathsf{c\_grip}}
\def\GRABM{\mathsf{c\_grab}}
\def\IDLEM{\mathsf{m\_idle}}
\def\MOVEM{\mathsf{m\_move}}
\def\IDLEMC{\mathsf{c\_idle}}
\def\IDLEMT{\mathsf{t\_idle}}
\def\WORKM{\mathsf{work}}
\def\PICKM{\mathsf{pick}}
\def\PLACEM{\mathsf{place}}

\definecolor{ruleColor}{rgb}{0.1, 0.3, 0.1}%
\definecolor{groundColor}{rgb}{0.38, 0.25, 0.32}%

%\definecolor{roleColor}{rgb}{0.5, 0.0, 0.0}%
\definecolor{roleColor}{rgb}{0.1, 0.3, 0.1}%
\newcommand{\roleCol}[1]{{\color{roleColor}#1}}%
\newcommand{\roleSet}{\roleCol{\mathbb{R}}}%
\newcommand{\roleFmt}[1]{\boldsymbol{\roleCol{\mathtt{#1}}}}%
\newcommand{\roleP}[1][]{%
  \ifempty{#1}{{\color{roleColor}\roleFmt{p}}}{{\color{roleColor}\roleFmt{p}_{#1}}}%
}%
\newcommand{\pc}{{\roleP}}
\newcommand{\roleVar}[1][]{%
  \ifempty{#1}{{\color{roleColor}\roleFmt{x}}}{{\color{roleColor}\roleFmt{x}_{#1}}}%
}%
\newcommand{\procvar}{{\roleVar}}
\newcommand{\rolePi}[1][]{%
  \ifempty{#1}{{\color{roleColor}\roleFmt{p}'}}{{\color{roleColor}\roleFmt{p}'_{#1}}}%
}%
\newcommand{\roleQ}[1][]{%
  \ifempty{#1}{{\color{roleColor}\roleFmt{q}}}{{\color{roleColor}\roleFmt{q}_{#1}}}%
}%
\newcommand{\roleQi}[1][]{%
  \ifempty{#1}{{\color{roleColor}\roleFmt{q}'}}{{\color{roleColor}\roleFmt{q}'_{#1}}}%
}%
\newcommand{\roleR}[1][]{%
  \ifempty{#1}{{\color{roleColor}\roleFmt{r}}}{{\color{roleColor}\roleFmt{r}_{\!#1}}}%
}%
\newcommand{\roleRi}[1][]{%
  \ifempty{#1}{{\color{roleColor}\roleFmt{r}'}}{{\color{roleColor}\roleFmt{r}'_{\!#1}}}%
}%
\newcommand{\roleRii}[1][]{%
  \ifempty{#1}{{\color{roleColor}\roleFmt{r}''}}{{\color{roleColor}\roleFmt{r}''_{\!#1}}}%
}%
\newcommand{\roleS}[1][]{%
  \ifempty{#1}{{\color{roleColor}\roleFmt{s}}}{{\color{roleColor}\roleFmt{s}_{\!#1}}}%
}%
\newcommand{\roleSi}[1][]{%
  \ifempty{#1}{{\color{roleColor}\roleFmt{s}'}}{{\color{roleColor}\roleFmt{s}'_{\!#1}}}%
}%
\newcommand{\roleSii}[1][]{%
  \ifempty{#1}{{\color{roleColor}\roleFmt{s}''}}{{\color{roleColor}\roleFmt{s}''_{\!#1}}}%
}%

\newcommand{\GL}{\ensuremath{{\sf G}}}
\newcommand{\GLPre}{\ensuremath{g}}
\newcommand{\TLPre}{\ensuremath{T}}
% \newcommand{\GLPAR}{\ensuremath{\Vert}}
\newcommand{\GLPAR}{\ensuremath{\ast}}
\newcommand{\SL}{\ensuremath{{\sf S}}}
\newcommand{\NUL}{\ensuremath{\epsilon}}

\newcommand{\Sec}{{Sec.}}
\newcommand\AT{\text{\small{\tt @}}}
%\newcommand\ASENDPC{\mathit{PC}}
\newcommand\ASENDPC{\vec{\pc}}



==> packages.tex <==
\usepackage[utf8]{inputenc}
% Simplified management of FIXMEs
\usepackage[nomargin,inline,index,status=draft]{fixme}
%% Setup FIXME style and register authors of comments
\fxusetheme{colorsig}%
\FXRegisterAuthor{fxNY}{anfxNY}{\underline{\textbf{NY}}}%
\FXRegisterAuthor{fxRM}{anfxRM}{\underline{\textbf{RM}}}%
\FXRegisterAuthor{fxDZ}{anfxDZ}{\underline{\textbf{DZ}}}%

\usepackage{microtype}


%\usepackage{makeidx}
\usepackage{xspace}
\usepackage{bbm}
\usepackage{color}
\usepackage[inline,shortlabels]{enumitem}% Custimisable enumerations
%\usepackage[mathcal]{euscript}% Nicer mathcal font
\usepackage{yfonts}% Nicer \mathfrak font
\usepackage{stmaryrd}
%\input{macros}
\usepackage{mathpartir}
%\usepackage{amsmath,amssymb,amsthm}
\usepackage{nicefrac}% Nice fractions
\usepackage{thmtools}% For restatable
\usepackage{prooftree}
\usepackage{mathtools}
\usepackage{booktabs} 
\usepackage{xspace}
\usepackage{bold-extra}
\usepackage{euscript} [mathcal]
% In order to save space or manage large tables or figures in a
% landcape-like text, you can use the rotating and pdflscape
% packages. Uncomment the desired from the below.
%
% \usepackage{rotating}
% \usepackage{pdflscape}


\usepackage{subcaption} %% For complex figures with subfigures/subcaptions
                        %% http://ctan.org/pkg/subcaption
\usepackage{multirow}                        
\usepackage{wrapfig}                        

\usepackage{xifthen}% Conditionals
\usepackage[all]{xy}% Diagrams

% Maybe we will want to remove the following lines in the final version
\usepackage{hyperref}% Load cleveref last!
\hypersetup{final}% Needed to generate hyperlinks even in draft mode

\usepackage{tikz}
\usetikzlibrary{patterns}



\usepackage{todonotes}
\newcommand\RM[1]{\todo[color=red!20!white]{RM, #1}}
\newcommand\NY[1]{\todo[color=violet!20!white]{NY, #1}}
\newcommand\DZ[1]{\todo[color=cyan!20!white]{DZ, #1}}
\newcommand\RMi[1]{\todo[color=white,inline]{\textcolor{red}{RM, #1}}}
\newcommand\NYi[1]{\todo[color=white,inline]{\textcolor{violet}{NY, #1}}}
\newcommand\DZi[1]{\todo[color=white,inline]{\textcolor{cyan}{DZ, #1}}}

% Long/proceeding version
\usepackage{etoolbox}
\newtoggle{full}




==> proof.tex <==
\section{Motion Choreographies} 
\label{sec:proof-system}
In this section, we develop a multiparty session typing discipline to
prove communication safety and collision freedom.
% There are two difficulties in lifting the proof system for motion primitives to the concurrent setting.
% First, our semantics is truly concurrent as time is global in the system and every component evolves in time at the same time.
% Thus, we check that all concurrent executions of motion primitives
% specified in the global type are \emph{compatible}: 
% the assumptions of all components are simultaneously satisfied and there exists a partition of space so that
% the footprints of the motion primitives do not intersect.
% 
Our session types extend usual multiparty session types by introducing
new operators and by reasoning
about joint motion in real-time. Moreover, as message exchanges can be a proxy to exchange permissions for motion primitives, 
our types have predicates as guards in order to model permissions for motion primitives.
% During type checking, these predicates must be transformed through reference frame transformations.

\subsection{Global Types with Motions and Predicates}
\label{subsec:global}
We start with a choreography given as a \emph{global type}. 
The global type constrains the possible sequences of messages and controller actions that may occur in any execution of the system.
We extend \cite{ECOOP19} by 
framing and predicate refinements, together with 
separation conjunctions. 

{\em Sorts}, ranged over by $\SL,$ are used to define base types:
\[\SL \quad::=\quad \tunit \SEP \treal \SEP \text{\sf{point}}(ℝ³) \SEP \text{\sf{vector}} \SEP 
% (ℝ³)\SEP ℝ^{4\times 4} \SEP 
	\ldots \SEP \SL\times \SL\]
A \emph{predicate refinement} is of the form $\set{\nu : \SL\mid \pred}$, where 
$\nu$ is a \emph{value variable}
not appearing in the program, $\SL$ a sort, and 
$\pred$ a Boolean predicate.
Intuitively, a predicate refinement represents assumptions on the 
state of the sender and the communicated value to the recipient.
We write $\SL$ as abbreviation for $\set{\nu: \SL\mid\true}$ and
$\pred$ for $\set{\nu:\SL\mid \pred}$ if 
$\SL$ is not important. 

\begin{definition}[Global types]
  \label{def:global-types}%
  {\em Global types} ($\GL, \GL', ...$) are generated by the following grammar:
\[
\begin{array}{rcl}
%\GL & ::=   & \Gvti{\pp}{\q}{[\pred_i]\ell}{\set{\nu:\SL\mid\pred'_i}}{\GL} 
%    \; \SEP  \; \GLPre.\GL \\
%    & \SEP & \ty \;\SEP\; \mu \ty.\GL \\[1mm]
\GL & ::=   & %\Gvti{\pp}{\q}{[\pred_i]\ell}{\set{\nu:\SL\mid\pred'_i}}{\GL} 
 \GLPre.\GL \;\SEP\; \ty \;\SEP\; \mu \ty.\GL \\[1mm]
  \GLPre & ::= & \motion{\dtsess}{(\pp_i{:}\ma_i)}\;\SEP\;
                 \GvtPre{\pp}{\q}{[\pred]\ell}{\set{\nu:\SL\mid\pred'}}
\; \SEP \; \GLPre.\GLPre \;\SEP\; \GLPre + \GLPre \;\SEP\; 
\GLPre \GLPAR \GLPre 
% \;\SEP\; \NUL
\end{array}
\]
where $\pp, \q$ range over $\PC$, $\ma_i$ range over 
abstract motion primitives, and
$\pred_i, \pred'$ range over predicates. 
$\GLPre$ corresponds to the prefix of global types where we do not allow
the recursion. 
We require that
    $\pp \neq \q$,
    $I \neq \emptyset$,
    $\freevars(\pred_i) ⊆ \pp.X ∪ \pp.W$,
    $\freevars(\pred'_i) ⊆ \pp.X ∪ \pp.W ∪ \set{\nu}$,
    and $\ell_i \neq \ell_j$ whenever $i \neq j,$ for all $i,j\in I$.
We postulate that recursion is guarded and recursive types with the same regular tree are considered equal.
We omit the predicate annotation if the predicate is $\true$ or not important.
\end{definition}

In Definition~\ref{def:global-types}, the main syntax 
follows the standard definition of global types in multiparty session types
\cite{KY13,KY2015,DGJPY15}, with the inclusion of more flexible syntax
of choreographies (\emph{separation} $\GLPre \GLPAR \GLPre$, 
\emph{sequencing} $\GLPre.\GLPre$ and summation $\GLPre + \GLPre$)
and \emph{motion} primitive $\motion{\dtsess}{(\pp_i{:}\ma_i)}$ 
extended from \cite{ECOOP19},  
and branching
$\GvtPre{\pp}{\q}{[\pred]\ell}{\set{\nu:\SL\mid\pred'}}$. 

The motion primitive explicitly declares 
a \emph{synchronisation} by AG contracts 
among all the participants $\pp_i$.
The {\em branching} type 
%$\Gvti{\pp}{\pq}{[\pred_i]\ell}{\set{\nu:\SL\mid\pred'_i}}{\GL}$ 
formalises a protocol where participant $\pp$ 
first tests if the guard $[\pred]$, then sends to $\pq$ one message with label $\ell$ 
and a value satisfying the predicate refinement $\pred'$. 
%, for some $i \in I$; 
%then, depending on which $\ell_i$ was sent by $\pp$, the protocol
%continues as $\GL_i$.
Recursion is modelled as $\mu\ty.\GL$, %
where  variable  $\ty$ is bound and guarded in $G$, e.g.,  
$\mu\ty.\ty$ is not a valid type. 
% We assume $\NUL.\GLPre=\GLPre.\NUL=\NUL\GLPAR \GLPre=\GLPre\GLPAR \NUL =\GLPre+\NUL=\NUL+\GLPre=\GLPre$ and $\NUL.\GL=\GL$. 
Following the standard session types, 
in $\GLPre_1 + \GLPre_2 + ... + \GLPre_n$, we assume: 
$g_i = \GvtPre{\pp}{\q}{[\pred_i]\ell_i}{\set{\nu:\SL\mid\pred'_i}}.g_i'$ 
and $\ell_i \not=\ell_j$; and similarly for $\GL$. 
By this rule, hereafter we write: 
%\[
$\Gvti{\pp}{\pq}{[\pred_i]\ell}{\pred'}{\GL}$,  
%\]
combining summations and branchings and putting $\GL$ in the tail into
each branching as the standard multiparty session types. 
$\participant{\GL}$ denotes a set of participants appeared in
$\GL$, inductively defined by $\participant{\motion{\dtsess}{(\pp_1{:}\ma_1,\ldots,\pp_k{:}\ma_k)}}
= \set{\pp_1,\ldots,\pp_k}$ and 
$\participant{\GvtPre{\pp}{\q}{\ell_i[\pred]}{\set{\nu:\SL\mid\pred'}}}=\{\pp,\q\}$
  with other homomorphic rules. 

A ``separating conjunction'' $\GLPAR$  allows us
to reason about subsets of participants.
It places two constraints on the processes and motion primitives on 
the two sides of $\GLPAR$: 
first, there should not be any communication that crosses the boundary and second, the motion
primitives executed on one side should not be coupled (through
physical inputs) with motion primitives on the other.
We call 
$\GLPre_1 \GLPAR \GLPre_2$
\textbf{\emph{fully-separated}} if $\participant{\GLPre_1} \cap \participant{\GLPre_2} = \emptyset$, there exist
$\FP_1$, $\FP_2$ with $\FP_1\cap \FP_2 = \emptyset$, and 
for every motion primitive $\judgement{\ma}{\pre,A, G,\post, \FP, D,\timestep}$ in $\GLPre_i$, we have
$A$ depends only on state variables in $\participant{\GLPre_i}$ and for all $t$, $\FP\{t/\clock\} \subseteq \FP_i\{t/\clock\}$,
for $i\in\set{1,2}$. 
$\GL$ is \textbf{\emph{fully-separated}} if each $\GLPre_1 \GLPAR \GLPre_2$ in $\GL$
is fully-separated. 

%This use of $\GLPAR$ is different from the use in multiparty session types, where $\GLPAR$ indicates causally
%independent messages \cite{WHO?}.

% \begin{remark}
% \label{rem:noend}  
Our global type does not include an $\tend$ type.
An $\tend$ introduces an implicit global synchronisation that requires 
all components to finish exactly at the same time.
% As mentioned before, our process syntax in \Sec~\ref{sec:calculus} 
% does not include the null process. 
% The physical state of the component and its geometric footprint 
% continues to exist even if the 
% program terminates and must be accounted for when reasoning about other components.
% % We sometimes use $\tend$ for notational simplicity, where $\tend$ stands for 
% % $\Gmotion{\dtsess}{(\pp_i: \ma_i)}{G}$ which preserve their last contracts\DZ{only if no time}.
% % \RMi{is this $\mu \ty.\Gmotion{\dtsess}{...}{\ty}$?}
Informally, ``ending'' a program is interpreted as robots stopping their motion and staying idle forever (by forever
executing an ``idle'' primitive).
Our progress theorem will show that well-typed programs have 
infinite executions. 
% \end{remark}


\myparagraph{Data Flow Analysis on Choreographies}
%
Not every syntactically correct global type is meaningful.
%First, we require that any motion type
%$\motion{\dtsess}{(\pp_i{:}\ma_i)}$ 
%consists 
%of compatible motion primitives. 
We need to check that the AG contracts work together and that the
sends and receive work w.r.t the time taken by the different motions.
These checks can be performed as a ``dataflow analysis'' on the tree obtained
by unfolding the global type.
We start with a few definitions and properties.

\textbf{\emph{Well-scopedness.}}
Consider the unfolding of a global type $\GL$ as a tree. The leaves
of the tree are labeled with motions $\motion{\dtsess}{(\pp_i{:}\ma_i)}$ or message $\pp\to\q$, and internal nodes are labeled with the operators $.$, $\GLPAR$, or $+$.
By our assumption, we decorate each $+$ node with the sender and receiver $\pp\to\q$
below it.

We say the tree is \textbf{\emph{well-scoped}} if there is a way to label the nodes of the tree
following the rules below:
(1) The root is labeled with the set $\PC$ of all participants.
(2) If a ``.'' node labeled with $\PC'$, both its children are also labeled with $\PC'$, if possible.
(3) If a ``+'' node associated with a message exchange $\pp\to\q$ is labeled with $\PC'$, and both
$\pp,\q\in \PC'$, then each of its children are also labeled with $\PC'$, if possible.
(4) If a ``\GLPAR'' node is labeled with $\PC'$, then we label its children with $\PC_1$ and $\PC_2$
such that $\PC_1 \cap \PC_2 = \emptyset$ and $\PC_1 \cup \PC_2 = \PC'$.
(5) A leaf node $\motion{\dtsess}{\pc_i:\ma_i}$ is labeled with $\PC'$ if all $\pc_i$ are in $\PC'$, otherwise the labeling fails.
(6) A leaf node $\pp \to \q$ is labeled with $\PC'$ if both $\pp, \q$ are in $\PC'$, otherwise the labeling fails.

Such a scope labeling is unique if the global type is fully-separated and no participant is ``dropped,''
and so we can define the scope of a node in an unambiguous way.
% \NYi{ \textbf{\emph{total and compatible motion}} includes well-scopedness?}
% A well-scoped global type has \textbf{\emph{total and compatible motion}} if 
% every motion type $\motion{\dtsess}{(\pp_i:\ma_i)}$ has a motion primitive for every participant in scope and 
% the tuple of motion primitives $(\pp_i:\ma_i)$ is compatible.

\textbf{\emph{Unique minimal communication}.}\ 
We first define a notion of \emph{happens-before}
with \emph{events} as nodes labeled with motions $\motion{\dtsess}{(\pp_i{:}\ma_i)}$ or message exchanges $\pp\to \q$.
We define a \emph{happens before} relation on events as the smallest strict partial order such that: 
there is an edge $n:e \to n':e'$ if
there is an internal node $n^*$ in the tree labeled with $.$ and $n$ is in the left subtree of $n^*$ and
$n'$ is in the right subtree of $n^*$, and one of the following holds:
(1)~$e \equiv \pp\to\q$, $e' \equiv \pp'\to\q'$ and $\pp'$ is either
$\pp$ or $\q$; or
(2)~$\participant{e} \cap \participant{e'} \not = \emptyset$.  
%$e \equiv \motion{\dtsess}{(\pp_i{:}\ma_i)}$ and
%$e' \equiv \motion{\dtsess}{(\q_i{:}\ma'_i)}$ and some $\pp_i$ equals $\q_j$;
%(2)~$e \equiv \motion{\dtsess}{(\pp_i{:}\ma_i)}$ and
%$e' \equiv \pp\to \q$ and there is some $\pp_i$ that equals $\pp$ or $\q$;
%and
%(4)~$e \equiv \pp\to\q$, $e' \equiv \motion{\dtsess}{(\pp_i{:}\ma_i)}$ and
%$\pp$ or $\q$ are among the $\pp_i$'s.
We say there is an \emph{immediate happens before} edge $n\to n'$ if $n\to n'$ is in the happens before
relation but there is no $n''$ such that $n \to n''$ and $n''\to n'$.
A global type has \textbf{\emph{unique minimal communication}} after
motion 
iff every motion node $n:\motion{\dtsess}{\pp_i:\ma_i}$
has a \emph{unique} immediate happens before edge to some node $n':\pp\to\q$.

\textbf{\emph{Sender readiness}.}\ 
Consider now a type with unique minimal communication after motion and consider the unique immediate happens before edge 
$n:\motion{\dtsess}{(\pp_i{:}\ma_i)} \to n':(\pp\to\q)$.
Suppose $\pp$ is among the processes executing the motion primitives.
Since the motion primitives are assumed to be compatible, we know that at most one process is executing a non-interruptible motion,
and all the others are executing interruptible motions.
Since $\pp$ is the next process to send a message, we must ensure that it is the unique process executing the non-interruptible motion.
Compatibility ensures that the durations of all other processes are such that they are ready to receive the message from $\pp$.
We call this condition \textbf{\emph{sender readiness}}: whenever there is a communication after a motion, the sender of the communication
was the unique participant executing a non-interruptible motion; or every process in the motion was executing an interruptible motion.
On the other hand, if $\pp$ is not among the processes (this can happen when to parallel branches merge),
every participant in the motion must have been executing an interruptible motion.

% Now consider a type $\Gmotion{\dtsess}{(\pp_i {:} \ma_i)}{
% \Gvti{\pp}{\q}{[\pred_i]\ell}{\pred'}{\GL}}$
% suppose that $\pp$ is the unique minimal sender.
% We want to ensure that when $\pp$ finishes executing its motion primitive and is ready to send,
% it is not blocked by other components because their 
% motion primitives have not finished executing.
% This is where we require the interruptibility annotation step $\timestep$ in the judgement.
% We say $\pp$ is \emph{ready to send} for the judgement 
% $\judgement{\Pi}{\true, \true, \cdot, \cdot, \FP, \timestep}$ 
% if in the derivation, $\pp$'s motion primitive satisfied the judgement 
% $\judgement{\pp\plays S}{\cdot, \cdot, \cdot, \cdot, \cdot, \timestep'}$ 
% and $\timestep = \timestep'$.
% Intuitively, the minimal sender is ready to send if it is the only component
% to have executed a non-interruptible motion primitive in the previous step.

\textbf{\emph{Total synchronisation}.}\ 
It is not enough that $\pp$ sends a message to only one other participant: if $\pp$ and $\q$ decide to switch to
a different motion primitive, every other participant in scope must also be informed.
This is ensured by the \textbf{\emph{total synchronisation}} between motions: 
we require that whenever there is a happens before edge between $n:\motion{\dtsess}{(\pp_i:\ma_i)}$ to $n':\motion{\dtsess}{(\pp'_i:\ma'_i)}$,
then for every $\pp_i$, there is a node where $\pp_i$ is a sender or a recipient that happens before $n'$. 

\textbf{\emph{Synchronisability}.} \ 
We call a global type is \textbf{\emph{synchronisable}} if it satisfies 
unique minimal communication, 
sender readiness, and 
total synchronisation. 
Synchronisability of a global type can be checked in time polynomial
in the size of the type by unfolding each recursive type once.  

\begin{example}[Synchronisability] \rm 
We illustrate the synchronisability condition. 
In general, a node can have multiple outgoing immediate happens before edges.
Consider, for distinct participants $\pp,\q,\pp'$, the type
${\pp}\rightarrow {\q}:{\ell}.
{\pp'}\rightarrow {\q}:{\ell'}.\GL$. 
The minimal senders are $\pp$ and $\pp'$, because these two sends cannot be uniquely ordered in an execution.
We avoid such a situation because in a process $\q$ we would not know whether to expect
a message from $\pp$ or from $\pp'$ or from both.

Note that synchronisability disallows a sequence of two motions without an intervening
message exchange.
Thus,
$\motion{\dtsess}{(\pp{:}\ma_1,\q{:}\ma_1')}.\motion{\dtsess}{(\pp{:}\ma_2,
  \q{:}\ma_2')}.\GL$ is not well-formed. 
This is because the implementation of the participants do not have any mechanism to synchronize 
when to shift from the first motion primitive to the second.

We require the total synchronisation between motions to notify every participant by some message between any change of motion primitives.
We disallow the type 
$\motion{\dtsess}{(\pp{:}\ma_{11},\pq{:}\ma_{12}, \pr{:}\ma_{13})}.{\pp}\rightarrow{\pq}:\ell.\motion{\dtsess}{(\pp{:}\ma_{21}, \pq{:}\ma_{22}, \pr{:}\ma_{23})}.\GL$.
because $\pr$ does not know when to shift from 
$\ma_{13}$ to $\ma_{23}$.

Note however, that the scoping introduced by $\GLPAR$ requires messages to be sent only to ``local'' subgroups.
The following type is fine, even though $\pp_3$ was not informed when $\pp_1$ and $\pp_2$ changed motion primitives, as it is in a different branch and there is no
happens before edge:
\begin{align*}
\left((
\begin{array}{l}
%% (\motion{\dtsess}{(\pp_1{:}\ma_1, \pp_2{:}\ma_2)}.\\
%% {\pp_1}\rightarrow{\pp_2}:{\ell_1}.\\
  %% \motion{\dtsess}{(\pp_1{:}\ma_1',\pp_2{:}\ma_2')})
(\motion{\dtsess}{(\pp_1{:}\ma_1, \pp_2{:}\ma_2)}.
{\pp_1}\rightarrow{\pp_2}:{\ell_1}.
\motion{\dtsess}{(\pp_1{:}\ma_1',\pp_2{:}\ma_2')}) 
\end{array}  
) \GLPAR \motion{\dtsess}{\pp_3{:}\ma_3} \right)
.{\pp_1}\rightarrow{\pp_2}{:\ell_1}.{\pp_1}\rightarrow{\pp_3}{:\ell_3}.G
\end{align*}
%
\end{example}

\begin{example}\rm
By inspection, the motion type in Figure~\ref{fig:basic-example} is well-scoped and fully separated.
It is also synchronizable: to see this, note that for every joint motion primitive, there is at most
one motion which is non-interruptible and the participant corresponding to that motion primitive
is the unique minimal sender.
Moreover, the unique minimal sender sends messages to every participant in the scope of the separating conjunction,
thus the type is totally synchronized.
\end{example}

We are ready to define when global types are well-formed.

\begin{definition}[Well-formed global types]
  \label{def:well-formed}
%
A global type $\GL$ is \emph{well-formed} if it satisfies the following conditions:
\begin{enumerate}
\item \emph{Total choice:} for each branching type $\Gvti{\pp}{\q}{[\pred_i]\ell}{\pred'}{G}$, we have $\bigvee_i \pred_i$ is valid.

\item 
\emph{Well-scoped:} 
$\GL$ is well-scoped and fully-separated.

\item
\emph{Total and compatible motion:} 
For every motion type $\motion{\dtsess}{(\pp_i {:} \ma_i)}$, there exists a motion primitive
for each participant in scope 
and moreover the tuple of motion primitives $(\pp_i{:}\ma_i)$ is compatible.
% A well-scoped global type has \textbf{\emph{total and compatible motion}} if 
% every motion type $\motion{\dtsess}{(\pp_i:\ma_i)}$ has a motion primitive for every participant in scope and 
% the tuple of motion primitives $(\pp_i:\ma_i)$ is compatible.


\item \emph{Synchronisability:}
The global type is synchronisable.
% \footnote{
% 	This requirement suggests that the first event in $G$ (after unrolling recursion) is a branching type. In particular, the global
% 	type cannot have sequences of motion primitives. This is not a restriction as 
% 	sequences of motions can be combined using the rule [\textsc{HSeq}] and [\textsc{HWhile}] in Figure~\ref{fig:proof-system}.}
%
%
% s.t. the minimal sender $min_T$ in $(\pp_i: \ma_i)$ must be larger than the $max_T$ of every other process. \DZ{adapt to new thing}
%
% \RMi{there should be a rule for receive that says receive is ready in 0-time.}
% \DZi{like that?}
% $
% \inferrule[\rulename{HRecv}]
%     {\judgement{\pc \plays S}{φ,A,G,φ, \FP, \delayed}}
%     {\judgement{\pc \plays \srecv(\pc,S)\{(l_i, x_i, S_i)_{i∈I}\}}{φ,A,G,φ,\FP, \instantaneous}}
% $
% \DZi{but we have to be careful not to use that outside of the
% compatibility check.}
% 
% \item messages: one process sends, all the other processes receive
% \NYi{Do not understand this comment. We should formalise?}
% 
\end{enumerate}
%
\end{definition}
%
\noindent Hereafter we assume global types are well-formed.
%% The
%% following proposition is by the fact that it is sufficient 
%% to check each condition for a finite global type 
%% where all recursive variables are unfold once, cf.~\cite{HYC2016}.

\begin{restatable}[Well-formedness]{proposition}{theoremWF}
\label{pro:WF}
Synchronisability is decidable in polynomial time.
Checking well-formedness of global types reduces to checking validity in the 
underlying logic of predicates in global types and motion primitives.
\end{restatable}
\begin{proof}
All causalities in global types can be checked 
when unfolding each recursive type once 
(cf.~\cite[\Sec.~3.5]{HYC2016}).
Hence synchronisability of a global type can be checked in time polynomial
in the size of the type by checking unique minimum communication,
sender readiness and total synchronisation simultaneously. 
By Definition \ref{def:well-formed}, checking well-formedness depends on 
checking validity in the 
underlying logic. 
\end{proof}

% \item no connection accross parallel (we don't have a proof rule to deal with mismatched motion primitives)
% \item $\GLPAR$ creates a partition of the participants, 
%       i.e. $\participant{\GLPre_1}\cap \participant{\GLPre_2}=\emptyset$
% in $\GLPre_1\GLPAR \GLPre_2$.  
% \NYi{Not sure this is correct since then we cannot write 
% $ (p \rightarrow q) \ast (p \rightarrow r)$. 
% }
% \RMi{our $\GLPAR$ is a stronger condition: no information flows across a parallel -- it is a separationg conjunction}

\subsection{Local Types and Projection}
\label{sec:local}

Next, we project global types to their end points against which each
end-point process is typed. 
The syntax of \emph{local types} extends local types from \cite{ECOOP19}.
Each local type represents a specification for each component. 

\begin{definition}[Local motion session types]
  \label{def:session-types}%
  The grammar of local types, ranged over by $T$, is:
  \begin{align*}
  T ::=  \ \Lmotion{\dtsess}{\ma}{T} \SEP \oplus\{[\pred_i]\tout\q{\ell_i}{\pred_i'}.T_i\}_{i\in I} 
          \SEP  \&\{\tin\pp{\ell_i}{\pred_i}.T_i\}_{i\in I} 
     \SEP  \&\{\tin\pp{\ell_i}{\pred_i}.T_i\}_{i\in I}\ \& \ \Lmotion{\dtsess}{\ma}{T} 
          \SEP \mu \ty.T \SEP \ty
  \end{align*}
  where $\ma$ ranges over motion primitives. 
  We require that $\ell_i \neq \ell_j$ whenever $i \neq j$, for all $i,j\in I$.
  We postulate that recursion is always guarded. 
  Unless otherwise noted, types are closed.
\end{definition}

Our goal is to \emph{project} a global type onto a participant to get a local type.
To define this notion formally, we first need the following definition that merges two
global types.

% We use $\proj{\GL}{\pr}{T}$ to denote a \emph{projection of a global type $\GL$ onto a participant $\pr$ to a local type $T$}.
% \iffull
% (see Appendix~\ref{app:proof} for the full definition),
% \else
% (see \cite{fullversion} for the full definition), 
% \fi
% which is explained by the following example. 
% \myparagraph{Projections of Global Types}
%
% Before defining the projection, we need to define how predicates such as the guards and the messages which are given in the 
% world's frame $\world$ are transformed when projected on the individual processes.
% The frame transformation uses the $\shiftTo{\pp}(\pred, P)$ function, which is defined recursively by
% \begin{itemize}
% \item $\shiftTo{\pp}(\pred,\pp\plays \proc{⋅}{{X}}{{W}}{{V}}) = ∃ v. \pred$ where $v = \freevars(\pred) \setminus (X ∪ W ∪ V)$;
% \item $\shiftTo{\pp}(\pred, \comp{P}{\con}{\fs}{Q}) = \shiftTo{\pp}(\con(\pred), P)$ if $\pp$ occurs in $P$;
% \item $\shiftTo{\pp}(\pred, \comp{P}{\con}{\fs}{Q}) = \shiftTo{\pp}(\con(\pToc(\pred)), P)$ if $\pp$ occurs in $Q$.
% \end{itemize}
% We write $\shiftTo{\pp}(\pred)$ as shorthand for $\shiftTo{\pp}(\pred,Π)$.
% We extend frame shifts to motion primitives by applying the shift to each component of a motion primitive.
% 
% Notice that $\shiftTo{\pp}$ may introduce new variables in a predicate as it collects the frame shifts.
% We eliminate these variables at the end.
% It it possible to increase the precision of the shift by collecting information about the state of the other processes.
% However, this requires a more complex global analysis and we chose this version which is a conservative overapproximation.

\begin{definition}[Merging] 
  \label{def:merge}%
We define a \emph{merging operator} $\bigsqcap$, which is a partial operation over global types, as:
\[
\small
  \textstyle%
  T_1 \mathbin{\bigsqcap} T_2 \;=\; 
  % T_3%
 % \qquad\text{if either}
  \left\{%
\text{%
    \begin{tabular}{@{\hskip 0mm}l}
      $T_1$ \hfill if $T_1 = T_2$ \hspace{2mm}
      \iftoggle{full}{$\rulename{mrg-id}$}{}  \\[2mm]%
      $\&\{\tin{\pp'}{\ell_k}{\pred_k}{.T_k}\}_{k \in I \cup J}$ \quad\quad
      \hfill if \(%
      \left\{%
      \begin{array}{l}
        T_1 = \&\{ \tin{\pp'}{\ell_i}{\pred_i}{.T_i}\}_{i \in I} \hfill \text{ and}\\%
        T_2 = \&\{ \tin{\pp'}{\ell_j}{\pred_j}{.T_j}\}_{j \in J}%
      \end{array}
      \right.%
      \)\\[3mm]
      \iftoggle{full}{\hfill $\rulename{mrg-bra1}$\\}{}
      $\&\{\tin{\pp'}{\ell_k}{\pred_k}{.T_k}\}_{k \in I \cup J} \& \ \Lmotion{\dtsess}{\ma \bigsqcap \ma'}{T'}$ \quad\quad
      \hfill if \(%
      \left\{%
      \begin{array}{l}
        T_1 = \&\{ \tin{\pp'}{\ell_i}{\pred_i}{.T_i}\}_{i \in I} \& \ \Lmotion{\dtsess}{\ma}{T'} \hfill \text{ and}\\%
        T_2 = \&\{ \tin{\pp'}{\ell_j}{\pred_j}{.T_j}\}_{j \in J} \& \ \Lmotion{\dtsess}{\ma'}{T'}%
      \end{array}
      \right.%
      \)\\[3mm]
      \iftoggle{full}{\hfill $\rulename{mrg-bra2}$\\}{}
      $\&\{\tin{\pp'}{\ell_k}{\pred_k}{.T_k}\}_{k \in I \cup J} \& \ \Lmotion{\dtsess}{\ma}{T'}$ 
      \hfill if \(%
      \left\{%
      \begin{array}{l}
        T_1 = \&\{ \tin{\pp'}{\ell_i}{\pred_i}{.T_i}\}_{i \in I} \hfill \text{ and} \\ 
        T_2 = \&\{ \tin{\pp'}{\ell_j}{\pred_j}{.T_j}\}_{j \in J} \& \ \Lmotion{\dtsess}{\ma}{T'}%
      \end{array}
      \right.%
      \) \\[3mm]
      \iftoggle{full}{\hfill $\rulename{mrg-bra3}$\\}{} 
      $\&\{\tin{\pp'}{\ell_i}{\pred_i}{.T_i}\}_{i \in I} \& \ \Lmotion{\dtsess}{\ma \bigsqcap \ma'}{T'}$ 
      \hfill if \(%
      \left\{%
      \begin{array}{l}
        T_1 = \Lmotion{\dtsess}{\ma}{T'} \hfill \text{ and} \\%
        T_2 = \&\{ \tin{\pp'}{\ell_i}{\pred_i}{.T_i}\}_{i \in I} \& \ \Lmotion{\dtsess}{\ma'}{T'}%
      \end{array}
      \right.%
      \) \\[3mm]
      \iftoggle{full}{\hfill $\rulename{mrg-bra4}$\\}{}
      $\&\{\tin{\pp'}{\ell_i}{\pred_i}{.T_i}\}_{i \in I} \& \ \Lmotion{\dtsess}{\ma}{T'}$ 
      \hfill if \(%
      \left\{%
      \begin{array}{l}
        T_1 = \Lmotion{\dtsess}{\ma}{T'} \hfill \text{ and} \\%
        T_2 = \&\{ \tin{\pp'}{\ell_j}{\pred_j}{.T_j}\}_{i \in I}%
      \end{array}
      \right. %
      \) \\[3mm]
      \if{\hfill $\rulename{mrg-bra5}$\\}\else{}\fi 
      $T_2 \mathbin{\bigsqcap} T_1$ \hfill if $T_2 \mathbin{\bigsqcap} T_1$ is defined, \\[2mm]
      undefined \hfill otherwise.
    \end{tabular}
  } %
  \right.%
\]
  %
The merge operator for motion $\ma \bigsqcap \ma'$ returns a motion primitive $\ma''$ such that $\ma'' \refines \ma$ and $\ma'' \refines \ma'$.
We can build such $\ma''$ by taking the union of the assumptions and precondition and the intersection of the guarantees, postcondition, and footprint. 
\end{definition}
%% Note that our definition is slightly simplified %
%% w.r.t.~the one of~\cite{YDBH10} and \cite{DYBH12}. 
%% Instead of this mergeability operator, one might use 
%% more general approach from \cite{SY2019}. 
%% This definition is sufficient for our purposes (i.e., to demonstrate 
%% an application of session types to robotics communications).

\begin{definition}[Projection] 
  \label{pro}%
  \label{def:projection}%
  The \emph{projection of a global type onto a participant $\pr$} is the largest relation $\proj{}{\pr}{}$ between global and session types such that, whenever
  $\proj{\GL}{\pr}{T}$:
\begin{enumerate}
    \item  if ${\GL}=\Gvti{\pp}{\pr}{[\pred_i]\ell}{\pred'}{\GL}$ then ${T}=\&\{ \tin\pp{\ell_i}{\pred'_i}.{T_i}\}_{i\in I}$ with $\proj{\GL_i} \pr T_i$;
    \item  if ${\GL}=\Gvti{\pr}{\q}{[\pred_i]\ell}{\pred'}{\GL}$ then ${T}= \oplus\{[\pred_i]\tout\pq{\ell_i}{\pred'_i}.{T_i}\}_{i\in I} $ and $\proj{\GL_i}\pr  T_i,$ $\forall i \!\in\! I$;
    \item  if ${\GL}=\Gvti{\pp}{\pq}{[\pred_i]\ell}{\pred'}{\GL}$ and $\pr \!\not\in\! \{\pp,\pq\}$ then there are $T_{\!i},$ $i \in I$ s.t.
    ${T} = \bigsqcap_{i \in I}\!\!{T_{\!i}}$, and
    $\proj{\GL_i\!}{\pr}{\!T_{\!i}},$ for every $i\in I$; 
  \item  if $\GL = \mu\ty. \GL'$ then $T=\mu\ty.T'$ with $\proj{\GL'}\pr T'$ if $\pr$ occurs in $\GL'$, otherwise undefined; and
\item if $\GL = \GLPre. \GL$ then $T=T' . T''$ 
with $\proj{\GLPre}{\pr}{T'}$ and 
$\proj{\GL}{\pr}{T''}$.\footnote{We abuse $T$ to denote \emph{a local type 
prefix} which is given replacing $\ty$ and $\mu\ty.T$ by $\NUL$ (as
defined for global type prefix $g$).}  

 \item 
$\proj{\motion{\dtsess}{(\pp_i {:} \ma_i)}}{\pr}{
\motion{\dtsess}{a_j}}$ with $\pr = \pp_j$;

\item  $\proj{(\GLPre_1 \GLPAR \GLPre_2)}{\pr}{\TLPre_i}$ 
and $\proj{\GLPre_i}{\pr}{\TLPre_i}$ if 
$\pr \in \participant {\GLPre_i}$ ($i\in \{1,2\}$)

\item  $\proj{\GLPre_1.\GLPre_2}{\pr}{\TLPre_1.\TLPre_2}$ 
with $\proj{\GLPre_i}{\pr}{\TLPre_i}$ ($i=1,2$)

\end{enumerate}
%
We omit the cases for recursions and selections 
(defined as \cite[Section~3]{SY2019}). The branching prefix 
is defined as the branching in (1-3). 
\end{definition}

\begin{example}[Projection of Figure~\ref{fig:basic-example}]\rm 
For the example from \Sec~\ref{sec:example}, 
the local type of the cart is:
\begin{align*}
\small
\mu \ty.\left(
\begin{array}{l}
	 \ (\Green!\ARRIVE(t).\Red!\FREE.\\
         \ \ \motion{\dtsess}{\MOVEM(\Green)}.\Green!\READY.
        \motion{\dtsess}{\IDLEM}.\Green?\OK.\motion{\dtsess}{\MOVEM}) \\
        \& \ (\Red!\ARRIVE(t).\Green!\FREE. \ldots \text{symmetric} \ldots)\ 
\end{array}
\right).\ty
\end{align*}
% and for the other two robots, it is:
% \begin{align*}
% \small
% \mu \ty. & (\Cart?\START.\motion{\dtsess}{\WORKM}.\\
%          & (\ (\Cart?\ARRIVE(t).\motion{\dtsess}{\WORKM}.
%                 \Cart?\READY.\motion{\dtsess}{\PICKM}.\Cart!\OK) \\
%          & \&  (\Cart?\FREE.\motion{\dtsess}{\WORKM}) \ ).\ty
% \end{align*}
%
\end{example}

\subsection{Subtyping and Typing Processes}
The local types are a specification for the processes and there is some freedom to implement these specifications.
The subtyping relation helps bridge the gap between the specification and the implementation.

\begin{definition}[Subtyping]
\label{def:subt}%
\label{tab:sync:subt}%
{\em Subtyping} $\subt$ is the largest relation between session types coinductively defined by rules in Figure~\ref{fig:subtyping}.
\end{definition}

\begin{figure}[t]
\[
\small
\begin{array}{@{}c@{}}
\cinferrule[\rulename{sub-motion}]{
    \ma \refines \ma' \\
    T \subt T'
}{
  \Lmotion{\dtsess}{\ma}{T} \subt  \Lmotion{\dtsess}{\ma'}{T'}
}\quad
%
\cinferrule[\rulename{sub-out}]{
 \forall i\in I.\ \pred_i ⇒ \pred''_i ∧ \pred'_i ⇒ \pred'''_i  ∧ T_i \subt T'_i  
}{ \oplus\{[\pred_i]\tout\pp{\ell_i}{\pred'_i}.T_i\}_{i\in I} \subt
   \oplus\{[\pred''_i]\tout\pp{\ell_i}{\pred_i'''}.T_i'\}_{i\in I\cup J}
}
\\[5mm]

\cinferrule[\rulename{sub-in1}]{
    \forall i\in I.\ \pred_i' ⇒ \pred_i ∧ T_i \subt T_i' \\ 
    \Lmotion{\dtsess}{\ma}{T} \subt \Lmotion{\dtsess}{\ma'}{T'}
}{
  \&\{\tin\pp{\ell_i}{\pred_i}.T_i\}_{i\in I\cup J} \ \& \ \Lmotion{\dtsess}{\ma}{T}
    \subt 
   \&\{\tin\pp{\ell_i}{\pred_i'}.T_i'\}_{i\in I}\ \& \ \Lmotion{\dtsess}{\ma'}{T'}
}
\\[5mm]

\cinferrule[\rulename{sub-in2}]{
\forall i\in I.\ \pred_i' ⇒ \pred_i ∧ T_i \subt T_i'}{
  \&\{\tin\pp{\ell_i}{\pred_i}.T_i\}_{i\in I\cup J}\ \& \ \Lmotion{\dtsess}{\ma}{T}
    \subt 
   \&\{\tin\pp{\ell_i}{\pred_i'}.T_i'\}_{i\in I}
}
\quad 
\cinferrule[\rulename{sub-in3}]{
    \Lmotion{\dtsess}{\ma}{T} \subt \Lmotion{\dtsess}{\ma'}{T'}
}{
  \&\{\tin\pp{\ell_i}{\pred_i}.T_i\}_{i\in I}\ \& \ \Lmotion{\dtsess}{\ma}{T}
  \subt 
  \Lmotion{\dtsess}{\ma'}{T'}
}
\end{array}
\]
\caption{Subtyping rules\label{fig:subtyping}}
\end{figure}

A subtype has fewer requirements and provide stronger guarantees.
The subtyping of motion primitives (\rulename{sub-motion}) 
allows replacing an abstract motion primitive
by a concrete one if $\ma$ refines $\ma'$ and $T \subt T'$. 
For internal choice and sending (\rulename{sub-out}), the subtyping ensure the all the messages along with the associated predicate are allowed by the supertype.
Predicate refinements are converted to logical implication.

For the external choice and message reception (\rulename{sub-in1,2,3}), subtyping makes sure the process reacts properly to the messages expected by the super type.
A subtype can have cases for more messages but they don't matter.
The subtype guarantees that the process will never receive theses messages.
On the other hand, the sender of the messages has to be the same.
We enforce this directly in the syntax of the programming language and the type system.
It may seem that (\rulename{sub-in3}) introduces a new sender in the subtype 
but this rule is correct because, in our synchronous model, sending is blocking
and cannot be delayed.
Therefore, if the supertype only contains a motion, we know for a fact that no messages can
arrive unexpectedly in the subtype. 

Our subtyping conditions generalise those of motion session types of \citet{ECOOP19} in multiple ways.
First, we allow refinement of motion primitives (\rulename{sub-motion}) as a way to abstract trajectories.
In \cite{ECOOP19}, the actions are abstract symbols and are fixed statically. 
Second, the rules for communication must check predicate refinements---in \cite{ECOOP19}, global
types did not have refinements.  


The final step in our workflow checks that the process of each
participant in a program implements its local type using the typing
rules from Table~\ref{tab:sync:typing}.  
%
Our typing rules additionally
maintain a logical context to deal with the predicate refinements
\cite{LiquidTypes}.

We write $\der{\Gamma,\Sigma}{S}{T}$ to indicate the statement $S$ has
type $T$ 
under the variable context $Γ$ and the logical context $Σ$.
$\Gamma$ is the usual typing context; $\Sigma$ is a formula characterising what is known about the state of the 
system when a process is about to execute. 
The typing rules are shown in Table~\ref{tab:sync:typing}. 
\rulename{t-motion} considers $\Sigma$ derives the pre-condition 
of motion $a$, while $Q$ guarantees its post-condition.
\rulename{t-out} assumes $\Sigma$ of $P$ derives a conjunction of the guard and
refined predicates declared in types. \rulename{t-choice1} is its
dual and \rulename{t-choice2} includes the default motion branch. 
\rulename{t-cond} is similar with the usual conditional proof
rule. 
\rulename{t-sess} combines well-typed participants each of which
follows a projection of some global type $\GL$ given assumptions over the initial state $\bigwedge_{i\in I}𝓟_i$ of each participant.
We requires the initial state to be collision free as the global types only maintains collision freedom.

\begin{table}[t]
\caption{\label{tab:sync:typing} Typing rules for motion processes.}
\centerline{$
\small
\begin{array}{c}
\inferrule[\rulename{t-sub}]{
    \der{\Gamma,\Sigma}{\PP}T \quad T\subt T'
}{
    \der{\Gamma,\Sigma}{\PP}T'
}
\qquad
\inferrule[\rulename{t-rec}]{\der{\Gamma\cup\set{\procvar:T},\true}{\PP}{T}}{\der{\Gamma,\Sigma}{\mu \procvar.\PP}T}
\qquad
\inferrule[\rulename{t-motion}]{
\der{\Gamma,a.\post}{{Q}}{T}\\
\Sigma \Rightarrow a.\pre\\
}{\der{\Gamma,\Sigma}{\motion{dt}{a}.{Q}}{\Lmotion{dt}{a}{T}}}
\\\\
\inferrule[\rulename{t-out}]{
    \Sigma \Rightarrow \pred\wedge \pred'\set{e/\nu}\\
    \der{\Gamma,\Sigma}{\e}{S}\\
    \der{\Gamma,\Sigma}{P}T
}{
    \der{\Gamma,\Sigma}{{\q}!{\ell(\e)}.{P}}{[\pred]\q!\ell(\set{\nu: S\mid\pred'}).T}
}
\quad 
\inferrule[\rulename{t-choice1}]{
    \forall i\in I \quad \der{\Gamma\cup\set{x_i:\S_i},\Sigma\wedge \pred_i\set{x_i/\nu}}{\PP_i}\T_i
}{
    \der{\Gamma,\Sigma}{\sum\limits_{i\in I}{\procin  \q   {\ell_i(x_i)} \PP_i}}{\&\{\q?\ell_i(\pred_i).\T_i}\}_{i\in I}
}
\\\\
\rulename{t-choice2}
\inferrule%[\rulename{t-choice2}]
    {
    \forall i\in I \quad \der{\Gamma\cup \set{x_i:\S_i},\Sigma\wedge \pred_i\set{x_i/\nu}}{\PP_i}\T_i \quad
    \der{\Gamma,\Sigma}{\motion{dt}{a}.{Q}}{\T}
}{
    \der{\Gamma,\Sigma}{\sum\limits_{i\in I}{\procin  \q   {\ell_i(x_i)} \PP_i}+\motion{dt}{a}.{Q}}{\&\{\q?\ell_i(\set{\nu:S\mid\pred_i}).T_i}\}_{i\in I}\ \&\ T
}
\\\\
\rulename{t-cond}
\inferrule%[\rulename{t-cond}]
    {
    \der\Gamma\e\tbool \
    \exists k \in I \
    \Sigma \wedge \e \Rightarrow \pred_k\
    \der{\Gamma,\Sigma\wedge \e}{\PP_1}{T_k} \
    \der{\Gamma, \Sigma\wedge \lnot \e}{\PP_2}{\oplus\{[\pred_i]T_i\}_{i \in I \setminus \{k\}}}
}{
    \der{\Gamma,\Sigma}{{\cond{\e}{\PP_1}{\PP_2}}}{ \oplus\{[\pred_i]T_i\}_{i\in I}}
}
    \\\\
    \rulename{t-sess}
    \inferrule%[\rulename{t-sess}]
        {
    \forall i\in I\quad\der{∅,𝓟_i}{\PP_i}{\projt \GL {{\pp_i}}} \\
    \participant \GL = \PC \\
    \forall j\in I.\ j≠i ⇒ \geom{\pp_i}(𝓟_i)\cap\geom{\pp_j}(𝓟_j) = \emptyset
}{
    \der{\bigwedge\limits_{i\in I}𝓟_i}{\prod\limits_{i\in I}\pa {\pp_i}\PP_i}\GL
}
\end{array}
$}
\vspace*{-1em}
\end{table}



\begin{comment}
\RMi{We don't have the process description. I don't know if we should add this in the main text or have it in the appendix.}
\begin{example}{(Local Types for Load Transfer)}\label{ex:overview:mpst}\rm 
\ In our example, the local types for the $\Trolley$, $\Cart$, and
$\Crane$ are:
\NYi{I commented out the old example}
%\[
%\begin{array}{rlll}
%  \small
%  \Trolley: &
%  \mu \ty.& \Cart!\PICK(\set{\nu = (x_i, y_i, lh)}).\dtsess\tuple{\IDLEM}.\Cart?\OK(\tunit).\ty\\[1mm]
%  \Cart: &
%  \mu \ty. & \Trolley?\PICK(\set{\nu= (x_i, y_i, lh)}).\Crane!\FOLD(0).\dtsess\tuple{\IDLEM}.\Crane?\OK(R=0\wedge \theta=0).\\
%  & & \dtsess\tuple{\MOVEM(x_i)}.\Crane!\GRAB(\set{\nu:\treal\mid \nu=y_i-lh\wedge x=x_i\wedge v=0}).\dtsess\tuple{\IDLEM}.\\
%  & & \Crane?\OK(\tunit).\Trolley!\OK(\tunit). \ty\\[1mm]
%    \Crane: &
%\mu \ty. & \Cart?\FOLD(y).\dtsess\tuple{\FOLDM(y)}.\Cart!\OK(\set{R=0\wedge \theta=0}).\dtsess\tuple{\IDLEMC}.\\
%         & & \Cart?\GRAB(\set{\nu\mid \nu=y_i-lh\wedge 0=x_i-x\wedge v=0}).\dtsess\tuple{\GRABM(y_i-lh)}.\Cart!\OK(\tunit).\ty\\
%\end{array}
%\]
% An interesting point is the transfer of the frame in going from the cart to the crane: the original
% message $x=x_i$ is transformed to $x-x=x_i-x$, because of the frame shift between the cart and the crane.

We type check the process (code) from Figure~\ref{fig:cart-crane-code} against these types.
\rulename{motion} rule connects the predicate refinements to the motion primitives.
The typing of the $\Crane$ uses unfolding and subtyping to go from the
type
\NYi{I commented out the old example of types}
\[
\small
\mu \ty.\&\left\{
\begin{array}{l}
%\Cart?\FOLD(y)\dtsess\tuple{\FOLDM(y)}\Cart!\OK(\set{R=0\wedge\theta=0}).\ty,\\
%\Cart?\UNFOLD(y)\dtsess\tuple{\UNFOLDM(y)}\Cart!\OK(\set{R=0\wedge\theta=0}).\ty,\\
%\Cart?\GRAB(\set{\nu\mid\nu=y\wedge x=x_i\wedge v=0})\dtsess\tuple{\GRABM(y)}.\Cart!\OK(\set{R=0\wedge\theta=0}).\ty
\end{array}\right\}\&\dtsess\tuple{\IDLEMC}
\]
to the type above.
\qed
\end{example}  

\end{comment}

\subsection{Soundness}

The soundness of multiparty sessions is shown, using subject reduction (typed sessions reduce
to typed sessions) and progress.
%% Additionally, we use Theorem~\ref{th:motion-compatibility}(2) to ensure collision freedom.
In order to state soundness, 
we need to formalise how global types are reduced 
when local session types evolve. 
To define the consumption of global types, as done for processes in \Sec~\ref{sec:opsem}, 
we extend the syntax of global types to allow \emph{partial consumption} 
of motion types.
In addition, we extend $\GLPre$, annotating each motion type with its unique minimal sender,  
%\[
%\GLPre\; ::=\; \ldots  
%\SEP \NUL 
$\motion{\dtsess}{(\pp_i{:}\ma_i)\AT t}^{\pp}$ for $t\geq 0$.  
%The null type $\NUL$ denotes a fully consumed type.
%% We also replace every occurrence of 
%% $\motion{\dtsess}{(\pp_i{:}\ma_i)}$ 
%% with 
%% $\motion{\dtsess}{(\pp_i{:}\ma_i)\AT 0}^\pp$ where $\pp$ is the unique minimal sender.

\begin{definition}[Global types consumption and reduction]
\label{def:global-type-consumption}%
\label{def:global-type-reduction}%
The {\em consumption} of the communication $\pp\lts{\ell}\q$ or motion $\motion{\dtsess}{a}[t_1,t_2]$ %
for the global type $\GL$ 
(notation $\redG \GL\pp\ell\q$ and 
$\redGM{\GL}{\motion{\dtsess}{a}[t_1,t_2]}$) %
is the global type %
defined (up to unfolding of recursive types) using the following rules: 
\begin{enumerate}
\item\label{Item:GC1}  $\redG{\big(\GvtPair \pp\q {{\ell}_i.{\GL_i}}\big)}\pp\ell\q
  = \GL_{k}$
            if there exists $k \in I$ with $\ell = \ell_k$;
\item\label{Item:GC1}
  $\redG{\big(\GvtPair \pr\ps {{\ell}_i.{\GL_i}}\big)}\pp\ell\q
   =\GvtPair \pr \ps {{\ell}_i.{(\redG{\GL_i}{\pp}{\ell}{\q})}}$
if $\{\pr, \ps\} \cap \{\pp, \q\} = \emptyset$;
%% and $\forall i \!\in\! I: \{\pp, \q\} \!\subseteq\! G_i$;
\item\label{Item:GC3}
  $\redG{(\GLPre₁ \ast \GLPre₂)}\pp\ell\q  =  (\GLPre₁' \ast \GLPre₂)$ if $\set{\pp,\q}\subseteq \participant{\GLPre_1}$ and $\redG{\GLPre₁}\pp\ell\q = \GLPre₁'$ and 
  symmetrically if $\set{\pp,\q}\subseteq\participant{\GLPre_2}$;
  %% $\redG{(\GLPre₁ ∥ \GLPre₂)}\pp\ell\q     =  (\GLPre₁ ∥ \GLPre₂')$ if $\redG{\GLPre_2}\pp\ell\q = \GLPre_2'$;  

\item\label{Item:GC41}  
  $\redGM{\motion{\dtsess}{(\pp_i{:}\ma_i)}}
     {\motion{\dtsess}{(\pp_i{:}\ma_i[t_i;t'_i])}} =
      \motion{\dtsess}{(\pp_i{:}\ma_i)\AT 0}^\pp$ 
      %
      where $\pp$ is the unique minimal sender in $\GL$.
\item\label{Item:GC4}
  $\redGM{\motion{\dtsess}{(\pp_i{:}\ma_i)\AT t}^\pp}
     {\motion{\dtsess}{(\pp_i{:}\ma_i[t_i;t'_i])}} =
      \motion{\dtsess}{(\pp_i{:}\ma_i)\AT t'}^\pp$
% 
            if $t' > t$ and for all $i$, $t'_i-t_i = t'-t$  and $t' \leq \lceil\ma_i.D\rceil$ where $\lceil D\rceil$ denotes the upper
	    bound of the interval $D$;
\item\label{Item:GC5}
  $\redGM{(\GLPre₁ \GLPAR \GLPre₂)}
{\motion{\dtsess}{(\pp_i{:}\ma_i[t_i;t'_i])_{\pp_i∈
      \participant{\GLPre_1} \uplus \participant{\GLPre_2}}}}  =  
(\GLPre₁' \GLPAR \GLPre₂')$ 
            if
            $\redGM{\GLPre_j}{\motion{\dtsess}{(\pp_i:\ma_i[t_i;t'_i])_{\pp_i∈\participant{\GLPre_j}}}} = \GLPre_j'$ ($j=1,2$)
%            and $\redGM{\GLPre₂}{\motion{\dtsess}{(\pp_j:\ma_j[t_j;t'_j]\}_{\pp_j∈ \participant{\GLPre_2}}}} = \GLPre₂'$; 
%  $\redGM{(\GLPre₁ ∥ \GLPre₂)}{\motion{\dtsess}{\{\pp_i:\ma_i[t_i;t'_i]\}_{i∈I⊎J}}}  =  (\GLPre₁' ∥ \GLPre₂')$ 
%            if
%
%            $\redGM{(\GLPre₁}{\motion{\dtsess}{\{a_i[t_i;t'_i]\}_{i∈I}}} = \GLPre₁' ∧ \redGM{\GLPre₂}{\motion{\dtsess}{\{a_i[t_i;t'_i]\}_{i∈J}}} = \GLPre₂'$; 


\item\label{Item:GC6} 
$\redGM{\GLPre}{x}= \GLPre'$ then 
$\redGM{\GLPre.\GLPre_1}{x}= \GLPre'.\GLPre_1$ and 
$\redGM{\GLPre.\GL}{x}= \GLPre'.\GL$. 
%
\item\label{Item:GC7} 
$\redGM{\GLPre}{x} = \GLPre'$ 
if $∃\GLPre''.\exists \ASENDPC.\, 
\redastGequiv{\emptyset\rhd \GLPre}{\ASENDPC \rhd \GLPre''}$ and 
$\redGM{\GLPre''}{x} = \GLPre'$ 
where $C$ is a reduction 
context of the prefix defined as: $C = C.g \SEP   C\GLPAR g \SEP   g
\GLPAR C \SEP [\ ]$ and $\ASENDPC$ is a set of enabled senders
such that $\ASENDPC\subseteq \PC$ and  
\begin{enumerate}
\item\label{Item:GC7A} $\redGequiv{\ASENDPC\rhd C[\motion{\dtsess}{(\pp_i{:}\ma_i)\AT t}^\pp]}{
  \ASENDPC \cup\set{\pp} \rhd C }$ 
if $∃ i.~\pp_i = \pp \wedge t ∈ D_i \wedge \timestep_i =
\delayed$.

\item\label{Item:GC7B} $\redGequiv{\ASENDPC\rhd C[\motion{\dtsess}{(\pp_i{:}\ma_i)\AT
      t}^\pp]}{\ASENDPC \rhd C}$ with $\pp\in\ASENDPC$ and  
for all $i$, $\pp_i\not = \pp$ and $t\in D_i$.
\end{enumerate}

\begin{comment}
\RMi{OLD 7a, 7b:}
\item 
$\redGM{\GLPre}{x} =\GLPre'$ and 
if $∃\GLPre''.\, \redGequiv{\GLPre}{\GLPre''} ∧
\redGM{\GLPre''}{x} = \GLPre'$ 
\begin{enumerate}
\item $\redGequiv{C[\motion{\dtsess}{(\pp_i{:}\ma_i)\AT t}]}{C}$ 
if $∃ i.~ t ∈ D_i ∧ \timestep_i = \delayed$ 
where $C$ is a reduction 
context of the prefix defined as: $C = C.g \SEP   C\GLPAR g 
\SEP   g \GLPAR C \SEP [\ ]$.

\item $\redGequiv{C^-[\motion{\dtsess}{(\pp_i: \ma_i)\AT t}]}{C^-}$
if $\forall i.~ t ∈ D_i ∧ \timestep_i = \instantaneous$ 
where $C^-$ is a separation reduction 
context of the prefix defined as: $C^- =  C^-\GLPAR g 
\SEP   C^- \GLPAR g \SEP [\ ]$.
\end{enumerate}
\end{comment}
%
\end{enumerate}

%Finally, we define 
%a relation $\redGequiv{\GL}{\GL'}$ as
%\[
%\begin{array}{l}
%% \redGequiv{\motion{\dtsess}{a}}{\motion{\dtsess}{a\AT 0}} \\
%\redGequiv{\motion{\dtsess}{\{\pp_i:\ma_i\}_{i∈I}\AT t}}{\NUL} \qquad \text{if\;} ∃ i ∈ I.~ t ∈ D_i ∧ \timestep_i = \delayed \\
%\redGequiv{\NUL ∥(\motion{\dtsess}{(\pp_i: \ma_i)_{i∈I}\AT t}.g)}{\NUL ∥ g } \qquad \text{if\;} \forall i ∈ I.~ t ∈ D_i ∧ \timestep_i = \instantaneous \\
%\redGequiv{(\NUL  ∥\NUL).\GLPre}{\GLPre} \quad \redGequiv{\NUL.g}{g}
%\end{array}
%\]
%and let $\redGM{\GLPre}{x} =\GLPre'$ if $∃\GLPre''.\, \redGequiv{\GLPre}{\GLPre''} ∧ \redGM{\GLPre''}{x} = \GLPre'$. 
%
%
\begin{comment}
\[
\small
\begin{array}{r@{\hskip 2mm}c@{\hskip 2mm}l}
  \redG{\big(\Gvti \pp\q {[\pred_i]\ell} {\pred'}{\GL}\big)}\pp\ell\q     & = &   \GL_{k} \\
            &   &   \text{if\; }\exists k \in I : \ell = \ell_k \\[3mm]
  \redG{\big(\Gvti  \pr\ps {[\pred_i]\ell} {\pred'} {\GL}\big)}\pp\ell\q   & = &   \Gvtir  \pr \ps \ell {\pred'}{\GL} \\
            &   & \hspace{1mm} \text{if\; }  \{\pr, \ps\} \cap \{\pp, \q\} = \emptyset ~\land~ \forall i \!\in\! I: \{\pp, \q\} \!\subseteq\! G_i \\[3mm]
  \redG{(\GL₁ ∥ \GL₂).\GL}\pp\ell\q     & = &  (\GL₁' ∥ \GL₂).\GL  \\
            &   & \hspace{1mm} \text{if\; }\exists \redG{\GL₁}\pp\ell\q = \GL₁' \\[3mm]
  \redG{(\GL₁ ∥ \GL₂).\GL}\pp\ell\q     & = &  (\GL₁ ∥ \GL₂').\GL \\
            &   & \hspace{1mm} \text{if\; }\exists \redG{\GL₁}\pp\ell\q = \GL₂' \\[3mm]
  \redGM{\Gmotion{\dtsess}{\{a_i\}{i∈I}@t}{\GL} }{\motion{\dtsess}{\{a_i[t_i;t'_i]\}_{i∈I}}}   & = & \Gmotion{\dtsess}{\{a_i\}_{i∈I}@t'}{\GL} \\[3mm]
            &   & \hspace{1mm} \text{if\; } ∀ i, j.~ t'_i-t_i = t'_j-t_j = t'-t ∧ t' > t ∧ t' ∈ D_i\\[3mm]
  \redGM{(\GL₁ ∥ \GL₂).\GL}{\motion{\dtsess}{\{a_i[t_i;t'_i]\}_{i∈I⊎J}}}     & = &  (\GL₁' ∥ \GL₂').\GL \\
            &   & \hspace{1mm} \text{if\; } \redGM{\GL₁}{\motion{\dtsess}{\{a_i[t_i;t'_i]\}_{i∈I}}} = \GL₁' ∧ \redGM{\GL₂}{\motion{\dtsess}{\{a_i[t_i;t'_i]\}_{i∈J}}} = \GL₂' \\[3mm]
  \redGM{\GL}{x}           & = & \GL' \\
            &   & \hspace{1mm} \text{if\;} ∃\GL''.\, \redGequiv{\GL}{\GL''} ∧ \redGM{\GL''}{x} = \GL' \\[3mm]
\end{array}
\]
\end{comment}
In (6) and (7), we write $x$ as either
${\pp}\rightarrow{\q}$ or $\motion{\dtsess}{a}[t_1,t_2]$.
The \emph{reduction of global types} %
is the smallest pre-order relation closed under the rule:
\(
\GL\RedG\redG \GL\pp{\ell}\q \quad \text{and} \quad \GL\RedG\redGM{\GL}{\motion{\dtsess}{\pp_i{:}\ma_i[t_i,t'_i]}}
\).
\end{definition}

\noindent Note that the above reduction preserves 
well-formedness of global types.
We can now state the main results.
Our typing system 
is based on one in \cite{DBLP:journals/jlp/GhilezanJPSY19}
with motion primitives and refinements. 
Since the global type reduction in 
Definition~\ref{def:global-type-consumption}
is only related to communications or synchronisation
of motions but not refinements, 
(1) when the two processes $\pp$ and $\q$ synchronise by a
communication, its global type can always reduce; or
(2) when all processes synchronise by the same motion
action, their corresponding global type can always be
consumed.

Thus process behaviours correspond to reductions of global types, which
is formulated as in the following theorem.
%Hence the following theorem directly
%follows from \cite[Theorem 3.21]{DBLP:journals/jlp/GhilezanJPSY19}.
Recall $\xrightarrow{\alpha}$ denotes any transition relation or reduction. 

\begin{restatable}[Subject Reduction]{theorem}{theoremSR}
\label{th:SR}
  Let  $\N$ be a multiparty session, $\GL$ be a well-formed global type, and a physical state $I$ such that $\der{I}{\N}{\GL}$.
  For all $\N'$, if $\N \xrightarrow{\alpha} \N'$, then
  $\der{I'}{\N'}{{\GL}'}$ for some ${\GL}'$, $I'$ such that ${\GL}\RedG{\GL}'$.
  Thus, if $\N\equiv \N'$ or $\N \xrightarrow{\alpha_1}\cdots\xrightarrow{\alpha_n} \N'$, then $\der{}{\N'}{{\GL}'}$ for some ${\GL}'$ such that ${\GL}\RedG{\GL}'$.
\end{restatable}

\iftoggle{full}{
See Appendix~\ref{app:sr} for the detailed proofs.
}{
See \cite{fullversion} for the detailed proofs.
}

Below we state the two progress properties as already explained
in \Sec~\ref{sec:example}. 
The first progress
is related to communications, while the second one gurantees
the typed multiparty session processes are always collision free.
As a consequence, if $\der{I}\N{\GL}$ for a well-formed type,
then $\N$ does not get stuck and can always reduce.
%  cf. Remark~\ref{rem:noend}. 

\begin{restatable}[Progress]{theorem}{theoremPROG}
\label{th:progress}
Let $\N$ be a multiparty session, $\GL$ be a well-formed type, and a physical state $I$. 
If $\der{I}\N{\GL}$ then:
\begin{enumerate}
\item 
{\sc (Communication and Motion Progress)}
there is $M'$ such that $M \red M'$ and
\item 
{\sc (Collision-free Progress)} If $M \red^\ast M'$, then 
$M'$ is also collision free.
\end{enumerate}
\end{restatable}

\begin{proof} ({\em Outline --
\iftoggle{full}{
see Appendix~\ref{app:sr} for the detailed proofs
}{
see \cite{fullversion} for the detailed proofs.
}
})

{\em (Communication Progress)} The proof is divided into two cases:
  (a) the guard appearing in the branching type followed by
  (b) a message exchange between two parties.
Case (a) follows from the fact that there is always at least one guard
  in a choice whose predicate is evaluated to true (Definition \ref{def:well-formed}(1)).
  The typing rules ensure that the predicates are satisfied when a
  message is sent.
Case (b) is proved using
  Theorem~\ref{th:SR} with
  Definition \ref{def:well-formed}(4) since the unique minimal
  sender in $G$ can always send a message.

{\em (Motion Progress)} 
For executing motions, Definition~\ref{def:well-formed}(3) and Theorem~\ref{th:motion-compat}
ensure local trajectories can be composed into global trajectories. 

{\em (Collision-free Progress)} 
By induction.
Under $I$ and by \rulename{t-sess}, $\N$ is initially collision free.
For the communication, note that it does not change the physical state, and therefore, does not impact the geometric footprint used by a process.
Hence the case $\redG \GL\pp\ell\q$ is straightforward.
For motion actions, Definition~\ref{def:well-formed}(3) and Theorem~\ref{th:motion-compat} ensures collision freedom through execution steps.
For a collision free program, collision freedom of the next state follows from compatibility of motion. 
\end{proof}
%

%% Here, we review the difference and explain how our extensions with motion primitives and flows changes the proof.
%% Theorem~\ref{th:SR} tells us that a well typed program remains well typed after taking a step.
%% To prove progress, we need to case split on the program with its type, and show that the program can always make a step.
%% When we have only messages, it is very similar to synchronous multiparty session types.
%% The only difference is dealing with the guarded choice.
%% Here, we use the fact the choice in the well-formed types is total.
%% There is always at least one guard which evaluates to true and can be taken.
%% This condition comes from the assumption on the global type and local types inherits this property though the projection.
%% Another important point during the communication is to preserve the collision freedom.
%% Notice that sending does not change the state and receiving only changes the logical state which does not impact the geometric footprint used by a process. 
%% Then we need to look at motions and the transitions between phases of communication and motions.
%% While motions executes, Theorem~\ref{th:motion-compatibility} guarantees that the system can make a step or the motion has terminated.
%% In case that the motion has terminated, we know that there is an unique minimal sender ready to send by the compatibility of motion primitive and the synchronisability of global types.
%% By the same argument we know that the other processes are ready to receive or do not expect any message.
%% Therefore, the minimal sender is able to take a step and send a message.
%% The transition from communication to motions is easier.
%% When all the communication has reduced (multiparty session types guarantees that no deadlock can occurs), before the processes can start executing motion primitives we need to show that the preconditions are satisfied.
%% The type checking phase guarantees that each process satisfies the precondition of its motion primitive.
%% Finally, the last remaining part is dealing with the initial state of the system.
%% Here we need the collision freedom assumption.
%% If the system starts in an arbitrary state a collision can happens before any transition is taken and, therefore, we need to assume that the system starts in a good state.
%% If the first instruction in the program is about communication then the footprints are preserved and the system stays collision free.
%% If the first instruction is a motion, the compatibility preserves collision freedom but we still need to assumes it holds when the motion starts executing.


% disjointness an init motion primitive
% bootstrapping the system
% assigments and synchronization of external store


\begin{comment}
\begin{remark}[Time Divergence]
\label{rem:timediv}
\NYi{We can look at our CONCUR paper today. This remark sounds a bit weak}
\DZi{The CONCUR paper looks at a sightly different problem.
    There the issue comes from the asynchronous communication.
    Here the issue comes from the flow and the imperative loops.
    For the communication, we could do like in the ECOOP paper: force loops to contain a flow.
    However, it would not fix the issue completely.
    Example such the bouncing ball (\url{https://www.mathworks.com/help/simulink/examples/simulation-of-a-bouncing-ball.html}) can be encoded with a flow and a loop, no communication needed.}
The progress theorem checks that a program can always make a step.
However, it does not guarantees that time progresses.
For instance, there could be a $0$ time loop where processes send and receive an unbounded number of messages.
Similarly, the proof system for motion primitive does not guarantee that a motion terminates.
Progress of time is a challenging issue when modeling cyber-physical systems.
Not only can there be $0$ time loops, there can as also be Zeno traces, i.e. flows which progress by smaller and smaller amount until they converge to a finite value.
Often, one simply assumes that time diverges \cite{Henzinger96}. %, or sufficient conditions are identified \cite{DBLP:journals/jcss/BenvenisteBCP12}.
As future work, we plan to investigate liveness concern and how to modify our proof and type system to also provide liveness guarantees.
\end{remark}
\end{comment}

\subsection{A More Complex Coordination Example with Producer}
\label{subsec:large}

% \input{example_figure}
% \begin{figure}[t]
% \centering
% %\includegraphics[width=0.35\textwidth]{sorting_setup.jpg}
% \includegraphics[width=0.35\textwidth]{example.png}
% \caption{Schematic representation of the motivating example}
% %A coordination manoeuvre with a Panda arm (white), a cart-mounted
% %open-source BCN3D MOVEO arm, and a custom-built cart}
% \label{fig:ex}
% \end{figure}

% \input{global_example}

% Figure~\ref{fig:ex}(a) shows an extended version of
% the example from \Sec~\ref{sec:example} that adds a producer robot
% to the cart and the two robot arms.
We now discuss an extended version of the coordination example from \Sec~\ref{sec:example}
that we shall implement on physical robots in \Sec~\ref{sec:eval}.
In addition to cart and two arms, we add a producer robot.
The $\Producer$ generates green or red parts and places them on to the cart.
The cart $\Cart$ carries the part to the two robot arms as before.
We shall use this extended version as the basis for one of our case studies.

The coordination protocol is as follows.
First, the protocol starts by syncing all participants.
Then, the cart moves to the producer after announcing a message $\ARRIVE$.
While the cart moves to the producer, the two consumer robots can work independently.
When the cart is at the producer, it synchronises through a message $\READY$, and idles
while the producer places an object on to it.
When the producer is done, it synchronises with the cart, and tells it whether the object is green or red.
Based on this information, the cart tells one of the consumers that it is arriving with a part and
tells the other consumer that it is free to work.
Subsequently, the cart moves to the appropriate consumer to deposit the part, while the other consumer
as well as the producer is free to continue their work.
When the robot is at the consumer, it syncs through a message, and idles until the part is taken off.
After this, the protocol starts again as the cart makes its journey back to the producer, while the consumers
independently continue their work.
%% Figure~\ref{fig:ex}(b) shows a message sequence chart for the messages exchanged by the components.

\begin{figure*}[t]
{\small
\begin{align*}
\text{Initial Phase} \ \equiv\ 
\begin{array}{l}
\Cart \to \Producer: \ARRIVE. \Cart\to \Green: \START.\Cart\to\Red:\START.\\
  \left( 
 \begin{array}{ccc}
 \left(
 \begin{array}{l}
 (\motion{\dtsess}{\tuple{\Cart:\MOVEM^\delayed(\Producer), \Producer:\WORKM^\instantaneous}}^\Cart.\\
  \Cart\to\Producer:\READY.\motion{\dtsess}{\Cart:\IDLEM^\instantaneous,\Producer:\PLACEM^\delayed})^\Producer.
 \end{array} \right) \\
 \quad\quad ~\GLPAR~ \motion{\dtsess}{\Red: \WORKM^\instantaneous}^\Producer 
 ~\GLPAR~ \motion{\dtsess}{\Green: \WORKM^\instantaneous}^\Producer 
 \end{array} 
 \right)
\end{array}
\end{align*}
\begin{align*}
\begin{array}{l}
\text{Process Green Item} \ \equiv\ \\
  \quad \quad \left( \begin{array}{cc}
               \motion{\dtsess}{\Producer:\WORKM^\instantaneous}^\Cart) ~\GLPAR~ & 
               \left( 
               \begin{array}{l}  
                    \Cart\to\Green:\ARRIVE.\Cart\to\Red:\FREE.  \\
                    \left(\begin{array}{cc}
     \text{as in the green box in Figure~\ref{fig:basic-example}}
     %RM                     \left( \begin{array}{l}
     %RM                         \motion{\dtsess}{\Cart:\MOVEM^\delayed(\Green),\Green:\WORKM^\instantaneous}^\Cart.\\
     %RM \Cart\to\Green:\READY.\\
     %RM  \motion{\dtsess}{\Cart:\IDLEM^\instantaneous,\Green:\PICKM^\delayed}^\Green.\\ 
     %RM                         \Green\to\Cart:\OK
     %RM                     \end{array}  \right)
                      & ~\GLPAR~ \motion{\dtsess}{\Red:\WORKM^\instantaneous}^\Cart
                      \end{array}\right)
               \end{array} \right)
          \end{array} \right) \\
\end{array}
\end{align*}
%
\begin{align*}
\text{Global Type} \ \equiv \ 
\mu \ty. & \langle \text{Initial Phase}\rangle.
 \left(
 \begin{array}{l}
 (\Producer  \to\Cart:\GREEN. \langle \text{Process Green Item} \rangle)\\
 + 
  (\Producer\to\Cart:\RED. \langle \text{Process Red Item} \rangle)
% 
% (\motion{\dtsess}{\Producer:\WORKM^\instantaneous}^\Cart) ~\GLPAR~ \text{\quad as the above replacing
%     $\Green$ by $\Red$\quad } ~\GLPAR~ \motion{\dtsess}{\Green:\WORKM^\instantaneous}) \big\} 
 \end{array} 
\right) .\ty
\end{align*}
}
\vspace{-3mm}
\caption{Motion session type annotated with minimal senders. For readability, we have broken the type into sub-parts:
the initial phase, and processing items (the type for processing red items is symmetric and omitted)\label{fig:annotated-global-session-type}}
\end{figure*}

\myparagraph{Global Type}
The global type for the example extends one in Figure~\ref{fig:basic-example}, and is shown
in 
Figure~\ref{fig:annotated-global-session-type}. 
% It not only contains message exchanges between participants (e.g., $\Cart\to\Red:\READY$ sends a message ``$\READY$''
% from the $\Cart$ process to the $\Red$ robot) and choices $+$ from multiparty session
% types, but also describes
% jointly executed motions (e.g., $\motion{\dtsess}{\Cart:\IDLEM,\Red:\PICKM}$ describes
% the situation where the cart is idling and the red robot is picking an
% item from the cart).
It can be seen that the global type has total choice (trivially), and is well-scoped and synchronisable. 
The motion primitive specifications are omitted;
we ensure in our evaluation that the motion primitives are compatible and the type is fully separated using calls
to the SMT solver dReal.

\myparagraph{Processes}
The processes in this example extend the processes from \Sec~\ref{sec:example} but the $\Red$ and $\Green$
processes are as before:
\[
\begin{array}{ll}
\Cart:
  &
\begin{array}{l}\small
\mu \procvar. \Producer!\ARRIVE.\Red!\START.\Green!\START.\MOVEM(\text{co-ord of }\Producer).\Producer!\READY.\IDLEM.\\
 \ (\Producer?\RED.\Red!\ARRIVE.\Green!\FREE.\MOVEM(\text{co-ord of }\Red).\\
 \ \ \ \quad\quad \Red!\READY.\IDLEM.\Red?\OK.\procvar\\
 \ + \Producer?\GREEN.\textrm{ symmetrically for $\Green$ })
\end{array}
\\[3mm]
\Producer: &
\begin{array}{l}\small
\mu \procvar.\Cart?\ARRIVE.\WORKM.\Cart?\READY.\PLACEM. (\Cart!\GREEN + \Cart!\RED).\WORKM.\procvar
% \\[2mm]
% \Red:
% \!\!\!\!\!\!\!\!\!\!\!\!\\
% \Green:\!\!\!\!\!\!\!\!\!\!\!\!\\
% \mu \procvar.\!\!\!\!\!\!& \Cart?\START.\WORKM.\\
% & \ ((\Cart?\ARRIVE.\WORKM.\Cart?\READY.\\& \quad \ \PICK.\Cart!\OK)\\
%     & \ + (\Cart?\FREE.\WORKM)).\procvar\\
\end{array}    
\end{array}  
\]
%
\begin{comment}
\[
\begin{array}{c|c}
\begin{array}{rl}\small
\Cart:\!\!\!\!\!\!\\  
\mu \procvar.\!\!\!\!\!\!
& \Producer!\ARRIVE.\Red!\START.\Green!\START.\\
& \MOVEM(\text{co-ord of }\Producer).\Producer!\READY.\IDLEM.\\
& \ (\Producer?\RED.\Red!\ARRIVE.\Green!\FREE.\\
& \ \quad \MOVEM(\text{co-ord of }\Red).\Red!\READY.\\
& \  \quad \IDLEM.\Red?\OK.\procvar\\
& \ + \Producer?\GREEN.\textrm{ symmetrically for $\Green$ })
\end{array}
& 
\begin{array}{rl}\small
\Producer:\!\!\!\!\!\!\!\!\!\!\\
\mu \procvar.\!\!\!\!\!\!& \Cart?\ARRIVE.\WORKM.\\ & \Cart?\READY.\PLACEM.\\
& (\Cart!\GREEN + \Cart!\RED).\WORKM.\procvar
% \\[2mm]
% \Red:
% \!\!\!\!\!\!\!\!\!\!\!\!\\
% \Green:\!\!\!\!\!\!\!\!\!\!\!\!\\
% \mu \procvar.\!\!\!\!\!\!& \Cart?\START.\WORKM.\\
% & \ ((\Cart?\ARRIVE.\WORKM.\Cart?\READY.\\& \quad \ \PICK.\Cart!\OK)\\
%     & \ + (\Cart?\FREE.\WORKM)).\procvar\\
\end{array}    
\end{array}  
\]
\end{comment}

\myparagraph{Local Types}
The local types for the components are:
\begin{align*}
\small
\begin{array}{c|c}
\small
\begin{array}{rl}
%
\Cart:\!\!\!\!\!\!\\
\mu \ty. & \Producer!\ARRIVE(t).\Red!\START.\Green!\START.\\
        & \motion{\dtsess}{\MOVEM(\Producer)}.\Producer!\READY.\motion{\dtsess}{\IDLEM}.\\
	& (\ (\Producer?\GREEN.\Green!\ARRIVE(t).\Red!\FREE.\\
        & \ \ \motion{\dtsess}{\MOVEM(\Green)}.\Green!\READY.\\
        & \ \ \motion{\dtsess}{\IDLEM}.\Green?\OK) \\
        & \& \ (\Producer?\RED. \ldots \text{symmetric} \ldots)\ ).\ty
\end{array}
&
\begin{array}{l}
\Producer:\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\\
\quad\mu \ty.  \Cart?\ARRIVE(t).\motion{\dtsess}{\WORKM}.\Cart?\READY.\motion{\dtsess}{\PLACEM}.\\
	 \quad\quad (\Cart!\GREEN.\motion{\dtsess}{\WORKM}.\ty\; \oplus \; \Cart!\RED.\motion{\dtsess}{\WORKM}.\ty)\\
\Red,\Green:\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\\
\quad\mu \ty.  (\Cart?\START.\motion{\dtsess}{\WORKM}.\\
          \quad\quad(\ (\Cart?\ARRIVE(t).\motion{\dtsess}{\WORKM}.\\
          \quad\quad      \Cart?\READY.\motion{\dtsess}{\PICKM}.\Cart!\OK) \\
          \quad\quad\& \; (\Cart?\FREE.\motion{\dtsess}{\WORKM}) \ ).\ty
\end{array}
\end{array}
\end{align*}
%
We can show that all the processes type check.
From the soundness theorems, we conclude that the example 
satisfies communication safety, motion compatibility, and collision freedom.



==> related.tex <==
\section{Related Work}
\label{sec:related}

% There are many instances of complex, concurrent, robotic systems in the world.  Indeed, 
The field of concurrent robotics has made enormous progress---from robot soccer to
self-driving systems and to industrial manufacturing.
However, to the best of our knowledge, none of these impressive systems come with formal
guarantees of correctness.
Our motivation, like many other similar projects in the area of high-confidence robotics and cyber-physical systems design, is to 
be able to reason formally about such systems.

A spectrum of computer-assisted formal methods techniques can be, and have been, applied to reasoning about concurrent robotics,
ranging from interactive theorem proving to automated analysis via model checking.
As is well known, these techniques provide a tradeoff between manual effort and the expressiveness of
specifications and the strength of guarantees.
Our choice using manually specified choreographies and motion primitive specifications and automatically
checked type correctness attempts to explore a point in the design space that requires manual abstraction
of motion and geometry but provides automated checks for the interaction.
We build on a type-based foundation rather than global model checking to again reflect the tradeoff:
our use of choreographies and projections from global to local types restricts the structure of programs
that can be type checked but enables a more scalable \emph{local} check for each process; 
in contrast, a model checking approach could lead to state-space explosion already at the level of concurrency.



% multiparty session types
There are a vast number of extensions and applications of session
types and choreographies~\cite{Huttel:2016:FST:2911992.2873052,ABBCCDGGGHJMMMNNPVY2016,BETTY2017},
but little work bringing types to practical programming in the domain of robotics or cyber-physical systems.
We discuss the most related work. 
Our starting point was the theory of motion session types and PGCD \cite{PGCD,ECOOP19}, whose goals are
similar to ours.
We considerably extend the scope and expressiveness of motion session types:
through \emph{continuous-time} motion primitives and through separating conjunction for modular synchronisation.
% As \Sec~\ref{sec:eval} indicates, the more expressiveness has advantages in scaling verification.

Syntactic extensions  
of original global types \cite{HYC08} to represent more expressive
communication structures have been studied, 
e.g.,~in \cite{DBLP:conf/popl/LangeTY15}, 
in the context of synthesis from communicating
automata; in~\cite{DBLP:journals/corr/abs-1203-0780} to include 
parallel and choices; in \cite{DH2012} 
to represent nested global types.
Our aim is to include the minimum syntax extension to 
\cite{HYC08} to represent separation and synchronisations 
best suited to implementing robotics applications. 
In turn, a combination of motion primitives and predicates 
required us to develop a novel and non-trivial data flow analysis of 
global choreographies for the well-formedness check.

%To ensure the progress and liveness properties, 
%the framework requires several additional conditions 
%on the shape of global protocols
%and a limitation to the recursion
%where in the loop, the clock should be always reset. 
%The mechanism is implemented in 
%runtime monitoring in Python by \citet{NeykovaBY17}.  
% The most recent work in \cite{BMVY2019}
% proposed a timed $\pi$-calculus
% which increases the modelling power 
% from \cite{BYY2014}, adding a blocking receive primitive
% with timeout, and a primitive that consumes
% an arbitrary amount of time in a given range.
% Moreover, the theory is not applicable in our setting as the focus
% is on timing behaviours of \emph{binary} session types.
% Apart from a scope of \cite{BMVY2019} is limited to theory, 
% there are two technical limitations 
% in \cite{BMVY2019}: first their theory
% treats only \emph{binary} session types;
% and in their system, the subject reduction theorem does \emph{not}
% hold unless one assumes that all composed processes make progress.
% Note that a progress property 
% cannot be guaranteed
% in binary session types 
% in general (if there are more than two parties)
% due to interleaved sessions. 
% Our framework based on motion primitives can specify
% timed behaviours and synchronisations among multiple components and typable
% processes can automatically ensure progress and liveness of
% communications, together with collision freedom.  


Hybrid extensions to process algebras \cite{RoundsS03,DBLP:journals/iandc/LynchSV03,BERGSTRA2005215,DBLP:conf/aplas/LiuLQZZZZ10}
extend process algebras with hybrid behaviour and
study classical concurrency issues such as process equivalences.
Extensions to timed (but not hybrid) specifications in the $\pi$-calculus are studied in  
\citet{BYY2014,BMVY2019} to  
express properties on times on top of \emph{binary} session typed processes. 

The theory of hybrid automata \cite{ACHH,Henzinger96} provides a foundation for verifying
models of hybrid systems.
The main emphasis in hybrid automaton research has been in defining semantics and designing
model checking algorithms---too many to enumerate, see \cite{Henzinger96,Platzer18}---and 
not on programmability. 
% In particular, most analysis techniques for hybrid automata construct the product automaton to reason about concurrent subsystems.
Assume guarantee reasoning for hybrid systems
has been studied, e.g.~\cite{Nuzzo:EECS-2015-189,DBLP:journals/fteda/BenvenisteCNPRR18,DBLP:journals/pieee/NuzzoSBGV15,DBLP:journals/pieee/Tripakis16}.
These works do not consider programmability or choreography aspects.


% deductive verification for hybrid systems
Deductive verification for hybrid systems attempts to define logics and invariant-based reasoning to hybrid systems.
% We have already mentioned the logics {\sc Hoare}${}^\dt$ \cite{DBLP:conf/icalp/SuenagaH11} as a starting point for our program logic.
Differential dynamic logic (dL) \cite{Platzer18,PlatzerT18} is a general logical framework to deductively reason about hybrid systems.
It extends \emph{dynamic logic} with differential operators and shows sound and (relatively) complete axiomatisations for the logic.
Keymaera \cite{DBLP:conf/cade/FultonMQVP15} and HHL Prover \cite{HHL} are interactive theorem provers based on hybrid progam logics. 
These tools can verify complex properties of systems at the cost of intensive manual effort.
In contrast, we explore a point in the design space with more automation but less expressiveness.
The ``trusted base'' in an interactive theorem prover is the core logic; optimizing the trusted base was not one of our goals.

A well-studied workflow in high-confidence cyber-physical systems is model-based design (see, e.g., \cite{HenzingerSifakis07} for an overview), 
where a system is constructed by successive refinement of an abstract model down to an implementation.
An important problem in model-based design is to ensure property-preserving refinement: one verifies properties of the system
at higher levels of abstraction, and ensures that properties are preserved through refinement.
In the presence of continuous dynamics, defining an appropriate notion of refinement and proving property-preserving
compilation formally are hard problems \cite{DBLP:journals/tosem/YanJWWZ20,DBLP:conf/pldi/BohrerTMMP18}.

In our implementation, we use \emph{automated} tools based on the dReal SMT solver \cite{dReal}.
Our verification is \emph{semi-automatic}, as we require user annotations for footprints or for
the motion primitive specifications, but discharge verification conditions through dReal.
Of course, there are programs that go past the capability of the solver---this
is already true for systems that \emph{only} have concurrency or only deal with dynamics. 
Our proof rules is to allow sound reasoning, potentially inside an interactive prover. 
Our implementation shows that---at least some---nontrivial examples do allow automation.
Non-linear arithmetic is difficult to scale.
Our observation is that a combination of manual specification of \emph{abstract} footprints
that replace complex geometrical shapes with simpler over-approximations along with the power of
state-of-the-art SMT solvers is reasonably effective even for complicated examples. 

Our choice of dReal (as opposed to a different SMT solver) is dReal's ``off the shelf'' support
for non-linear arithmetic and trigonometric functions. 
Trigonometry shows up in our handling of frame shifts. 
Note that dReal only considers $\delta$-decidability and can be incomplete in theory.
We expect that most implementations will be collision free in a ``robust'' way 
(that is, two robots will not just not collide, they would be separated by a minimum distance).
Therefore we believe the potential incompleteness is less of a concern.
Indeed, the main limiting factor in our experiments was scalability for larger verification conditions.



% Planning systems
Formal methods have been applied to multi-robot planning \cite{Drona,Antlab}.
These systems ignore programming or geometry concerns and view robots as sequences of motion primitives. 

\begin{comment}
% assume guarantee reasoning for hybrid systems, contracts
Assume guarantee reasoning for hybrid systems
has been studied, e.g.~\cite{Nuzzo:EECS-2015-189,DBLP:journals/fteda/BenvenisteCNPRR18,DBLP:journals/pieee/NuzzoSBGV15,DBLP:journals/pieee/Tripakis16}.
However, much of this work is described at the level of abstract models and not at the level of programs.
Moreover, usually assume guarantee reasoning and contracts do not, at the same time, consider the effects of message based
synchronisation.
Our work shows how assume guarantee contracts can be propagated through program syntax.


% Planning systems
Systems such as Drona \cite{Drona} or Antlab \cite{Antlab}
model robots as discrete systems with motion primitives, and the main technical contribution is 
to perform temporal multi-agent non-modular planning for tasks. 
Instead, we provide a concurrency model, a modular typing discipline, and proof rules that model correct 
interaction between dynamics 
(time is ignored in other task management and synthesis systems beyond atomic discrete-time motion primitives) 
and concurrency, and geometry (also ignored in these systems---robots are ``point objects”).

% Hybrid automata
The theory of hybrid automata \cite{ACHH,Henzinger96} provides a foundation for verifying
abstract models of hybrid systems.
The main emphasis in hybrid automaton research has been in defining semantics and designing
model checking algorithms---too many to enumerate, see \cite{Henzinger96,Platzer18}---and 
not on programmability or compositional reasoning.
In particular, most analysis techniques for hybrid automata construct the product automaton to reason
about concurrent subsystems.
Hybrid extensions to process algebras \cite{RoundsS03,DBLP:journals/iandc/LynchSV03,BERGSTRA2005215} extend process algebras with hybrid behaviour;
the emphasis is to define a formal model and study classical concurrency issues such as process equivalences.

% languages for hybrid systems
Programming languages incorporating hybrid behaviour have been studied in the synchronous programming literature \cite{Zelus,Averest}.
Hybrid synchronous languages, such as Zelus, extend a synchronous model with differential equations to capture
continuous-time evolution of state.
While these languages come with simulation, verification, and compilation tools, they restrict concurrency
and there is little work in compositional reasoning or geometric reasoning. 

% nonstandard semantics for hybrid systems
The use of nonstandard models to provide semantics to hybrid systems goes
back to Iwasaki et al.~\cite{DBLP:conf/ijcai/IwasakiFSBG95}.
Our inspiration came from the use of nonstandard analysis to provide semantics for hybrid synchronous
languages \cite{DBLP:journals/fuin/BliudzeK09,DBLP:journals/jcss/BenvenisteBCP12,DBLP:conf/hybrid/BenvenisteBCPP14}. 
\citet{DBLP:conf/icalp/SuenagaH11,DBLP:conf/cav/HasuoS12} give a nonstandard semantics for a hybrid ``while-language'' 
and use it as the basis for deductive program verification and static analysis \cite{DBLP:conf/vmcai/KidoCH16}.
In all these approaches, the discrete steps appear because of evaluating predicates: the semantics
provides a clear notion of when a signal crosses zero.
The languages do not have additional concurrency features, such as synchronisation through messages.
Moreover, none of the existing approaches consider compositional proof systems and, in particular, local
reasoning based on physical-variables-as-resource.







% geometric reasoning 
\citet{CardelliG12} define a process algebra for geometric interaction.
Their formalism combines communication and frame shifting.
However, they do not consider dynamics,  which is crucial in a robotics context.
% Moreover, the objective in their process algebra is an abstraction theorem, and not reasoning about programs.
% Spatial logics have also been explored from a topological perspective~\cite{lmcs:2067} 
% where the modal operators describe neighborhood relations.
% Such logics can express and check properties about arrangements, but do not model dynamics. 

% concurrent separation logics, resource reasoning
We were inspired by concurrent separation logics, which combine reasoning about concurrency, 
state, and separation \cite{CSL,JungSSSTBD15,DBLP:conf/wollic/GardnerZ07,DBLP:conf/concur/VafeiadisP07}.
These logics have mostly been studied for discrete systems, but our nonstandard view makes them applicable to 
continuous systems as well.
Our reasoning about geometric separation and about passing permissions through predicate refinements is reminiscent
of similar principles in concurrent separation logics.
The main obstacle to using separation logics in our context is the use of frame shifts, which make the footprint of a process
not a local property of a process but the property of its ancestors in the attached composition.
It is an interesting open problem to model geometric space as a resource in an appropriate separation logic;
we leave it for future work.
\end{comment}











\section{Discussion and Future Directions}
\label{sec:discussion}

% In this paper, we have made progress in compositional
% reasoning about concurrent robotic applications, both in setting out the foundations 
% (choreography types+motion+geometry) and in developing infrastructure for verifying
% and implementing concurrent robots on commercial and open source infrastructure.

In this paper, we have shown how choreographies can be extended with dynamic motion primitives to enable compositional
reasoning in the presence of continuous-time dynamics. 
We have developed an automated verification tool and a compiler from type-correct programs to distributed
robotics applications using ROS and commercial and custom-made robotics hardware.
Our goal is to \emph{integrate} types and static analysis techniques into existing robotics frameworks,
rather than provide fully verified stacks (see, e.g., \cite{DBLP:conf/pldi/BohrerTMMP18}). 
We explain our language features in terms of a calculus but session processes 
can be easily embedded into existing frameworks for robot programming. %---indeed, we integrate our programs with ROS.
% 
We have demonstrated that the language and type system are expressive enough to statically verify 
distributed manoeuvres on top of existing hardware and software. 
% Furthermore, the compositionality offered by choreographic type systems and our use of separating conjunction
% are crucial to verify complex examples.
% To the best of our knowledge, no existing static verification or typing system allows modelling,
% statically verifying, and implementing the kind of complex robotics coordinations---including concurrency, dynamics,
% and geometry---on real robots working in real physical environments that we can handle.

We view our paper as a first step in verifying robotics programs.
There are many other important but yet unmodelled aspects.
We outline several directions not addressed in our work.
%  indeed, each direction likely requires significant advances that go beyond the scope of any one paper. 

For example, we omit \emph{probabilistic robotics} aspects, including the perception stack (vision, LIDAR, etc.),
and aspects such as filtering, localisation, and mapping
% , or higher-level mission planning 
\cite{ProbabilisticRobotics,LaValle2012}.
These will require a probabilistic extension to our theory. 
Such a theory requires a nontrivial extension of program logics and analyses for probabilistic programs \cite{McIverMorgan} with
the verification and synthesis for stochastic continuous-state systems \cite{ZamaniEMAL14}.
We also omit any modeling of the perception stack or dynamic techniques, often based on machine learning, of learning the environment.
Instead, our models \emph{assume} worst-case disturbance bounds on the sensing or dynamics.
We believe an integration of learning techniques with formal methods is an interesting challenge
but goes beyond the scope of this paper.

Our framework statically verifies properties of a program.
In practice, robots work in dynamic, often unknown, environments \cite{LaValle,LaValle2012,Siegwart,ProbabilisticRobotics}.
When confronted with a formal method, domain experts often expect that
a verification methodology should be able to verify correctness of behaviors in an \emph{arbitrary} dynamic environment
and any failure to do so simply shows the inadequacy of verification techniques.
Formal methods cannot prove correctness in an \emph{arbitrary} dynamic environment.
When we verify a system, it is---as true in any formal methods---\emph{relative} to an environment assumption;
such assumptions are usually implicit in robotics implementations.
Thus, we can model moving obstacles, etc.\ in the environment through assumptions on the behaviour
of such obstacles (e.g., limits on their speed or trajectories); these assumptions are propagated
by our assume-guarantee proof system, and show up as a premise in the eventual correctness proof.
% We have not considered distributed feedback control strategies that are necessary for strongly coupled systems 
% (e.g., two robots simultaneously manipulating the same object).

We focus on communication safety and collision freedom as the basic correctness conditions any
system has to satisfy.
An interesting next step is to extend the reasoning to more expressive specifications.
For safety specifications, such as invariants, one could reduce the problem to checking
communication safety.
For liveness specifications, the proof system would need to be extended with ranking arguments.
% We also ignore Zeno behaviours that can cause an unbounded number of transitions within finite time.
% It is possible to reason it in a type-based setting \cite{DBLP:conf/hybrid/BenvenisteBCPP14,BLY2015}.

While all the above problems are interesting in their own right, they are orthogonal to our main contribution that 
one can reason about concurrency and dynamics in continuous time in a type-based setting. 
Our future work will look at more expressive scenarios, but the setting in our paper already required complex proofs and it 
was important for us to get the core correct.
%
We believe a verification system that can faithfully model and uniformly reason about more complex interactions and that scales
to larger implementations remains a grand challenge in computer science (see, e.g., \cite{Lozano-Perez} for an articulation of these challenges).


